Jagged-time-step technique improving convergence order of Fernandez's Explicit Robin-Neumann scheme for the coupling of incompressible fluid with thin-walled structure

Inspired by Rybak's multiple-time-step technique, jagged-time-step technique is proposed and applied to Fernandez's Explicit Robin-Neumann scheme. For some instances, numerical experiments demonstrate higher convergence orders and accuracy with lower computation cost as time and space get refined.

==> convRate/convRateAll0-4 <==

Number of fluid steps= 1 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02579 &	 -0.0367354 \\
2 &			 1.07106 &	 -0.0623039 \\
3 &			 1.08424 &	 -0.0176448 \\
4 &			 0.805303 &	 0.429081 \\
Number of fluid steps= 1 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02893 &	 -0.0411448 \\
2 &			 1.0859 &	 -0.0777464 \\
3 &			 1.08077 &	 0.00683172 \\
4 &			 0.725089 &	 0.57583 \\
Number of fluid steps= 1 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03021 &	 -0.0429384 \\
2 &			 1.09474 &	 -0.0876498 \\
3 &			 1.07887 &	 0.0210672 \\
4 &			 0.691975 &	 0.640729 \\
Number of fluid steps= 1 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03107 &	 -0.0441423 \\
2 &			 1.10104 &	 -0.0947246 \\
3 &			 1.07801 &	 0.0304963 \\
4 &			 0.674954 &	 0.675509 \\
Number of fluid steps= 1 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03185 &	 -0.0452333 \\
2 &			 1.10574 &	 -0.0997789 \\
3 &			 1.07764 &	 0.0371369 \\
4 &			 0.664974 &	 0.696505 \\
Number of fluid steps= 1 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03265 &	 -0.0463514 \\
2 &			 1.10936 &	 -0.103376 \\
3 &			 1.07749 &	 0.0420531 \\
4 &			 0.658577 &	 0.71025 \\
Number of fluid steps= 1 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03349 &	 -0.0475244 \\
2 &			 1.11221 &	 -0.105905 \\
3 &			 1.07747 &	 0.0457815 \\
4 &			 0.654208 &	 0.719826 \\
Number of fluid steps= 1 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03437 &	 -0.0487523 \\
2 &			 1.11452 &	 -0.10767 \\
3 &			 1.0775 &	 0.0487346 \\
4 &			 0.651074 &	 0.726794 \\
Number of fluid steps= 1 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03529 &	 -0.0500349 \\
2 &			 1.11643 &	 -0.108858 \\
3 &			 1.07757 &	 0.0511112 \\
4 &			 0.648741 &	 0.732067 \\
Number of fluid steps= 1 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03624 &	 -0.0513582 \\
2 &			 1.11802 &	 -0.109588 \\
3 &			 1.07765 &	 0.0530573 \\
4 &			 0.64695 &	 0.736163 \\
Number of fluid steps= 1 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03723 &	 -0.0527358 \\
2 &			 1.11937 &	 -0.109951 \\
3 &			 1.07774 &	 0.0546778 \\
4 &			 0.64554 &	 0.739431 \\
Number of fluid steps= 1 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03824 &	 -0.05414 \\
2 &			 1.12052 &	 -0.110028 \\
3 &			 1.07782 &	 0.0560521 \\
4 &			 0.644406 &	 0.742074 \\
Number of fluid steps= 1 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03927 &	 -0.0555705 \\
2 &			 1.12152 &	 -0.109885 \\
3 &			 1.07791 &	 0.0572186 \\
4 &			 0.64348 &	 0.74427 \\
Number of fluid steps= 1 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04032 &	 -0.0570274 \\
2 &			 1.12239 &	 -0.109547 \\
3 &			 1.07799 &	 0.0582303 \\
4 &			 0.64271 &	 0.746104 \\
Number of fluid steps= 1 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04139 &	 -0.0585105 \\
2 &			 1.12316 &	 -0.109053 \\
3 &			 1.07807 &	 0.0591126 \\
4 &			 0.642062 &	 0.747666 \\
Number of fluid steps= 1 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04247 &	 -0.0600059 \\
2 &			 1.12384 &	 -0.108431 \\
3 &			 1.07815 &	 0.0598787 \\
4 &			 0.641511 &	 0.749012 \\
Number of fluid steps= 1 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04356 &	 -0.0615136 \\
2 &			 1.12444 &	 -0.107693 \\
3 &			 1.07822 &	 0.0605551 \\
4 &			 0.641037 &	 0.750172 \\
Number of fluid steps= 1 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04465 &	 -0.0630197 \\
2 &			 1.12499 &	 -0.106893 \\
3 &			 1.07829 &	 0.0611669 \\
4 &			 0.640627 &	 0.751189 \\
Number of fluid steps= 1 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04575 &	 -0.064538 \\
2 &			 1.12548 &	 -0.106002 \\
3 &			 1.07835 &	 0.0617149 \\
4 &			 0.640267 &	 0.75208 \\
Number of fluid steps= 1 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04684 &	 -0.066041 \\
2 &			 1.12592 &	 -0.105063 \\
3 &			 1.07841 &	 0.0621985 \\
4 &			 0.639951 &	 0.752872 \\
Number of fluid steps= 2 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0247 &	 -0.0352016 \\
2 &			 1.06366 &	 -0.0538355 \\
3 &			 1.10668 &	 -0.0572011 \\
4 &			 1.12766 &	 -0.027094 \\
Number of fluid steps= 2 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02422  &  \\
1 &			 1.06849 &	 -0.0610478 \\
2 &			 1.08069 &	 -0.0163793 \\
3 &			 0.805655 &	 0.423719 \\
4 &			 0.471993 &	 0.771397 \\
Number of fluid steps= 2 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02415  &  \\
1 &			 1.0694 &	 -0.0623745 \\
2 &			 1.07651 &	 -0.00956014 \\
3 &			 0.773582 &	 0.476736 \\
4 &			 0.418724 &	 0.885555 \\
Number of fluid steps= 2 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0271  &  \\
1 &			 1.08208 &	 -0.0752305 \\
2 &			 1.07524 &	 0.00914845 \\
3 &			 0.725441 &	 0.567729 \\
4 &			 0.352577 &	 1.04092 \\
Number of fluid steps= 2 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02708  &  \\
1 &			 1.08129 &	 -0.0742049 \\
2 &			 1.07299 &	 0.0111169 \\
3 &			 0.715412 &	 0.58479 \\
4 &			 0.333159 &	 1.10256 \\
Number of fluid steps= 2 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0283  &  \\
1 &			 1.09005 &	 -0.0841331 \\
2 &			 1.07201 &	 0.0240759 \\
3 &			 0.692031 &	 0.63141 \\
4 &			 0.305358 &	 1.18034 \\
Number of fluid steps= 2 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02844  &  \\
1 &			 1.08872 &	 -0.0821753 \\
2 &			 1.07082 &	 0.023917 \\
3 &			 0.688582 &	 0.637016 \\
4 &			 0.296455 &	 1.21582 \\
Number of fluid steps= 2 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02914  &  \\
1 &			 1.09565 &	 -0.0903478 \\
2 &			 1.07019 &	 0.0339201 \\
3 &			 0.674684 &	 0.665583 \\
4 &			 0.281762 &	 1.25973 \\
Number of fluid steps= 2 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02937  &  \\
1 &			 1.09407 &	 -0.0879434 \\
2 &			 1.06966 &	 0.0325527 \\
3 &			 0.673907 &	 0.666531 \\
4 &			 0.277339 &	 1.2809 \\
Number of fluid steps= 2 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02989  &  \\
1 &			 1.09978 &	 -0.0947247 \\
2 &			 1.0691 &	 0.0408182 \\
3 &			 0.664408 &	 0.686255 \\
4 &			 0.268271 &	 1.30838 \\
Number of fluid steps= 2 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03022  &  \\
1 &			 1.09814 &	 -0.0921095 \\
2 &			 1.06899 &	 0.0388136 \\
3 &			 0.664884 &	 0.685074 \\
4 &			 0.266073 &	 1.32128 \\
Number of fluid steps= 2 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03067  &  \\
1 &			 1.10291 &	 -0.0977326 \\
2 &			 1.0684 &	 0.0458632 \\
3 &			 0.657758 &	 0.699823 \\
4 &			 0.259827 &	 1.34001 \\
Number of fluid steps= 2 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03107  &  \\
1 &			 1.10134 &	 -0.0951176 \\
2 &			 1.06858 &	 0.043565 \\
3 &			 0.658866 &	 0.697638 \\
4 &			 0.258842 &	 1.34791 \\
Number of fluid steps= 2 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03148  &  \\
1 &			 1.10535 &	 -0.0997874 \\
2 &			 1.06793 &	 0.0496862 \\
3 &			 0.653173 &	 0.70928 \\
4 &			 0.254184 &	 1.36159 \\
Number of fluid steps= 2 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03196  &  \\
1 &			 1.10392 &	 -0.0972486 \\
2 &			 1.06829 &	 0.0473323 \\
3 &			 0.654607 &	 0.706602 \\
4 &			 0.253901 &	 1.36636 \\
Number of fluid steps= 2 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03233  &  \\
1 &			 1.10731 &	 -0.101155 \\
2 &			 1.0676 &	 0.052688 \\
3 &			 0.649855 &	 0.716181 \\
4 &			 0.250218 &	 1.37693 \\
Number of fluid steps= 2 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03288  &  \\
1 &			 1.10602 &	 -0.0987048 \\
2 &			 1.06809 &	 0.0503443 \\
3 &			 0.651454 &	 0.713298 \\
4 &			 0.25036 &	 1.37966 \\
Number of fluid steps= 2 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03322  &  \\
1 &			 1.10891 &	 -0.101995 \\
2 &			 1.06736 &	 0.0550954 \\
3 &			 0.647364 &	 0.721398 \\
4 &			 0.247319 &	 1.3882 \\
Number of fluid steps= 2 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03384  &  \\
1 &			 1.10777 &	 -0.0996454 \\
2 &			 1.06794 &	 0.0528278 \\
3 &			 0.649039 &	 0.718454 \\
4 &			 0.247726 &	 1.38956 \\
Number of fluid steps= 2 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03414  &  \\
1 &			 1.11024 &	 -0.10244 \\
2 &			 1.06719 &	 0.0570545 \\
3 &			 0.645436 &	 0.725471 \\
4 &			 0.245132 &	 1.39672 \\
Number of fluid steps= 3 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02354 &	 -0.0335675 \\
2 &			 1.05762 &	 -0.0472539 \\
3 &			 1.10304 &	 -0.0606637 \\
Number of fluid steps= 3 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01313  &  \\
1 &			 1.06469 &	 -0.0716141 \\
2 &			 1.09962 &	 -0.0465716 \\
3 &			 1.03727 &	 0.0842136 \\
4 &			 0.981679 &	 0.0794682 \\
Number of fluid steps= 3 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04252  &  \\
1 &			 1.09027 &	 -0.0646104 \\
2 &			 0.951307 &	 0.196703 \\
3 &			 0.596548 &	 0.673273 \\
4 &			 0.343489 &	 0.796374 \\
Number of fluid steps= 3 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04247  &  \\
1 &			 1.09073 &	 -0.0652882 \\
2 &			 0.946816 &	 0.204138 \\
3 &			 0.576965 &	 0.7146 \\
4 &			 0.315791 &	 0.869514 \\
Number of fluid steps= 3 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04502  &  \\
1 &			 1.09774 &	 -0.0710058 \\
2 &			 0.929583 &	 0.239881 \\
3 &			 0.535769 &	 0.794973 \\
4 &			 0.271903 &	 0.978519 \\
Number of fluid steps= 3 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04967  &  \\
1 &			 1.09917 &	 -0.0664787 \\
2 &			 0.900469 &	 0.287666 \\
3 &			 0.486974 &	 0.886832 \\
4 &			 0.22842 &	 1.09216 \\
Number of fluid steps= 3 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04977  &  \\
1 &			 1.10084 &	 -0.0685315 \\
2 &			 0.903779 &	 0.284563 \\
3 &			 0.483912 &	 0.901225 \\
4 &			 0.21979 &	 1.13862 \\
Number of fluid steps= 3 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05132  &  \\
1 &			 1.10445 &	 -0.0711262 \\
2 &			 0.896367 &	 0.301167 \\
3 &			 0.467804 &	 0.938185 \\
4 &			 0.204279 &	 1.19536 \\
Number of fluid steps= 3 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05397  &  \\
1 &			 1.10264 &	 -0.065128 \\
2 &			 0.877891 &	 0.328848 \\
3 &			 0.442289 &	 0.989052 \\
4 &			 0.184334 &	 1.26267 \\
Number of fluid steps= 3 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05414  &  \\
1 &			 1.10473 &	 -0.0676273 \\
2 &			 0.882649 &	 0.323782 \\
3 &			 0.443573 &	 0.992668 \\
4 &			 0.181382 &	 1.29014 \\
Number of fluid steps= 3 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05549  &  \\
1 &			 1.10699 &	 -0.0687293 \\
2 &			 0.878861 &	 0.332935 \\
3 &			 0.435511 &	 1.01293 \\
4 &			 0.174017 &	 1.32348 \\
Number of fluid steps= 3 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0574  &  \\
1 &			 1.10439 &	 -0.0627285 \\
2 &			 0.865651 &	 0.351392 \\
3 &			 0.419359 &	 1.0456 \\
4 &			 0.16257 &	 1.36712 \\
Number of fluid steps= 3 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05758  &  \\
1 &			 1.10652 &	 -0.0652627 \\
2 &			 0.870541 &	 0.346045 \\
3 &			 0.422064 &	 1.04445 \\
4 &			 0.1619 &	 1.38236 \\
Number of fluid steps= 3 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05882  &  \\
1 &			 1.10809 &	 -0.0656177 \\
2 &			 0.86837 &	 0.351693 \\
3 &			 0.417401 &	 1.05688 \\
4 &			 0.157817 &	 1.40318 \\
Number of fluid steps= 3 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06032  &  \\
1 &			 1.10536 &	 -0.0600166 \\
2 &			 0.858139 &	 0.365233 \\
3 &			 0.405899 &	 1.08009 \\
4 &			 0.150262 &	 1.43364 \\
Number of fluid steps= 3 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0605  &  \\
1 &			 1.10742 &	 -0.0624579 \\
2 &			 0.862815 &	 0.360079 \\
3 &			 0.409059 &	 1.07674 \\
4 &			 0.150632 &	 1.44128 \\
Number of fluid steps= 3 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06164  &  \\
1 &			 1.1086 &	 -0.0624443 \\
2 &			 0.861475 &	 0.363858 \\
3 &			 0.406094 &	 1.085 \\
4 &			 0.148135 &	 1.4549 \\
Number of fluid steps= 3 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06287  &  \\
1 &			 1.10596 &	 -0.0573341 \\
2 &			 0.853126 &	 0.374468 \\
3 &			 0.397253 &	 1.1027 \\
4 &			 0.142653 &	 1.47755 \\
Number of fluid steps= 3 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06303  &  \\
1 &			 1.1079 &	 -0.0596454 \\
2 &			 0.857502 &	 0.369616 \\
3 &			 0.4005 &	 1.09834 \\
4 &			 0.143526 &	 1.48049 \\
Number of fluid steps= 3 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06407  &  \\
1 &			 1.10884 &	 -0.0594581 \\
2 &			 0.856635 &	 0.372299 \\
3 &			 0.398485 &	 1.10416 \\
4 &			 0.141888 &	 1.48977 \\
Number of fluid steps= 4 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02244 &	 -0.0320162 \\
2 &			 1.05271 &	 -0.0420919 \\
3 &			 1.09311 &	 -0.0543305 \\
Number of fluid steps= 4 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02211  &  \\
1 &			 1.05944 &	 -0.0517514 \\
2 &			 1.10144 &	 -0.056089 \\
3 &			 1.12424 &	 -0.0295591 \\
4 &			 1.18376 &	 -0.0744266 \\
Number of fluid steps= 4 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04061  &  \\
1 &			 1.08993 &	 -0.066806 \\
2 &			 1.04319 &	 0.0632335 \\
3 &			 0.897305 &	 0.217332 \\
4 &			 0.814145 &	 0.140313 \\
Number of fluid steps= 4 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05847  &  \\
1 &			 1.06556 &	 -0.00963145 \\
2 &			 0.806965 &	 0.401034 \\
3 &			 0.477817 &	 0.756048 \\
4 &			 0.274237 &	 0.801035 \\
Number of fluid steps= 4 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05869  &  \\
1 &			 1.06748 &	 -0.0119288 \\
2 &			 0.807415 &	 0.402827 \\
3 &			 0.466344 &	 0.791916 \\
4 &			 0.258064 &	 0.853666 \\
Number of fluid steps= 4 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0591  &  \\
1 &			 1.06043 &	 -0.00181058 \\
2 &			 0.775891 &	 0.450723 \\
3 &			 0.425638 &	 0.866227 \\
4 &			 0.227285 &	 0.905124 \\
Number of fluid steps= 4 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0639  &  \\
1 &			 1.06385 &	 6.78038e-05 \\
2 &			 0.761163 &	 0.483017 \\
3 &			 0.39875 &	 0.932721 \\
4 &			 0.198898 &	 1.00346 \\
Number of fluid steps= 4 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06753  &  \\
1 &			 1.0523 &	 0.0207306 \\
2 &			 0.726742 &	 0.534031 \\
3 &			 0.360135 &	 1.01291 \\
4 &			 0.170355 &	 1.07999 \\
Number of fluid steps= 4 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.068  &  \\
1 &			 1.05601 &	 0.0162882 \\
2 &			 0.733139 &	 0.526465 \\
3 &			 0.360068 &	 1.02582 \\
4 &			 0.166162 &	 1.11568 \\
Number of fluid steps= 4 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06685  &  \\
1 &			 1.05 &	 0.022968 \\
2 &			 0.71699 &	 0.550364 \\
3 &			 0.341163 &	 1.07149 \\
4 &			 0.152242 &	 1.16409 \\
Number of fluid steps= 4 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07054  &  \\
1 &			 1.05348 &	 0.0231758 \\
2 &			 0.713385 &	 0.56241 \\
3 &			 0.333678 &	 1.09622 \\
4 &			 0.144971 &	 1.20269 \\
Number of fluid steps= 4 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07245  &  \\
1 &			 1.04401 &	 0.0387749 \\
2 &			 0.692166 &	 0.592946 \\
3 &			 0.313105 &	 1.14447 \\
4 &			 0.131393 &	 1.25276 \\
Number of fluid steps= 4 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07295  &  \\
1 &			 1.04768 &	 0.0343847 \\
2 &			 0.699036 &	 0.583759 \\
3 &			 0.31579 &	 1.1464 \\
4 &			 0.130557 &	 1.27429 \\
Number of fluid steps= 4 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07127  &  \\
1 &			 1.04302 &	 0.0385553 \\
2 &			 0.688734 &	 0.598748 \\
3 &			 0.30437 &	 1.17812 \\
4 &			 0.121974 &	 1.31925 \\
Number of fluid steps= 4 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0744  &  \\
1 &			 1.0464 &	 0.0380968 \\
2 &			 0.68863 &	 0.603634 \\
3 &			 0.302521 &	 1.18669 \\
4 &			 0.120325 &	 1.3301 \\
Number of fluid steps= 4 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07566  &  \\
1 &			 1.03863 &	 0.0505403 \\
2 &			 0.673546 &	 0.624833 \\
3 &			 0.289224 &	 1.21959 \\
4 &			 0.112203 &	 1.36608 \\
Number of fluid steps= 4 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07617  &  \\
1 &			 1.042 &	 0.0465507 \\
2 &			 0.680021 &	 0.615704 \\
3 &			 0.292655 &	 1.21638 \\
4 &			 0.112658 &	 1.37725 \\
Number of fluid steps= 4 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07423  &  \\
1 &			 1.03834 &	 0.049024 \\
2 &			 0.672678 &	 0.626291 \\
3 &			 0.284841 &	 1.23976 \\
4 &			 0.1067 &	 1.4166 \\
Number of fluid steps= 4 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07694  &  \\
1 &			 1.04147 &	 0.0483166 \\
2 &			 0.67379 &	 0.62825 \\
3 &			 0.284958 &	 1.24155 \\
4 &			 0.106918 &	 1.41424 \\
Number of fluid steps= 4 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07784  &  \\
1 &			 1.0349 &	 0.0586517 \\
2 &			 0.662125 &	 0.644316 \\
3 &			 0.275323 &	 1.26598 \\
4 &			 0.101352 &	 1.44175 \\
Number of fluid steps= 5 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02143 &	 -0.0305903 \\
2 &			 1.04866 &	 -0.0379567 \\
Number of fluid steps= 5 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01738  &  \\
1 &			 1.05626 &	 -0.0541064 \\
2 &			 1.10178 &	 -0.0608712 \\
3 &			 1.15591 &	 -0.0691929 \\
Number of fluid steps= 5 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02705  &  \\
1 &			 1.08496 &	 -0.0791354 \\
2 &			 1.0859 &	 -0.0012494 \\
3 &			 1.0672 &	 0.0250607 \\
4 &			 1.10536 &	 -0.0506857 \\
Number of fluid steps= 5 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06455  &  \\
1 &			 1.08133 &	 -0.0225632 \\
2 &			 0.949449 &	 0.187644 \\
3 &			 0.771417 &	 0.29958 \\
4 &			 0.683357 &	 0.174871 \\
Number of fluid steps= 5 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06545  &  \\
1 &			 1.00699 &	 0.0814135 \\
2 &			 0.693507 &	 0.538067 \\
3 &			 0.403654 &	 0.780791 \\
4 &			 0.229625 &	 0.813839 \\
Number of fluid steps= 5 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06652  &  \\
1 &			 1.01123 &	 0.0767999 \\
2 &			 0.696872 &	 0.537146 \\
3 &			 0.396303 &	 0.81429 \\
4 &			 0.219097 &	 0.855034 \\
Number of fluid steps= 5 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06569  &  \\
1 &			 1.00365 &	 0.0865316 \\
2 &			 0.672788 &	 0.577032 \\
3 &			 0.368056 &	 0.870227 \\
4 &			 0.199518 &	 0.883406 \\
Number of fluid steps= 5 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06848  &  \\
1 &			 0.995372 &	 0.102252 \\
2 &			 0.650266 &	 0.614206 \\
3 &			 0.340737 &	 0.932371 \\
4 &			 0.175954 &	 0.95346 \\
Number of fluid steps= 5 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07032  &  \\
1 &			 0.989864 &	 0.11274 \\
2 &			 0.630087 &	 0.651679 \\
3 &			 0.317005 &	 0.991045 \\
4 &			 0.15679 &	 1.01567 \\
Number of fluid steps= 5 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0701  &  \\
1 &			 0.969327 &	 0.14269 \\
2 &			 0.596856 &	 0.699601 \\
3 &			 0.286723 &	 1.05773 \\
4 &			 0.136658 &	 1.06909 \\
Number of fluid steps= 5 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07161  &  \\
1 &			 0.97506 &	 0.136217 \\
2 &			 0.60425 &	 0.690345 \\
3 &			 0.287735 &	 1.0704 \\
4 &			 0.1344 &	 1.09821 \\
Number of fluid steps= 5 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07029  &  \\
1 &			 0.971898 &	 0.139125 \\
2 &			 0.593959 &	 0.710442 \\
3 &			 0.275873 &	 1.10636 \\
4 &			 0.125772 &	 1.13319 \\
Number of fluid steps= 5 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07208  &  \\
1 &			 0.967564 &	 0.147984 \\
2 &			 0.584823 &	 0.726357 \\
3 &			 0.26601 &	 1.13652 \\
4 &			 0.118319 &	 1.1688 \\
Number of fluid steps= 5 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0723  &  \\
1 &			 0.964902 &	 0.152254 \\
2 &			 0.575995 &	 0.744326 \\
3 &			 0.257087 &	 1.1638 \\
4 &			 0.11213 &	 1.19708 \\
Number of fluid steps= 5 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0712  &  \\
1 &			 0.949946 &	 0.17331 \\
2 &			 0.555675 &	 0.773604 \\
3 &			 0.24079 &	 1.20647 \\
4 &			 0.102342 &	 1.23438 \\
Number of fluid steps= 5 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07271  &  \\
1 &			 0.95523 &	 0.16734 \\
2 &			 0.56305 &	 0.762585 \\
3 &			 0.243703 &	 1.20814 \\
4 &			 0.102293 &	 1.25242 \\
Number of fluid steps= 5 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07146  &  \\
1 &			 0.953827 &	 0.167778 \\
2 &			 0.557335 &	 0.775183 \\
3 &			 0.23713 &	 1.23287 \\
4 &			 0.097206 &	 1.28656 \\
Number of fluid steps= 5 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07296  &  \\
1 &			 0.951244 &	 0.173709 \\
2 &			 0.552622 &	 0.783522 \\
3 &			 0.232373 &	 1.24985 \\
4 &			 0.0938374 &	 1.30821 \\
Number of fluid steps= 5 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07249  &  \\
1 &			 0.949995 &	 0.174972 \\
2 &			 0.548008 &	 0.793723 \\
3 &			 0.228281 &	 1.26339 \\
4 &			 0.0914663 &	 1.3195 \\
Number of fluid steps= 5 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07122  &  \\
1 &			 0.938306 &	 0.191124 \\
2 &			 0.533577 &	 0.814362 \\
3 &			 0.217592 &	 1.29407 \\
4 &			 0.0854429 &	 1.34859 \\
Number of fluid steps= 6 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0205 &	 -0.0292762 \\
2 &			 1.04525 &	 -0.0345719 \\
Number of fluid steps= 6 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02031  &  \\
1 &			 1.05256 &	 -0.0448949 \\
2 &			 1.09785 &	 -0.0607785 \\
Number of fluid steps= 6 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03601  &  \\
1 &			 1.07879 &	 -0.0583761 \\
2 &			 1.10607 &	 -0.0360286 \\
3 &			 1.14948 &	 -0.0555387 \\
4 &			 1.23161 &	 -0.0995641 \\
Number of fluid steps= 6 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05237  &  \\
1 &			 1.08074 &	 -0.0383775 \\
2 &			 1.02742 &	 0.0729934 \\
3 &			 0.97809 &	 0.0709869 \\
4 &			 0.997721 &	 -0.0286692 \\
Number of fluid steps= 6 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07728  &  \\
1 &			 1.04434 &	 0.0448018 \\
2 &			 0.855717 &	 0.287386 \\
3 &			 0.67063 &	 0.351617 \\
4 &			 0.584997 &	 0.197088 \\
Number of fluid steps= 6 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0599  &  \\
1 &			 0.936833 &	 0.178064 \\
2 &			 0.610213 &	 0.618479 \\
3 &			 0.352485 &	 0.791751 \\
4 &			 0.19803 &	 0.831843 \\
Number of fluid steps= 6 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06246  &  \\
1 &			 0.943095 &	 0.171934 \\
2 &			 0.61465 &	 0.617638 \\
3 &			 0.347383 &	 0.823238 \\
4 &			 0.190639 &	 0.865684 \\
Number of fluid steps= 6 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06001  &  \\
1 &			 0.932106 &	 0.185512 \\
2 &			 0.591838 &	 0.655292 \\
3 &			 0.32538 &	 0.863077 \\
4 &			 0.178121 &	 0.869268 \\
Number of fluid steps= 6 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05828  &  \\
1 &			 0.917873 &	 0.205355 \\
2 &			 0.566563 &	 0.696058 \\
3 &			 0.301053 &	 0.912219 \\
4 &			 0.163456 &	 0.881115 \\
Number of fluid steps= 6 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06056  &  \\
1 &			 0.9112 &	 0.218987 \\
2 &			 0.551638 &	 0.724046 \\
3 &			 0.282331 &	 0.966334 \\
4 &			 0.143288 &	 0.97847 \\
Number of fluid steps= 6 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05914  &  \\
1 &			 0.904431 &	 0.227811 \\
2 &			 0.5346 &	 0.758551 \\
3 &			 0.263789 &	 1.01908 \\
4 &			 0.129376 &	 1.02781 \\
Number of fluid steps= 6 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05435  &  \\
1 &			 0.879988 &	 0.260798 \\
2 &			 0.504881 &	 0.80154 \\
3 &			 0.239873 &	 1.07367 \\
4 &			 0.114482 &	 1.06715 \\
Number of fluid steps= 6 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05739  &  \\
1 &			 0.886937 &	 0.253604 \\
2 &			 0.512224 &	 0.792057 \\
3 &			 0.241241 &	 1.0863 \\
4 &			 0.11318 &	 1.09186 \\
Number of fluid steps= 6 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05564  &  \\
1 &			 0.882138 &	 0.259042 \\
2 &			 0.501674 &	 0.814254 \\
3 &			 0.231413 &	 1.11628 \\
4 &			 0.106829 &	 1.11517 \\
Number of fluid steps= 6 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.053  &  \\
1 &			 0.874293 &	 0.268317 \\
2 &			 0.489667 &	 0.836316 \\
3 &			 0.22065 &	 1.15004 \\
4 &			 0.100417 &	 1.13576 \\
Number of fluid steps= 6 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05497  &  \\
1 &			 0.87208 &	 0.27467 \\
2 &			 0.485333 &	 0.845486 \\
3 &			 0.215954 &	 1.16825 \\
4 &			 0.0959879 &	 1.1698 \\
Number of fluid steps= 6 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05298  &  \\
1 &			 0.869493 &	 0.276232 \\
2 &			 0.478534 &	 0.861553 \\
3 &			 0.209245 &	 1.19343 \\
4 &			 0.0913981 &	 1.19496 \\
Number of fluid steps= 6 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04895  &  \\
1 &			 0.852426 &	 0.299299 \\
2 &			 0.460449 &	 0.888533 \\
3 &			 0.196261 &	 1.23027 \\
4 &			 0.0840326 &	 1.22375 \\
Number of fluid steps= 6 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05182  &  \\
1 &			 0.858539 &	 0.292932 \\
2 &			 0.467573 &	 0.876692 \\
3 &			 0.199032 &	 1.23219 \\
4 &			 0.0843018 &	 1.23937 \\
Number of fluid steps= 6 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05054  &  \\
1 &			 0.855848 &	 0.295705 \\
2 &			 0.461185 &	 0.892009 \\
3 &			 0.193264 &	 1.25477 \\
4 &			 0.0803398 &	 1.26639 \\
Number of fluid steps= 7 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01965 &	 -0.028074 \\
2 &			 1.04234 &	 -0.0317519 \\
Number of fluid steps= 7 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01765  &  \\
1 &			 1.05003 &	 -0.0451891 \\
2 &			 1.09381 &	 -0.0589316 \\
Number of fluid steps= 7 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03735  &  \\
1 &			 1.07673 &	 -0.0537538 \\
2 &			 1.12013 &	 -0.0570097 \\
3 &			 1.18074 &	 -0.0760251 \\
Number of fluid steps= 7 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03771  &  \\
1 &			 1.0842 &	 -0.0632276 \\
2 &			 1.08217 &	 0.00270376 \\
3 &			 1.10884 &	 -0.0351241 \\
4 &			 1.17941 &	 -0.0890141 \\
Number of fluid steps= 7 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05271  &  \\
1 &			 1.05815 &	 -0.0074361 \\
2 &			 0.9621 &	 0.137285 \\
3 &			 0.893732 &	 0.106345 \\
4 &			 0.898769 &	 -0.00810808 \\
Number of fluid steps= 7 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07649  &  \\
1 &			 0.993111 &	 0.116308 \\
2 &			 0.773487 &	 0.360578 \\
3 &			 0.591086 &	 0.388009 \\
4 &			 0.509931 &	 0.213066 \\
Number of fluid steps= 7 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04279  &  \\
1 &			 0.869203 &	 0.262684 \\
2 &			 0.548601 &	 0.663936 \\
3 &			 0.314582 &	 0.802321 \\
4 &			 0.174311 &	 0.851773 \\
Number of fluid steps= 7 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04717  &  \\
1 &			 0.87676 &	 0.256242 \\
2 &			 0.553189 &	 0.66441 \\
3 &			 0.310839 &	 0.831605 \\
4 &			 0.16884 &	 0.880511 \\
Number of fluid steps= 7 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04374  &  \\
1 &			 0.869106 &	 0.264158 \\
2 &			 0.536449 &	 0.696091 \\
3 &			 0.294655 &	 0.864414 \\
4 &			 0.159632 &	 0.884277 \\
Number of fluid steps= 7 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04132  &  \\
1 &			 0.85731 &	 0.280525 \\
2 &			 0.516389 &	 0.731359 \\
3 &			 0.276037 &	 0.903597 \\
4 &			 0.14954 &	 0.88433 \\
Number of fluid steps= 7 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04072  &  \\
1 &			 0.844419 &	 0.301551 \\
2 &			 0.498466 &	 0.760464 \\
3 &			 0.257799 &	 0.951248 \\
4 &			 0.133972 &	 0.944315 \\
Number of fluid steps= 7 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03817  &  \\
1 &			 0.834026 &	 0.315878 \\
2 &			 0.482387 &	 0.789901 \\
3 &			 0.242281 &	 0.99351 \\
4 &			 0.120704 &	 1.00521 \\
Number of fluid steps= 7 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03319  &  \\
1 &			 0.824216 &	 0.326011 \\
2 &			 0.465121 &	 0.825416 \\
3 &			 0.226727 &	 1.03665 \\
4 &			 0.110134 &	 1.0417 \\
Number of fluid steps= 7 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02457  &  \\
1 &			 0.799182 &	 0.358423 \\
2 &			 0.439299 &	 0.863321 \\
3 &			 0.207542 &	 1.0818 \\
4 &			 0.0986901 &	 1.07243 \\
Number of fluid steps= 7 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02921  &  \\
1 &			 0.806631 &	 0.351557 \\
2 &			 0.44617 &	 0.854315 \\
3 &			 0.208989 &	 1.09417 \\
4 &			 0.0979118 &	 1.09387 \\
Number of fluid steps= 7 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02692  &  \\
1 &			 0.804454 &	 0.352242 \\
2 &			 0.439236 &	 0.873014 \\
3 &			 0.202332 &	 1.11827 \\
4 &			 0.0934962 &	 1.11374 \\
Number of fluid steps= 7 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02512  &  \\
1 &			 0.799361 &	 0.358874 \\
2 &			 0.430694 &	 0.892184 \\
3 &			 0.194558 &	 1.14646 \\
4 &			 0.0888379 &	 1.13095 \\
Number of fluid steps= 7 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0251  &  \\
1 &			 0.792998 &	 0.370376 \\
2 &			 0.423794 &	 0.903954 \\
3 &			 0.188397 &	 1.16959 \\
4 &			 0.0843845 &	 1.15873 \\
Number of fluid steps= 7 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0228  &  \\
1 &			 0.78797 &	 0.376311 \\
2 &			 0.417303 &	 0.917045 \\
3 &			 0.18334 &	 1.18657 \\
4 &			 0.0809267 &	 1.17983 \\
Number of fluid steps= 7 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01881  &  \\
1 &			 0.783267 &	 0.379309 \\
2 &			 0.409321 &	 0.936271 \\
3 &			 0.177077 &	 1.20886 \\
4 &			 0.077155 &	 1.19855 \\
Number of fluid steps= 8 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01887 &	 -0.02697 \\
2 &			 1.03984 &	 -0.0293916 \\
Number of fluid steps= 8 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01878  &  \\
1 &			 1.04724 &	 -0.0397496 \\
2 &			 1.08842 &	 -0.0556433 \\
Number of fluid steps= 8 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0269  &  \\
1 &			 1.07348 &	 -0.0639996 \\
2 &			 1.12402 &	 -0.0663724 \\
Number of fluid steps= 8 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04524  &  \\
1 &			 1.08116 &	 -0.0487458 \\
2 &			 1.11035 &	 -0.0384345 \\
3 &			 1.177 &	 -0.0840998 \\
4 &			 1.26551 &	 -0.104605 \\
Number of fluid steps= 8 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05521  &  \\
1 &			 1.06809 &	 -0.0175031 \\
2 &			 1.03722 &	 0.0423113 \\
3 &			 1.04772 &	 -0.0145313 \\
4 &			 1.10469 &	 -0.0763884 \\
Number of fluid steps= 8 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05713  &  \\
1 &			 1.01612 &	 0.057082 \\
2 &			 0.891119 &	 0.189381 \\
3 &			 0.812554 &	 0.133154 \\
4 &			 0.809252 &	 0.00587467 \\
Number of fluid steps= 8 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06373  &  \\
1 &			 0.93844 &	 0.180796 \\
2 &			 0.704147 &	 0.414388 \\
3 &			 0.527677 &	 0.416222 \\
4 &			 0.451291 &	 0.225597 \\
Number of fluid steps= 8 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01772  &  \\
1 &			 0.809936 &	 0.329461 \\
2 &			 0.501699 &	 0.690986 \\
3 &			 0.285094 &	 0.815384 \\
4 &			 0.15578 &	 0.871928 \\
Number of fluid steps= 8 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0239  &  \\
1 &			 0.818104 &	 0.323719 \\
2 &			 0.506067 &	 0.692956 \\
3 &			 0.282242 &	 0.842396 \\
4 &			 0.151569 &	 0.896958 \\
Number of fluid steps= 8 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01895  &  \\
1 &			 0.80946 &	 0.332052 \\
2 &			 0.490888 &	 0.721566 \\
3 &			 0.269204 &	 0.866694 \\
4 &			 0.144672 &	 0.895914 \\
Number of fluid steps= 8 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01754  &  \\
1 &			 0.799794 &	 0.347385 \\
2 &			 0.475459 &	 0.750308 \\
3 &			 0.255081 &	 0.898365 \\
4 &			 0.138291 &	 0.883248 \\
Number of fluid steps= 8 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01028  &  \\
1 &			 0.782251 &	 0.369052 \\
2 &			 0.454001 &	 0.784936 \\
3 &			 0.238968 &	 0.925878 \\
4 &			 0.131515 &	 0.86159 \\
Number of fluid steps= 8 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00902  &  \\
1 &			 0.776755 &	 0.377423 \\
2 &			 0.443231 &	 0.809401 \\
3 &			 0.224949 &	 0.978461 \\
4 &			 0.113794 &	 0.983173 \\
Number of fluid steps= 8 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00388  &  \\
1 &			 0.763551 &	 0.39479 \\
2 &			 0.427351 &	 0.837303 \\
3 &			 0.211638 &	 1.01382 \\
4 &			 0.103972 &	 1.0254 \\
Number of fluid steps= 8 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.998593  &  \\
1 &			 0.755253 &	 0.402937 \\
2 &			 0.413551 &	 0.868895 \\
3 &			 0.199521 &	 1.05152 \\
4 &			 0.0958871 &	 1.05713 \\
Number of fluid steps= 8 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.987522  &  \\
1 &			 0.731477 &	 0.433 \\
2 &			 0.391347 &	 0.902364 \\
3 &			 0.183871 &	 1.08975 \\
4 &			 0.0868258 &	 1.0825 \\
Number of fluid steps= 8 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.993457  &  \\
1 &			 0.738946 &	 0.426989 \\
2 &			 0.39762 &	 0.894079 \\
3 &			 0.185292 &	 1.10159 \\
4 &			 0.0863575 &	 1.10141 \\
Number of fluid steps= 8 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.990056  &  \\
1 &			 0.735552 &	 0.428683 \\
2 &			 0.390743 &	 0.912607 \\
3 &			 0.179697 &	 1.12065 \\
4 &			 0.0829082 &	 1.11598 \\
Number of fluid steps= 8 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.99006  &  \\
1 &			 0.732067 &	 0.43554 \\
2 &			 0.384982 &	 0.927185 \\
3 &			 0.174051 &	 1.14528 \\
4 &			 0.0795047 &	 1.1304 \\
Number of fluid steps= 8 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.985187  &  \\
1 &			 0.722586 &	 0.447228 \\
2 &			 0.374185 &	 0.949418 \\
3 &			 0.166389 &	 1.16919 \\
4 &			 0.0760942 &	 1.1287 \\
Number of fluid steps= 9 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01814 &	 -0.025936 \\
2 &			 1.03756 &	 -0.0272588 \\
Number of fluid steps= 9 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01704  &  \\
1 &			 1.04519 &	 -0.0393888 \\
2 &			 1.32409 &	 -0.341236 \\
Number of fluid steps= 9 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03108  &  \\
1 &			 1.06959 &	 -0.0529016 \\
2 &			 1.12214 &	 -0.0691948 \\
Number of fluid steps= 9 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04951  &  \\
1 &			 1.08339 &	 -0.0458368 \\
2 &			 1.13211 &	 -0.0634615 \\
3 &			 1.94209 &	 -0.778596 \\
Number of fluid steps= 9 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04145  &  \\
1 &			 1.07542 &	 -0.0463066 \\
2 &			 1.08836 &	 -0.0172556 \\
3 &			 1.14597 &	 -0.0744134 \\
4 &			 1.22691 &	 -0.0984601 \\
Number of fluid steps= 9 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0521  &  \\
1 &			 1.03536 &	 0.0231393 \\
2 &			 0.981247 &	 0.0774442 \\
3 &			 0.97915 &	 0.00308645 \\
4 &			 1.02478 &	 -0.0657124 \\
Number of fluid steps= 9 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0431  &  \\
1 &			 0.974984 &	 0.097427 \\
2 &			 0.830433 &	 0.231515 \\
3 &			 0.745298 &	 0.156046 \\
4 &			 0.735287 &	 0.0195099 \\
Number of fluid steps= 9 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04248  &  \\
1 &			 0.886163 &	 0.234376 \\
2 &			 0.64617 &	 0.455658 \\
3 &			 0.476324 &	 0.439971 \\
4 &			 0.40443 &	 0.236053 \\
Number of fluid steps= 9 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988738  &  \\
1 &			 0.760213 &	 0.379185 \\
2 &			 0.464844 &	 0.709657 \\
3 &			 0.261343 &	 0.830802 \\
4 &			 0.140871 &	 0.89157 \\
Number of fluid steps= 9 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.996409  &  \\
1 &			 0.768494 &	 0.374704 \\
2 &			 0.468876 &	 0.712828 \\
3 &			 0.259112 &	 0.855631 \\
4 &			 0.137533 &	 0.913798 \\
Number of fluid steps= 9 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.991487  &  \\
1 &			 0.762557 &	 0.378749 \\
2 &			 0.457204 &	 0.738007 \\
3 &			 0.248886 &	 0.877353 \\
4 &			 0.131965 &	 0.91533 \\
Number of fluid steps= 9 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98659  &  \\
1 &			 0.749421 &	 0.396674 \\
2 &			 0.441076 &	 0.764749 \\
3 &			 0.237173 &	 0.895087 \\
4 &			 0.129151 &	 0.876881 \\
Number of fluid steps= 9 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98338  &  \\
1 &			 0.741018 &	 0.40824 \\
2 &			 0.427115 &	 0.794884 \\
3 &			 0.224538 &	 0.927665 \\
4 &			 0.122399 &	 0.875368 \\
Number of fluid steps= 9 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98049  &  \\
1 &			 0.729277 &	 0.427036 \\
2 &			 0.413536 &	 0.818454 \\
3 &			 0.211498 &	 0.967369 \\
4 &			 0.11066 &	 0.93451 \\
Number of fluid steps= 9 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.971526  &  \\
1 &			 0.716279 &	 0.439731 \\
2 &			 0.398958 &	 0.844285 \\
3 &			 0.199503 &	 0.999826 \\
4 &			 0.0990307 &	 1.01046 \\
Number of fluid steps= 9 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.969115  &  \\
1 &			 0.70819 &	 0.452531 \\
2 &			 0.387807 &	 0.868798 \\
3 &			 0.189252 &	 1.03503 \\
4 &			 0.0915005 &	 1.04846 \\
Number of fluid steps= 9 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.96114  &  \\
1 &			 0.698301 &	 0.460898 \\
2 &			 0.374302 &	 0.899646 \\
3 &			 0.178719 &	 1.06651 \\
4 &			 0.0849134 &	 1.07363 \\
Number of fluid steps= 9 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.94899  &  \\
1 &			 0.676658 &	 0.487966 \\
2 &			 0.355242 &	 0.929625 \\
3 &			 0.165752 &	 1.09978 \\
4 &			 0.0775627 &	 1.09559 \\
Number of fluid steps= 9 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.955776  &  \\
1 &			 0.683869 &	 0.482953 \\
2 &			 0.360918 &	 0.922049 \\
3 &			 0.167108 &	 1.11089 \\
4 &			 0.077289 &	 1.11245 \\
Number of fluid steps= 9 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.952715  &  \\
1 &			 0.682102 &	 0.482057 \\
2 &			 0.356073 &	 0.937814 \\
3 &			 0.16303 &	 1.12704 \\
4 &			 0.074695 &	 1.12605 \\
Number of fluid steps= 10 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01747 &	 -0.0249863 \\
2 &			 1.03448 &	 -0.0239195 \\
Number of fluid steps= 10 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01747  &  \\
1 &			 1.04299 &	 -0.0357391 \\
Number of fluid steps= 10 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03229  &  \\
1 &			 1.06745 &	 -0.0483202 \\
Number of fluid steps= 10 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04127  &  \\
1 &			 1.08176 &	 -0.0550363 \\
2 &			 1.14185 &	 -0.0779927 \\
Number of fluid steps= 10 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04718  &  \\
1 &			 1.07637 &	 -0.0396646 \\
2 &			 1.11834 &	 -0.0551848 \\
3 &			 1.20162 &	 -0.103622 \\
4 &			 1.2899 &	 -0.102278 \\
Number of fluid steps= 10 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05023  &  \\
1 &			 1.05285 &	 -0.0035946 \\
2 &			 1.05043 &	 0.00331988 \\
3 &			 1.09813 &	 -0.0640688 \\
4 &			 1.16997 &	 -0.0914227 \\
Number of fluid steps= 10 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03856  &  \\
1 &			 1.00426 &	 0.0484517 \\
2 &			 0.931997 &	 0.107736 \\
3 &			 0.918279 &	 0.0213928 \\
4 &			 0.952381 &	 -0.0526063 \\
Number of fluid steps= 10 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02922  &  \\
1 &			 0.927246 &	 0.150527 \\
2 &			 0.77149 &	 0.265305 \\
3 &			 0.683711 &	 0.174261 \\
4 &			 0.670378 &	 0.0284118 \\
Number of fluid steps= 10 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01647  &  \\
1 &			 0.838747 &	 0.27726 \\
2 &			 0.597536 &	 0.48921 \\
3 &			 0.434059 &	 0.461134 \\
4 &			 0.36622 &	 0.245181 \\
Number of fluid steps= 10 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.959089  &  \\
1 &			 0.719217 &	 0.415238 \\
2 &			 0.435036 &	 0.725292 \\
3 &			 0.241714 &	 0.847834 \\
4 &			 0.128601 &	 0.910399 \\
Number of fluid steps= 10 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.967829  &  \\
1 &			 0.727302 &	 0.412198 \\
2 &			 0.438723 &	 0.729244 \\
3 &			 0.239936 &	 0.870661 \\
4 &			 0.125891 &	 0.930474 \\
Number of fluid steps= 10 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.961614  &  \\
1 &			 0.720729 &	 0.416001 \\
2 &			 0.427986 &	 0.751893 \\
3 &			 0.231341 &	 0.887543 \\
4 &			 0.12139 &	 0.930371 \\
Number of fluid steps= 10 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.959136  &  \\
1 &			 0.713101 &	 0.427629 \\
2 &			 0.416416 &	 0.776081 \\
3 &			 0.222066 &	 0.907037 \\
4 &			 0.118842 &	 0.901944 \\
Number of fluid steps= 10 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.954215  &  \\
1 &			 0.701572 &	 0.443723 \\
2 &			 0.402736 &	 0.800757 \\
3 &			 0.211865 &	 0.926689 \\
4 &			 0.115411 &	 0.876365 \\
Number of fluid steps= 10 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.94638  &  \\
1 &			 0.687342 &	 0.461391 \\
2 &			 0.387244 &	 0.827785 \\
3 &			 0.201331 &	 0.943674 \\
4 &			 0.112633 &	 0.83794 \\
Number of fluid steps= 10 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.942618  &  \\
1 &			 0.680601 &	 0.469864 \\
2 &			 0.377357 &	 0.850879 \\
3 &			 0.189333 &	 0.995004 \\
4 &			 0.0960739 &	 0.978709 \\
Number of fluid steps= 10 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.939048  &  \\
1 &			 0.671703 &	 0.483375 \\
2 &			 0.367244 &	 0.871085 \\
3 &			 0.180258 &	 1.02668 \\
4 &			 0.0876815 &	 1.03972 \\
Number of fluid steps= 10 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.931372  &  \\
1 &			 0.660522 &	 0.495751 \\
2 &			 0.354811 &	 0.896556 \\
3 &			 0.170893 &	 1.05396 \\
4 &			 0.0815292 &	 1.0677 \\
Number of fluid steps= 10 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.924888  &  \\
1 &			 0.652048 &	 0.504301 \\
2 &			 0.343674 &	 0.923937 \\
3 &			 0.162299 &	 1.08239 \\
4 &			 0.0762001 &	 1.09079 \\
Number of fluid steps= 10 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.912745  &  \\
1 &			 0.632842 &	 0.528367 \\
2 &			 0.327276 &	 0.951338 \\
3 &			 0.151401 &	 1.11213 \\
4 &			 0.0701174 &	 1.11053 \\
Number of fluid steps= 11 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01685 &	 -0.0241069 \\
2 &			 1.02658 &	 -0.0137392 \\
Number of fluid steps= 11 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01621  &  \\
1 &			 1.0413 &	 -0.0351872 \\
2 &			 76.7888 &	 -6.20444 \\
Number of fluid steps= 11 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02494  &  \\
1 &			 1.06492 &	 -0.0552056 \\
Number of fluid steps= 11 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03319  &  \\
1 &			 1.0812 &	 -0.0655278 \\
2 &			 3.3849 &	 -1.64648 \\
Number of fluid steps= 11 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05309  &  \\
1 &			 1.08309 &	 -0.0405244 \\
2 &			 1.14307 &	 -0.0777606 \\
3 &			 1.22156 &	 -0.095811 \\
Number of fluid steps= 11 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03854  &  \\
1 &			 1.06639 &	 -0.0381784 \\
2 &			 1.09936 &	 -0.0439287 \\
3 &			 1.1766 &	 -0.09796 \\
4 &			 1.25956 &	 -0.0982959 \\
Number of fluid steps= 11 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04471  &  \\
1 &			 1.0272 &	 0.0243854 \\
2 &			 1.0103 &	 0.0239334 \\
3 &			 1.04711 &	 -0.0516293 \\
4 &			 1.10858 &	 -0.0822999 \\
Number of fluid steps= 11 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02954  &  \\
1 &			 0.966671 &	 0.090903 \\
2 &			 0.880921 &	 0.134012 \\
3 &			 0.858817 &	 0.0366619 \\
4 &			 0.884628 &	 -0.0427202 \\
Number of fluid steps= 11 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00681  &  \\
1 &			 0.887464 &	 0.182031 \\
2 &			 0.723113 &	 0.295467 \\
3 &			 0.633216 &	 0.191523 \\
4 &			 0.616715 &	 0.0380938 \\
Number of fluid steps= 11 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988727  &  \\
1 &			 0.796843 &	 0.311277 \\
2 &			 0.556423 &	 0.518113 \\
3 &			 0.398747 &	 0.480708 \\
4 &			 0.334514 &	 0.253407 \\
Number of fluid steps= 11 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.930938  &  \\
1 &			 0.685526 &	 0.441474 \\
2 &			 0.410332 &	 0.74042 \\
3 &			 0.225169 &	 0.865783 \\
4 &			 0.118317 &	 0.928351 \\
Number of fluid steps= 11 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.940298  &  \\
1 &			 0.693247 &	 0.439749 \\
2 &			 0.413706 &	 0.744764 \\
3 &			 0.223735 &	 0.886815 \\
4 &			 0.116077 &	 0.946709 \\
Number of fluid steps= 11 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.934987  &  \\
1 &			 0.688349 &	 0.441806 \\
2 &			 0.405053 &	 0.76503 \\
3 &			 0.216679 &	 0.902551 \\
4 &			 0.112278 &	 0.948484 \\
Number of fluid steps= 11 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.932972  &  \\
1 &			 0.680535 &	 0.455164 \\
2 &			 0.394796 &	 0.785562 \\
3 &			 0.208923 &	 0.918136 \\
4 &			 0.110353 &	 0.920845 \\
Number of fluid steps= 11 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.929097  &  \\
1 &			 0.671495 &	 0.468453 \\
2 &			 0.383514 &	 0.808097 \\
3 &			 0.200796 &	 0.933549 \\
4 &			 0.109152 &	 0.879392 \\
Number of fluid steps= 11 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.922041  &  \\
1 &			 0.661257 &	 0.47962 \\
2 &			 0.370704 &	 0.834943 \\
3 &			 0.19149 &	 0.952999 \\
4 &			 0.10577 &	 0.856339 \\
Number of fluid steps= 11 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.918788  &  \\
1 &			 0.651984 &	 0.494895 \\
2 &			 0.360373 &	 0.855346 \\
3 &			 0.181609 &	 0.988655 \\
4 &			 0.0962007 &	 0.916716 \\
Number of fluid steps= 11 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.91093  &  \\
1 &			 0.642447 &	 0.503763 \\
2 &			 0.349654 &	 0.877649 \\
3 &			 0.172072 &	 1.02292 \\
4 &			 0.0848686 &	 1.01971 \\
Number of fluid steps= 11 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905112  &  \\
1 &			 0.633218 &	 0.515394 \\
2 &			 0.339808 &	 0.897982 \\
3 &			 0.164144 &	 1.04976 \\
4 &			 0.0785654 &	 1.063 \\
Number of fluid steps= 11 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.900334  &  \\
1 &			 0.623821 &	 0.529328 \\
2 &			 0.329904 &	 0.919086 \\
3 &			 0.156614 &	 1.07483 \\
4 &			 0.0736241 &	 1.08896 \\
Number of fluid steps= 12 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01626 &	 -0.0232695 \\
2 &			 1.01081 &	 0.00775771 \\
Number of fluid steps= 12 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01633  &  \\
1 &			 1.03951 &	 -0.0325347 \\
Number of fluid steps= 12 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02725  &  \\
1 &			 1.06208 &	 -0.0481051 \\
Number of fluid steps= 12 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0367  &  \\
1 &			 1.07847 &	 -0.0569876 \\
Number of fluid steps= 12 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04126  &  \\
1 &			 1.08518 &	 -0.059604 \\
2 &			 1.15056 &	 -0.0844019 \\
Number of fluid steps= 12 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04295  &  \\
1 &			 1.07052 &	 -0.0376418 \\
2 &			 1.12848 &	 -0.0760691 \\
3 &			 1.2225 &	 -0.115454 \\
4 &			 1.30809 &	 -0.0976273 \\
Number of fluid steps= 12 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04042  &  \\
1 &			 1.04522 &	 -0.0066406 \\
2 &			 1.06902 &	 -0.0324822 \\
3 &			 1.13895 &	 -0.0914156 \\
4 &			 1.21509 &	 -0.0933588 \\
Number of fluid steps= 12 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02666  &  \\
1 &			 0.991724 &	 0.0499479 \\
2 &			 0.963195 &	 0.0421108 \\
3 &			 0.991558 &	 -0.0418693 \\
4 &			 1.04506 &	 -0.0758167 \\
Number of fluid steps= 12 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00886  &  \\
1 &			 0.925521 &	 0.124388 \\
2 &			 0.830125 &	 0.156937 \\
3 &			 0.802394 &	 0.0490178 \\
4 &			 0.822533 &	 -0.0357627 \\
Number of fluid steps= 12 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.985703  &  \\
1 &			 0.845729 &	 0.220958 \\
2 &			 0.676972 &	 0.321099 \\
3 &			 0.586915 &	 0.205945 \\
4 &			 0.569162 &	 0.0443122 \\
Number of fluid steps= 12 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.961361  &  \\
1 &			 0.760243 &	 0.338618 \\
2 &			 0.521347 &	 0.544217 \\
3 &			 0.368847 &	 0.499221 \\
4 &			 0.30781 &	 0.260982 \\
Number of fluid steps= 12 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905489  &  \\
1 &			 0.657705 &	 0.461256 \\
2 &			 0.389443 &	 0.756028 \\
3 &			 0.211005 &	 0.884135 \\
4 &			 0.109568 &	 0.945451 \\
Number of fluid steps= 12 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.915061  &  \\
1 &			 0.664989 &	 0.460537 \\
2 &			 0.392544 &	 0.760476 \\
3 &			 0.209838 &	 0.903578 \\
4 &			 0.107687 &	 0.962432 \\
Number of fluid steps= 12 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.908666  &  \\
1 &			 0.659611 &	 0.462135 \\
2 &			 0.384459 &	 0.778786 \\
3 &			 0.203719 &	 0.916249 \\
4 &			 0.104493 &	 0.963174 \\
Number of fluid steps= 12 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905614  &  \\
1 &			 0.652037 &	 0.473942 \\
2 &			 0.375181 &	 0.797367 \\
3 &			 0.197168 &	 0.928161 \\
4 &			 0.103143 &	 0.93478 \\
Number of fluid steps= 12 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.901228  &  \\
1 &			 0.643375 &	 0.486232 \\
2 &			 0.364999 &	 0.817767 \\
3 &			 0.190855 &	 0.935416 \\
4 &			 0.10432 &	 0.871461 \\
Number of fluid steps= 12 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.899464  &  \\
1 &			 0.636632 &	 0.498606 \\
2 &			 0.355608 &	 0.840172 \\
3 &			 0.183002 &	 0.958428 \\
4 &			 0.100673 &	 0.862183 \\
Number of fluid steps= 12 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.890098  &  \\
1 &			 0.624113 &	 0.512157 \\
2 &			 0.343243 &	 0.862577 \\
3 &			 0.175868 &	 0.964737 \\
4 &			 0.100378 &	 0.80905 \\
Number of fluid steps= 12 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.887852  &  \\
1 &			 0.618843 &	 0.520746 \\
2 &			 0.335395 &	 0.883712 \\
3 &			 0.165428 &	 1.01966 \\
4 &			 0.0844785 &	 0.969547 \\
Number of fluid steps= 12 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.87936  &  \\
1 &			 0.608048 &	 0.532269 \\
2 &			 0.325365 &	 0.902126 \\
3 &			 0.157657 &	 1.04527 \\
4 &			 0.0762797 &	 1.04742 \\
Number of fluid steps= 13 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0157 &	 -0.0224743 \\
2 &			 1.0992 &	 -0.11398 \\
Number of fluid steps= 13 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01537  &  \\
1 &			 1.03808 &	 -0.0319121 \\
Number of fluid steps= 13 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02817  &  \\
1 &			 1.0601 &	 -0.0441215 \\
Number of fluid steps= 13 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03937  &  \\
1 &			 1.07767 &	 -0.0522061 \\
2 &			 156457 &	 -17.1475 \\
Number of fluid steps= 13 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04221  &  \\
1 &			 1.08601 &	 -0.0593914 \\
2 &			 9.76022 &	 -3.16788 \\
Number of fluid steps= 13 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05009  &  \\
1 &			 1.08063 &	 -0.0413597 \\
2 &			 1.15369 &	 -0.094383 \\
3 &			 4.21531 &	 -1.86938 \\
Number of fluid steps= 13 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03143  &  \\
1 &			 1.05948 &	 -0.0387104 \\
2 &			 1.11206 &	 -0.0698783 \\
3 &			 1.20156 &	 -0.111674 \\
4 &			 1.28325 &	 -0.0948936 \\
Number of fluid steps= 13 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02692  &  \\
1 &			 1.02022 &	 0.00944351 \\
2 &			 1.03455 &	 -0.0201231 \\
3 &			 1.09621 &	 -0.0835208 \\
4 &			 1.16471 &	 -0.0874466 \\
Number of fluid steps= 13 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00882  &  \\
1 &			 0.964166 &	 0.0653153 \\
2 &			 0.924486 &	 0.0606301 \\
3 &			 0.943134 &	 -0.0288113 \\
4 &			 0.987477 &	 -0.0662844 \\
Number of fluid steps= 13 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988269  &  \\
1 &			 0.893477 &	 0.145473 \\
2 &			 0.789133 &	 0.179162 \\
3 &			 0.755422 &	 0.0629857 \\
4 &			 0.769488 &	 -0.026616 \\
Number of fluid steps= 13 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.962504  &  \\
1 &			 0.812372 &	 0.244652 \\
2 &			 0.63917 &	 0.345941 \\
3 &			 0.548593 &	 0.220463 \\
4 &			 0.529267 &	 0.0517405 \\
Number of fluid steps= 13 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.935677  &  \\
1 &			 0.728404 &	 0.361272 \\
2 &			 0.491142 &	 0.568599 \\
3 &			 0.343228 &	 0.516973 \\
4 &			 0.285023 &	 0.268089 \\
Number of fluid steps= 13 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.883247  &  \\
1 &			 0.634523 &	 0.477144 \\
2 &			 0.371483 &	 0.772376 \\
3 &			 0.198724 &	 0.90253 \\
4 &			 0.102032 &	 0.961744 \\
Number of fluid steps= 13 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.892698  &  \\
1 &			 0.641355 &	 0.477049 \\
2 &			 0.374353 &	 0.776724 \\
3 &			 0.197769 &	 0.920583 \\
4 &			 0.100433 &	 0.977583 \\
Number of fluid steps= 13 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.88769  &  \\
1 &			 0.636962 &	 0.478849 \\
2 &			 0.367596 &	 0.793086 \\
3 &			 0.192581 &	 0.932656 \\
4 &			 0.0976608 &	 0.979614 \\
Number of fluid steps= 13 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.885135  &  \\
1 &			 0.630871 &	 0.488552 \\
2 &			 0.359692 &	 0.810583 \\
3 &			 0.18688 &	 0.94465 \\
4 &			 0.0962398 &	 0.957407 \\
Number of fluid steps= 13 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.881561  &  \\
1 &			 0.62366 &	 0.499301 \\
2 &			 0.350873 &	 0.829811 \\
3 &			 0.181309 &	 0.952498 \\
4 &			 0.0971324 &	 0.900426 \\
Number of fluid steps= 13 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.877876  &  \\
1 &			 0.616054 &	 0.51096 \\
2 &			 0.341971 &	 0.849183 \\
3 &			 0.175172 &	 0.965102 \\
4 &			 0.0962421 &	 0.864032 \\
Number of fluid steps= 13 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.872218  &  \\
1 &			 0.607077 &	 0.522809 \\
2 &			 0.331847 &	 0.871361 \\
3 &			 0.168436 &	 0.978318 \\
4 &			 0.094789 &	 0.829409 \\
Number of fluid steps= 13 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.86958  &  \\
1 &			 0.600155 &	 0.534984 \\
2 &			 0.323861 &	 0.88996 \\
3 &			 0.1606 &	 1.0119 \\
4 &			 0.0866142 &	 0.890796 \\
Number of fluid steps= 14 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01516 &	 -0.0217071 \\
2 &			 2.0784 &	 -1.03377 \\
Number of fluid steps= 14 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01534  &  \\
1 &			 1.03659 &	 -0.0298825 \\
Number of fluid steps= 14 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02277  &  \\
1 &			 1.05832 &	 -0.0492942 \\
Number of fluid steps= 14 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03398  &  \\
1 &			 1.07563 &	 -0.0569736 \\
Number of fluid steps= 14 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03433  &  \\
1 &			 1.08636 &	 -0.0708057 \\
Number of fluid steps= 14 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04135  &  \\
1 &			 1.08448 &	 -0.0585484 \\
2 &			 1.16076 &	 -0.0980663 \\
Number of fluid steps= 14 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03514  &  \\
1 &			 1.06575 &	 -0.0420432 \\
2 &			 1.13934 &	 -0.0963293 \\
3 &			 1.24001 &	 -0.122153 \\
4 &			 1.32212 &	 -0.0925014 \\
Number of fluid steps= 14 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02895  &  \\
1 &			 1.03801 &	 -0.0126475 \\
2 &			 1.08534 &	 -0.0643267 \\
3 &			 1.16976 &	 -0.108066 \\
4 &			 1.24671 &	 -0.0919134 \\
Number of fluid steps= 14 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01724  &  \\
1 &			 0.992953 &	 0.0348628 \\
2 &			 0.998329 &	 -0.0077899 \\
3 &			 1.05167 &	 -0.0750948 \\
4 &			 1.11263 &	 -0.0812918 \\
Number of fluid steps= 14 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.994591  &  \\
1 &			 0.930527 &	 0.0960554 \\
2 &			 0.882343 &	 0.0767084 \\
3 &			 0.893959 &	 -0.0188691 \\
4 &			 0.931804 &	 -0.0598179 \\
Number of fluid steps= 14 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.970229  &  \\
1 &			 0.86009 &	 0.173838 \\
2 &			 0.748917 &	 0.199682 \\
3 &			 0.711153 &	 0.0746459 \\
4 &			 0.721084 &	 -0.0200074 \\
Number of fluid steps= 14 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.941464  &  \\
1 &			 0.778391 &	 0.274411 \\
2 &			 0.603033 &	 0.368258 \\
3 &			 0.513078 &	 0.233059 \\
4 &			 0.493381 &	 0.056476 \\
Number of fluid steps= 14 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.91236  &  \\
1 &			 0.700693 &	 0.380821 \\
2 &			 0.4649 &	 0.591862 \\
3 &			 0.321047 &	 0.534136 \\
4 &			 0.265361 &	 0.274828 \\
Number of fluid steps= 14 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.864263  &  \\
1 &			 0.614989 &	 0.49091 \\
2 &			 0.355832 &	 0.789364 \\
3 &			 0.187963 &	 0.920748 \\
4 &			 0.0954705 &	 0.977322 \\
Number of fluid steps= 14 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.873342  &  \\
1 &			 0.621385 &	 0.491059 \\
2 &			 0.358507 &	 0.793486 \\
3 &			 0.187179 &	 0.937583 \\
4 &			 0.0940963 &	 0.992209 \\
Number of fluid steps= 14 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.867408  &  \\
1 &			 0.616659 &	 0.492238 \\
2 &			 0.35212 &	 0.808406 \\
3 &			 0.182575 &	 0.947578 \\
4 &			 0.0917029 &	 0.99345 \\
Number of fluid steps= 14 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.867234  &  \\
1 &			 0.611876 &	 0.503182 \\
2 &			 0.345718 &	 0.823644 \\
3 &			 0.177768 &	 0.9596 \\
4 &			 0.090404 &	 0.975537 \\
Number of fluid steps= 14 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.862673  &  \\
1 &			 0.605135 &	 0.511557 \\
2 &			 0.337761 &	 0.841254 \\
3 &			 0.173006 &	 0.965181 \\
4 &			 0.0914484 &	 0.919792 \\
Number of fluid steps= 14 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.861162  &  \\
1 &			 0.599081 &	 0.523534 \\
2 &			 0.330282 &	 0.859053 \\
3 &			 0.16822 &	 0.973349 \\
4 &			 0.0924786 &	 0.863158 \\
Number of fluid steps= 14 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.854726  &  \\
1 &			 0.590573 &	 0.533347 \\
2 &			 0.321171 &	 0.878774 \\
3 &			 0.162322 &	 0.984483 \\
4 &			 0.091044 &	 0.834223 \\
Number of fluid steps= 15 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01463 &	 -0.0209537 \\
Number of fluid steps= 15 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01456  &  \\
1 &			 1.03537 &	 -0.0292922 \\
Number of fluid steps= 15 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0242  &  \\
1 &			 1.05591 &	 -0.0439894 \\
Number of fluid steps= 15 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02883  &  \\
1 &			 1.07421 &	 -0.0622714 \\
Number of fluid steps= 15 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0371  &  \\
1 &			 1.08472 &	 -0.0647677 \\
Number of fluid steps= 15 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03915  &  \\
1 &			 1.08717 &	 -0.0651736 \\
2 &			 943.971 &	 -9.76202 \\
Number of fluid steps= 15 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04326  &  \\
1 &			 1.07811 &	 -0.0474056 \\
2 &			 1.16385 &	 -0.110401 \\
3 &			 1.31889 &	 -0.180419 \\
Number of fluid steps= 15 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02251  &  \\
1 &			 1.05492 &	 -0.0450186 \\
2 &			 1.12492 &	 -0.0926888 \\
3 &			 1.22203 &	 -0.119457 \\
4 &			 1.30117 &	 -0.0905298 \\
Number of fluid steps= 15 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01512  &  \\
1 &			 1.01447 &	 0.00092408 \\
2 &			 1.05521 &	 -0.0568039 \\
3 &			 1.13329 &	 -0.102987 \\
4 &			 1.20458 &	 -0.0880131 \\
Number of fluid steps= 15 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.995738  &  \\
1 &			 0.960593 &	 0.0518409 \\
2 &			 0.958117 &	 0.00372345 \\
3 &			 1.00483 &	 -0.0686777 \\
Number of fluid steps= 15 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv


==> convRate/convRate_F10_S1 <==
Number of fluid steps= 10 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01747 &	 -0.0249863 \\
2 &			 1.03448 &	 -0.0239195 \\


==> convRate/convRate_F10_S10 <==
Number of fluid steps= 10 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.959089  &  \\
1 &			 0.719217 &	 0.415238 \\
2 &			 0.435036 &	 0.725292 \\
3 &			 0.241714 &	 0.847834 \\
4 &			 0.128601 &	 0.910399 \\


==> convRate/convRate_F10_S11 <==
Number of fluid steps= 10 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.967829  &  \\
1 &			 0.727302 &	 0.412198 \\
2 &			 0.438723 &	 0.729244 \\
3 &			 0.239936 &	 0.870661 \\
4 &			 0.125891 &	 0.930474 \\


==> convRate/convRate_F10_S12 <==
Number of fluid steps= 10 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.961614  &  \\
1 &			 0.720729 &	 0.416001 \\
2 &			 0.427986 &	 0.751893 \\
3 &			 0.231341 &	 0.887543 \\
4 &			 0.12139 &	 0.930371 \\


==> convRate/convRate_F10_S13 <==
Number of fluid steps= 10 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.959136  &  \\
1 &			 0.713101 &	 0.427629 \\
2 &			 0.416416 &	 0.776081 \\
3 &			 0.222066 &	 0.907037 \\
4 &			 0.118842 &	 0.901944 \\


==> convRate/convRate_F10_S14 <==
Number of fluid steps= 10 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.954215  &  \\
1 &			 0.701572 &	 0.443723 \\
2 &			 0.402736 &	 0.800757 \\
3 &			 0.211865 &	 0.926689 \\
4 &			 0.115411 &	 0.876365 \\


==> convRate/convRate_F10_S15 <==
Number of fluid steps= 10 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.94638  &  \\
1 &			 0.687342 &	 0.461391 \\
2 &			 0.387244 &	 0.827785 \\
3 &			 0.201331 &	 0.943674 \\
4 &			 0.112633 &	 0.83794 \\


==> convRate/convRate_F10_S16 <==
Number of fluid steps= 10 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.942618  &  \\
1 &			 0.680601 &	 0.469864 \\
2 &			 0.377357 &	 0.850879 \\
3 &			 0.189333 &	 0.995004 \\
4 &			 0.0960739 &	 0.978709 \\


==> convRate/convRate_F10_S17 <==
Number of fluid steps= 10 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.939048  &  \\
1 &			 0.671703 &	 0.483375 \\
2 &			 0.367244 &	 0.871085 \\
3 &			 0.180258 &	 1.02668 \\
4 &			 0.0876815 &	 1.03972 \\


==> convRate/convRate_F10_S18 <==
Number of fluid steps= 10 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.931372  &  \\
1 &			 0.660522 &	 0.495751 \\
2 &			 0.354811 &	 0.896556 \\
3 &			 0.170893 &	 1.05396 \\
4 &			 0.0815292 &	 1.0677 \\


==> convRate/convRate_F10_S19 <==
Number of fluid steps= 10 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.924888  &  \\
1 &			 0.652048 &	 0.504301 \\
2 &			 0.343674 &	 0.923937 \\
3 &			 0.162299 &	 1.08239 \\
4 &			 0.0762001 &	 1.09079 \\


==> convRate/convRate_F10_S2 <==
Number of fluid steps= 10 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01747  &  \\
1 &			 1.04299 &	 -0.0357391 \\


==> convRate/convRate_F10_S20 <==
Number of fluid steps= 10 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.912745  &  \\
1 &			 0.632842 &	 0.528367 \\
2 &			 0.327276 &	 0.951338 \\
3 &			 0.151401 &	 1.11213 \\
4 &			 0.0701174 &	 1.11053 \\


==> convRate/convRate_F10_S3 <==
Number of fluid steps= 10 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03229  &  \\
1 &			 1.06745 &	 -0.0483202 \\


==> convRate/convRate_F10_S4 <==
Number of fluid steps= 10 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04127  &  \\
1 &			 1.08176 &	 -0.0550363 \\
2 &			 1.14185 &	 -0.0779927 \\


==> convRate/convRate_F10_S5 <==
Number of fluid steps= 10 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04718  &  \\
1 &			 1.07637 &	 -0.0396646 \\
2 &			 1.11834 &	 -0.0551848 \\
3 &			 1.20162 &	 -0.103622 \\
4 &			 1.2899 &	 -0.102278 \\


==> convRate/convRate_F10_S6 <==
Number of fluid steps= 10 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05023  &  \\
1 &			 1.05285 &	 -0.0035946 \\
2 &			 1.05043 &	 0.00331988 \\
3 &			 1.09813 &	 -0.0640688 \\
4 &			 1.16997 &	 -0.0914227 \\


==> convRate/convRate_F10_S7 <==
Number of fluid steps= 10 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03856  &  \\
1 &			 1.00426 &	 0.0484517 \\
2 &			 0.931997 &	 0.107736 \\
3 &			 0.918279 &	 0.0213928 \\
4 &			 0.952381 &	 -0.0526063 \\


==> convRate/convRate_F10_S8 <==
Number of fluid steps= 10 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02922  &  \\
1 &			 0.927246 &	 0.150527 \\
2 &			 0.77149 &	 0.265305 \\
3 &			 0.683711 &	 0.174261 \\
4 &			 0.670378 &	 0.0284118 \\


==> convRate/convRate_F10_S9 <==
Number of fluid steps= 10 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01647  &  \\
1 &			 0.838747 &	 0.27726 \\
2 &			 0.597536 &	 0.48921 \\
3 &			 0.434059 &	 0.461134 \\
4 &			 0.36622 &	 0.245181 \\


==> convRate/convRate_F11_S1 <==
Number of fluid steps= 11 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01685 &	 -0.0241069 \\
2 &			 1.02658 &	 -0.0137392 \\


==> convRate/convRate_F11_S10 <==
Number of fluid steps= 11 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988727  &  \\
1 &			 0.796843 &	 0.311277 \\
2 &			 0.556423 &	 0.518113 \\
3 &			 0.398747 &	 0.480708 \\
4 &			 0.334514 &	 0.253407 \\


==> convRate/convRate_F11_S11 <==
Number of fluid steps= 11 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.930938  &  \\
1 &			 0.685526 &	 0.441474 \\
2 &			 0.410332 &	 0.74042 \\
3 &			 0.225169 &	 0.865783 \\
4 &			 0.118317 &	 0.928351 \\


==> convRate/convRate_F11_S12 <==
Number of fluid steps= 11 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.940298  &  \\
1 &			 0.693247 &	 0.439749 \\
2 &			 0.413706 &	 0.744764 \\
3 &			 0.223735 &	 0.886815 \\
4 &			 0.116077 &	 0.946709 \\


==> convRate/convRate_F11_S13 <==
Number of fluid steps= 11 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.934987  &  \\
1 &			 0.688349 &	 0.441806 \\
2 &			 0.405053 &	 0.76503 \\
3 &			 0.216679 &	 0.902551 \\
4 &			 0.112278 &	 0.948484 \\


==> convRate/convRate_F11_S14 <==
Number of fluid steps= 11 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.932972  &  \\
1 &			 0.680535 &	 0.455164 \\
2 &			 0.394796 &	 0.785562 \\
3 &			 0.208923 &	 0.918136 \\
4 &			 0.110353 &	 0.920845 \\


==> convRate/convRate_F11_S15 <==
Number of fluid steps= 11 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.929097  &  \\
1 &			 0.671495 &	 0.468453 \\
2 &			 0.383514 &	 0.808097 \\
3 &			 0.200796 &	 0.933549 \\
4 &			 0.109152 &	 0.879392 \\


==> convRate/convRate_F11_S16 <==
Number of fluid steps= 11 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.922041  &  \\
1 &			 0.661257 &	 0.47962 \\
2 &			 0.370704 &	 0.834943 \\
3 &			 0.19149 &	 0.952999 \\
4 &			 0.10577 &	 0.856339 \\


==> convRate/convRate_F11_S17 <==
Number of fluid steps= 11 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.918788  &  \\
1 &			 0.651984 &	 0.494895 \\
2 &			 0.360373 &	 0.855346 \\
3 &			 0.181609 &	 0.988655 \\
4 &			 0.0962007 &	 0.916716 \\


==> convRate/convRate_F11_S18 <==
Number of fluid steps= 11 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.91093  &  \\
1 &			 0.642447 &	 0.503763 \\
2 &			 0.349654 &	 0.877649 \\
3 &			 0.172072 &	 1.02292 \\
4 &			 0.0848686 &	 1.01971 \\


==> convRate/convRate_F11_S19 <==
Number of fluid steps= 11 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905112  &  \\
1 &			 0.633218 &	 0.515394 \\
2 &			 0.339808 &	 0.897982 \\
3 &			 0.164144 &	 1.04976 \\
4 &			 0.0785654 &	 1.063 \\


==> convRate/convRate_F11_S2 <==
Number of fluid steps= 11 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01621  &  \\
1 &			 1.0413 &	 -0.0351872 \\
2 &			 76.7888 &	 -6.20444 \\


==> convRate/convRate_F11_S20 <==
Number of fluid steps= 11 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.900334  &  \\
1 &			 0.623821 &	 0.529328 \\
2 &			 0.329904 &	 0.919086 \\
3 &			 0.156614 &	 1.07483 \\
4 &			 0.0736241 &	 1.08896 \\


==> convRate/convRate_F11_S3 <==
Number of fluid steps= 11 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02494  &  \\
1 &			 1.06492 &	 -0.0552056 \\


==> convRate/convRate_F11_S4 <==
Number of fluid steps= 11 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03319  &  \\
1 &			 1.0812 &	 -0.0655278 \\
2 &			 3.3849 &	 -1.64648 \\


==> convRate/convRate_F11_S5 <==
Number of fluid steps= 11 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05309  &  \\
1 &			 1.08309 &	 -0.0405244 \\
2 &			 1.14307 &	 -0.0777606 \\
3 &			 1.22156 &	 -0.095811 \\


==> convRate/convRate_F11_S6 <==
Number of fluid steps= 11 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03854  &  \\
1 &			 1.06639 &	 -0.0381784 \\
2 &			 1.09936 &	 -0.0439287 \\
3 &			 1.1766 &	 -0.09796 \\
4 &			 1.25956 &	 -0.0982959 \\


==> convRate/convRate_F11_S7 <==
Number of fluid steps= 11 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04471  &  \\
1 &			 1.0272 &	 0.0243854 \\
2 &			 1.0103 &	 0.0239334 \\
3 &			 1.04711 &	 -0.0516293 \\
4 &			 1.10858 &	 -0.0822999 \\


==> convRate/convRate_F11_S8 <==
Number of fluid steps= 11 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02954  &  \\
1 &			 0.966671 &	 0.090903 \\
2 &			 0.880921 &	 0.134012 \\
3 &			 0.858817 &	 0.0366619 \\
4 &			 0.884628 &	 -0.0427202 \\


==> convRate/convRate_F11_S9 <==
Number of fluid steps= 11 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00681  &  \\
1 &			 0.887464 &	 0.182031 \\
2 &			 0.723113 &	 0.295467 \\
3 &			 0.633216 &	 0.191523 \\
4 &			 0.616715 &	 0.0380938 \\


==> convRate/convRate_F12_S1 <==
Number of fluid steps= 12 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01626 &	 -0.0232695 \\
2 &			 1.01081 &	 0.00775771 \\


==> convRate/convRate_F12_S10 <==
Number of fluid steps= 12 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.985703  &  \\
1 &			 0.845729 &	 0.220958 \\
2 &			 0.676972 &	 0.321099 \\
3 &			 0.586915 &	 0.205945 \\
4 &			 0.569162 &	 0.0443122 \\


==> convRate/convRate_F12_S11 <==
Number of fluid steps= 12 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.961361  &  \\
1 &			 0.760243 &	 0.338618 \\
2 &			 0.521347 &	 0.544217 \\
3 &			 0.368847 &	 0.499221 \\
4 &			 0.30781 &	 0.260982 \\


==> convRate/convRate_F12_S12 <==
Number of fluid steps= 12 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905489  &  \\
1 &			 0.657705 &	 0.461256 \\
2 &			 0.389443 &	 0.756028 \\
3 &			 0.211005 &	 0.884135 \\
4 &			 0.109568 &	 0.945451 \\


==> convRate/convRate_F12_S13 <==
Number of fluid steps= 12 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.915061  &  \\
1 &			 0.664989 &	 0.460537 \\
2 &			 0.392544 &	 0.760476 \\
3 &			 0.209838 &	 0.903578 \\
4 &			 0.107687 &	 0.962432 \\


==> convRate/convRate_F12_S14 <==
Number of fluid steps= 12 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.908666  &  \\
1 &			 0.659611 &	 0.462135 \\
2 &			 0.384459 &	 0.778786 \\
3 &			 0.203719 &	 0.916249 \\
4 &			 0.104493 &	 0.963174 \\


==> convRate/convRate_F12_S15 <==
Number of fluid steps= 12 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905614  &  \\
1 &			 0.652037 &	 0.473942 \\
2 &			 0.375181 &	 0.797367 \\
3 &			 0.197168 &	 0.928161 \\
4 &			 0.103143 &	 0.93478 \\


==> convRate/convRate_F12_S16 <==
Number of fluid steps= 12 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.901228  &  \\
1 &			 0.643375 &	 0.486232 \\
2 &			 0.364999 &	 0.817767 \\
3 &			 0.190855 &	 0.935416 \\
4 &			 0.10432 &	 0.871461 \\


==> convRate/convRate_F12_S17 <==
Number of fluid steps= 12 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.899464  &  \\
1 &			 0.636632 &	 0.498606 \\
2 &			 0.355608 &	 0.840172 \\
3 &			 0.183002 &	 0.958428 \\
4 &			 0.100673 &	 0.862183 \\


==> convRate/convRate_F12_S18 <==
Number of fluid steps= 12 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.890098  &  \\
1 &			 0.624113 &	 0.512157 \\
2 &			 0.343243 &	 0.862577 \\
3 &			 0.175868 &	 0.964737 \\
4 &			 0.100378 &	 0.80905 \\


==> convRate/convRate_F12_S19 <==
Number of fluid steps= 12 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.887852  &  \\
1 &			 0.618843 &	 0.520746 \\
2 &			 0.335395 &	 0.883712 \\
3 &			 0.165428 &	 1.01966 \\
4 &			 0.0844785 &	 0.969547 \\


==> convRate/convRate_F12_S2 <==
Number of fluid steps= 12 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01633  &  \\
1 &			 1.03951 &	 -0.0325347 \\


==> convRate/convRate_F12_S20 <==
Number of fluid steps= 12 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.87936  &  \\
1 &			 0.608048 &	 0.532269 \\
2 &			 0.325365 &	 0.902126 \\
3 &			 0.157657 &	 1.04527 \\
4 &			 0.0762797 &	 1.04742 \\


==> convRate/convRate_F12_S3 <==
Number of fluid steps= 12 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02725  &  \\
1 &			 1.06208 &	 -0.0481051 \\


==> convRate/convRate_F12_S4 <==
Number of fluid steps= 12 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0367  &  \\
1 &			 1.07847 &	 -0.0569876 \\


==> convRate/convRate_F12_S5 <==
Number of fluid steps= 12 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04126  &  \\
1 &			 1.08518 &	 -0.059604 \\
2 &			 1.15056 &	 -0.0844019 \\


==> convRate/convRate_F12_S6 <==
Number of fluid steps= 12 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04295  &  \\
1 &			 1.07052 &	 -0.0376418 \\
2 &			 1.12848 &	 -0.0760691 \\
3 &			 1.2225 &	 -0.115454 \\
4 &			 1.30809 &	 -0.0976273 \\


==> convRate/convRate_F12_S7 <==
Number of fluid steps= 12 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04042  &  \\
1 &			 1.04522 &	 -0.0066406 \\
2 &			 1.06902 &	 -0.0324822 \\
3 &			 1.13895 &	 -0.0914156 \\
4 &			 1.21509 &	 -0.0933588 \\


==> convRate/convRate_F12_S8 <==
Number of fluid steps= 12 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02666  &  \\
1 &			 0.991724 &	 0.0499479 \\
2 &			 0.963195 &	 0.0421108 \\
3 &			 0.991558 &	 -0.0418693 \\
4 &			 1.04506 &	 -0.0758167 \\


==> convRate/convRate_F12_S9 <==
Number of fluid steps= 12 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00886  &  \\
1 &			 0.925521 &	 0.124388 \\
2 &			 0.830125 &	 0.156937 \\
3 &			 0.802394 &	 0.0490178 \\
4 &			 0.822533 &	 -0.0357627 \\


==> convRate/convRate_F13_S1 <==
Number of fluid steps= 13 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0157 &	 -0.0224743 \\
2 &			 1.0992 &	 -0.11398 \\


==> convRate/convRate_F13_S10 <==
Number of fluid steps= 13 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988269  &  \\
1 &			 0.893477 &	 0.145473 \\
2 &			 0.789133 &	 0.179162 \\
3 &			 0.755422 &	 0.0629857 \\
4 &			 0.769488 &	 -0.026616 \\


==> convRate/convRate_F13_S11 <==
Number of fluid steps= 13 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.962504  &  \\
1 &			 0.812372 &	 0.244652 \\
2 &			 0.63917 &	 0.345941 \\
3 &			 0.548593 &	 0.220463 \\
4 &			 0.529267 &	 0.0517405 \\


==> convRate/convRate_F13_S12 <==
Number of fluid steps= 13 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.935677  &  \\
1 &			 0.728404 &	 0.361272 \\
2 &			 0.491142 &	 0.568599 \\
3 &			 0.343228 &	 0.516973 \\
4 &			 0.285023 &	 0.268089 \\


==> convRate/convRate_F13_S13 <==
Number of fluid steps= 13 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.883247  &  \\
1 &			 0.634523 &	 0.477144 \\
2 &			 0.371483 &	 0.772376 \\
3 &			 0.198724 &	 0.90253 \\
4 &			 0.102032 &	 0.961744 \\


==> convRate/convRate_F13_S14 <==
Number of fluid steps= 13 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.892698  &  \\
1 &			 0.641355 &	 0.477049 \\
2 &			 0.374353 &	 0.776724 \\
3 &			 0.197769 &	 0.920583 \\
4 &			 0.100433 &	 0.977583 \\


==> convRate/convRate_F13_S15 <==
Number of fluid steps= 13 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.88769  &  \\
1 &			 0.636962 &	 0.478849 \\
2 &			 0.367596 &	 0.793086 \\
3 &			 0.192581 &	 0.932656 \\
4 &			 0.0976608 &	 0.979614 \\


==> convRate/convRate_F13_S16 <==
Number of fluid steps= 13 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.885135  &  \\
1 &			 0.630871 &	 0.488552 \\
2 &			 0.359692 &	 0.810583 \\
3 &			 0.18688 &	 0.94465 \\
4 &			 0.0962398 &	 0.957407 \\


==> convRate/convRate_F13_S17 <==
Number of fluid steps= 13 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.881561  &  \\
1 &			 0.62366 &	 0.499301 \\
2 &			 0.350873 &	 0.829811 \\
3 &			 0.181309 &	 0.952498 \\
4 &			 0.0971324 &	 0.900426 \\


==> convRate/convRate_F13_S18 <==
Number of fluid steps= 13 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.877876  &  \\
1 &			 0.616054 &	 0.51096 \\
2 &			 0.341971 &	 0.849183 \\
3 &			 0.175172 &	 0.965102 \\
4 &			 0.0962421 &	 0.864032 \\


==> convRate/convRate_F13_S19 <==
Number of fluid steps= 13 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.872218  &  \\
1 &			 0.607077 &	 0.522809 \\
2 &			 0.331847 &	 0.871361 \\
3 &			 0.168436 &	 0.978318 \\
4 &			 0.094789 &	 0.829409 \\


==> convRate/convRate_F13_S2 <==
Number of fluid steps= 13 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01537  &  \\
1 &			 1.03808 &	 -0.0319121 \\


==> convRate/convRate_F13_S20 <==
Number of fluid steps= 13 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.86958  &  \\
1 &			 0.600155 &	 0.534984 \\
2 &			 0.323861 &	 0.88996 \\
3 &			 0.1606 &	 1.0119 \\
4 &			 0.0866142 &	 0.890796 \\


==> convRate/convRate_F13_S3 <==
Number of fluid steps= 13 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02817  &  \\
1 &			 1.0601 &	 -0.0441215 \\


==> convRate/convRate_F13_S4 <==
Number of fluid steps= 13 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03937  &  \\
1 &			 1.07767 &	 -0.0522061 \\
2 &			 156457 &	 -17.1475 \\


==> convRate/convRate_F13_S5 <==
Number of fluid steps= 13 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04221  &  \\
1 &			 1.08601 &	 -0.0593914 \\
2 &			 9.76022 &	 -3.16788 \\


==> convRate/convRate_F13_S6 <==
Number of fluid steps= 13 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05009  &  \\
1 &			 1.08063 &	 -0.0413597 \\
2 &			 1.15369 &	 -0.094383 \\
3 &			 4.21531 &	 -1.86938 \\


==> convRate/convRate_F13_S7 <==
Number of fluid steps= 13 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03143  &  \\
1 &			 1.05948 &	 -0.0387104 \\
2 &			 1.11206 &	 -0.0698783 \\
3 &			 1.20156 &	 -0.111674 \\
4 &			 1.28325 &	 -0.0948936 \\


==> convRate/convRate_F13_S8 <==
Number of fluid steps= 13 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02692  &  \\
1 &			 1.02022 &	 0.00944351 \\
2 &			 1.03455 &	 -0.0201231 \\
3 &			 1.09621 &	 -0.0835208 \\
4 &			 1.16471 &	 -0.0874466 \\


==> convRate/convRate_F13_S9 <==
Number of fluid steps= 13 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00882  &  \\
1 &			 0.964166 &	 0.0653153 \\
2 &			 0.924486 &	 0.0606301 \\
3 &			 0.943134 &	 -0.0288113 \\
4 &			 0.987477 &	 -0.0662844 \\


==> convRate/convRate_F14_S1 <==
Number of fluid steps= 14 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01516 &	 -0.0217071 \\
2 &			 2.0784 &	 -1.03377 \\


==> convRate/convRate_F14_S10 <==
Number of fluid steps= 14 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.994591  &  \\
1 &			 0.930527 &	 0.0960554 \\
2 &			 0.882343 &	 0.0767084 \\
3 &			 0.893959 &	 -0.0188691 \\
4 &			 0.931804 &	 -0.0598179 \\


==> convRate/convRate_F14_S11 <==
Number of fluid steps= 14 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.970229  &  \\
1 &			 0.86009 &	 0.173838 \\
2 &			 0.748917 &	 0.199682 \\
3 &			 0.711153 &	 0.0746459 \\
4 &			 0.721084 &	 -0.0200074 \\


==> convRate/convRate_F14_S12 <==
Number of fluid steps= 14 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.941464  &  \\
1 &			 0.778391 &	 0.274411 \\
2 &			 0.603033 &	 0.368258 \\
3 &			 0.513078 &	 0.233059 \\
4 &			 0.493381 &	 0.056476 \\


==> convRate/convRate_F14_S13 <==
Number of fluid steps= 14 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.91236  &  \\
1 &			 0.700693 &	 0.380821 \\
2 &			 0.4649 &	 0.591862 \\
3 &			 0.321047 &	 0.534136 \\
4 &			 0.265361 &	 0.274828 \\


==> convRate/convRate_F14_S14 <==
Number of fluid steps= 14 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.864263  &  \\
1 &			 0.614989 &	 0.49091 \\
2 &			 0.355832 &	 0.789364 \\
3 &			 0.187963 &	 0.920748 \\
4 &			 0.0954705 &	 0.977322 \\


==> convRate/convRate_F14_S15 <==
Number of fluid steps= 14 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.873342  &  \\
1 &			 0.621385 &	 0.491059 \\
2 &			 0.358507 &	 0.793486 \\
3 &			 0.187179 &	 0.937583 \\
4 &			 0.0940963 &	 0.992209 \\


==> convRate/convRate_F14_S16 <==
Number of fluid steps= 14 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.867408  &  \\
1 &			 0.616659 &	 0.492238 \\
2 &			 0.35212 &	 0.808406 \\
3 &			 0.182575 &	 0.947578 \\
4 &			 0.0917029 &	 0.99345 \\


==> convRate/convRate_F14_S17 <==
Number of fluid steps= 14 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.867234  &  \\
1 &			 0.611876 &	 0.503182 \\
2 &			 0.345718 &	 0.823644 \\
3 &			 0.177768 &	 0.9596 \\
4 &			 0.090404 &	 0.975537 \\


==> convRate/convRate_F14_S18 <==
Number of fluid steps= 14 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.862673  &  \\
1 &			 0.605135 &	 0.511557 \\
2 &			 0.337761 &	 0.841254 \\
3 &			 0.173006 &	 0.965181 \\
4 &			 0.0914484 &	 0.919792 \\


==> convRate/convRate_F14_S19 <==
Number of fluid steps= 14 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.861162  &  \\
1 &			 0.599081 &	 0.523534 \\
2 &			 0.330282 &	 0.859053 \\
3 &			 0.16822 &	 0.973349 \\
4 &			 0.0924786 &	 0.863158 \\


==> convRate/convRate_F14_S2 <==
Number of fluid steps= 14 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01534  &  \\
1 &			 1.03659 &	 -0.0298825 \\


==> convRate/convRate_F14_S20 <==
Number of fluid steps= 14 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.854726  &  \\
1 &			 0.590573 &	 0.533347 \\
2 &			 0.321171 &	 0.878774 \\
3 &			 0.162322 &	 0.984483 \\
4 &			 0.091044 &	 0.834223 \\


==> convRate/convRate_F14_S3 <==
Number of fluid steps= 14 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02277  &  \\
1 &			 1.05832 &	 -0.0492942 \\


==> convRate/convRate_F14_S4 <==
Number of fluid steps= 14 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03398  &  \\
1 &			 1.07563 &	 -0.0569736 \\


==> convRate/convRate_F14_S5 <==
Number of fluid steps= 14 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03433  &  \\
1 &			 1.08636 &	 -0.0708057 \\


==> convRate/convRate_F14_S6 <==
Number of fluid steps= 14 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04135  &  \\
1 &			 1.08448 &	 -0.0585484 \\
2 &			 1.16076 &	 -0.0980663 \\


==> convRate/convRate_F14_S7 <==
Number of fluid steps= 14 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03514  &  \\
1 &			 1.06575 &	 -0.0420432 \\
2 &			 1.13934 &	 -0.0963293 \\
3 &			 1.24001 &	 -0.122153 \\
4 &			 1.32212 &	 -0.0925014 \\


==> convRate/convRate_F14_S8 <==
Number of fluid steps= 14 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02895  &  \\
1 &			 1.03801 &	 -0.0126475 \\
2 &			 1.08534 &	 -0.0643267 \\
3 &			 1.16976 &	 -0.108066 \\
4 &			 1.24671 &	 -0.0919134 \\


==> convRate/convRate_F14_S9 <==
Number of fluid steps= 14 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01724  &  \\
1 &			 0.992953 &	 0.0348628 \\
2 &			 0.998329 &	 -0.0077899 \\
3 &			 1.05167 &	 -0.0750948 \\
4 &			 1.11263 &	 -0.0812918 \\


==> convRate/convRate_F15_S1 <==
Number of fluid steps= 15 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01463 &	 -0.0209537 \\


==> convRate/convRate_F15_S10 <==
Number of fluid steps= 15 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.995738  &  \\
1 &			 0.960593 &	 0.0518409 \\
2 &			 0.958117 &	 0.00372345 \\
3 &			 1.00483 &	 -0.0686777 \\


==> convRate/convRate_F15_S2 <==
Number of fluid steps= 15 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01456  &  \\
1 &			 1.03537 &	 -0.0292922 \\


==> convRate/convRate_F15_S3 <==
Number of fluid steps= 15 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0242  &  \\
1 &			 1.05591 &	 -0.0439894 \\


==> convRate/convRate_F15_S4 <==
Number of fluid steps= 15 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02883  &  \\
1 &			 1.07421 &	 -0.0622714 \\


==> convRate/convRate_F15_S5 <==
Number of fluid steps= 15 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0371  &  \\
1 &			 1.08472 &	 -0.0647677 \\


==> convRate/convRate_F15_S6 <==
Number of fluid steps= 15 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03915  &  \\
1 &			 1.08717 &	 -0.0651736 \\
2 &			 943.971 &	 -9.76202 \\


==> convRate/convRate_F15_S7 <==
Number of fluid steps= 15 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04326  &  \\
1 &			 1.07811 &	 -0.0474056 \\
2 &			 1.16385 &	 -0.110401 \\
3 &			 1.31889 &	 -0.180419 \\


==> convRate/convRate_F15_S8 <==
Number of fluid steps= 15 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02251  &  \\
1 &			 1.05492 &	 -0.0450186 \\
2 &			 1.12492 &	 -0.0926888 \\
3 &			 1.22203 &	 -0.119457 \\
4 &			 1.30117 &	 -0.0905298 \\


==> convRate/convRate_F15_S9 <==
Number of fluid steps= 15 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01512  &  \\
1 &			 1.01447 &	 0.00092408 \\
2 &			 1.05521 &	 -0.0568039 \\
3 &			 1.13329 &	 -0.102987 \\
4 &			 1.20458 &	 -0.0880131 \\


==> convRate/convRate_F1_S1 <==
Number of fluid steps= 1 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02579 &	 -0.0367354 \\
2 &			 1.07106 &	 -0.0623039 \\
3 &			 1.08424 &	 -0.0176448 \\
4 &			 0.805303 &	 0.429081 \\


==> convRate/convRate_F1_S10 <==
Number of fluid steps= 1 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03624 &	 -0.0513582 \\
2 &			 1.11802 &	 -0.109588 \\
3 &			 1.07765 &	 0.0530573 \\
4 &			 0.64695 &	 0.736163 \\


==> convRate/convRate_F1_S11 <==
Number of fluid steps= 1 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03723 &	 -0.0527358 \\
2 &			 1.11937 &	 -0.109951 \\
3 &			 1.07774 &	 0.0546778 \\
4 &			 0.64554 &	 0.739431 \\


==> convRate/convRate_F1_S12 <==
Number of fluid steps= 1 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03824 &	 -0.05414 \\
2 &			 1.12052 &	 -0.110028 \\
3 &			 1.07782 &	 0.0560521 \\
4 &			 0.644406 &	 0.742074 \\


==> convRate/convRate_F1_S13 <==
Number of fluid steps= 1 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03927 &	 -0.0555705 \\
2 &			 1.12152 &	 -0.109885 \\
3 &			 1.07791 &	 0.0572186 \\
4 &			 0.64348 &	 0.74427 \\


==> convRate/convRate_F1_S14 <==
Number of fluid steps= 1 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04032 &	 -0.0570274 \\
2 &			 1.12239 &	 -0.109547 \\
3 &			 1.07799 &	 0.0582303 \\
4 &			 0.64271 &	 0.746104 \\


==> convRate/convRate_F1_S15 <==
Number of fluid steps= 1 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04139 &	 -0.0585105 \\
2 &			 1.12316 &	 -0.109053 \\
3 &			 1.07807 &	 0.0591126 \\
4 &			 0.642062 &	 0.747666 \\


==> convRate/convRate_F1_S16 <==
Number of fluid steps= 1 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04247 &	 -0.0600059 \\
2 &			 1.12384 &	 -0.108431 \\
3 &			 1.07815 &	 0.0598787 \\
4 &			 0.641511 &	 0.749012 \\


==> convRate/convRate_F1_S17 <==
Number of fluid steps= 1 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04356 &	 -0.0615136 \\
2 &			 1.12444 &	 -0.107693 \\
3 &			 1.07822 &	 0.0605551 \\
4 &			 0.641037 &	 0.750172 \\


==> convRate/convRate_F1_S18 <==
Number of fluid steps= 1 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04465 &	 -0.0630197 \\
2 &			 1.12499 &	 -0.106893 \\
3 &			 1.07829 &	 0.0611669 \\
4 &			 0.640627 &	 0.751189 \\


==> convRate/convRate_F1_S19 <==
Number of fluid steps= 1 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04575 &	 -0.064538 \\
2 &			 1.12548 &	 -0.106002 \\
3 &			 1.07835 &	 0.0617149 \\
4 &			 0.640267 &	 0.75208 \\


==> convRate/convRate_F1_S2 <==
Number of fluid steps= 1 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02893 &	 -0.0411448 \\
2 &			 1.0859 &	 -0.0777464 \\
3 &			 1.08077 &	 0.00683172 \\
4 &			 0.725089 &	 0.57583 \\


==> convRate/convRate_F1_S20 <==
Number of fluid steps= 1 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04684 &	 -0.066041 \\
2 &			 1.12592 &	 -0.105063 \\
3 &			 1.07841 &	 0.0621985 \\
4 &			 0.639951 &	 0.752872 \\


==> convRate/convRate_F1_S3 <==
Number of fluid steps= 1 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03021 &	 -0.0429384 \\
2 &			 1.09474 &	 -0.0876498 \\
3 &			 1.07887 &	 0.0210672 \\
4 &			 0.691975 &	 0.640729 \\


==> convRate/convRate_F1_S4 <==
Number of fluid steps= 1 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03107 &	 -0.0441423 \\
2 &			 1.10104 &	 -0.0947246 \\
3 &			 1.07801 &	 0.0304963 \\
4 &			 0.674954 &	 0.675509 \\


==> convRate/convRate_F1_S5 <==
Number of fluid steps= 1 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03185 &	 -0.0452333 \\
2 &			 1.10574 &	 -0.0997789 \\
3 &			 1.07764 &	 0.0371369 \\
4 &			 0.664974 &	 0.696505 \\


==> convRate/convRate_F1_S6 <==
Number of fluid steps= 1 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03265 &	 -0.0463514 \\
2 &			 1.10936 &	 -0.103376 \\
3 &			 1.07749 &	 0.0420531 \\
4 &			 0.658577 &	 0.71025 \\


==> convRate/convRate_F1_S7 <==
Number of fluid steps= 1 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03349 &	 -0.0475244 \\
2 &			 1.11221 &	 -0.105905 \\
3 &			 1.07747 &	 0.0457815 \\
4 &			 0.654208 &	 0.719826 \\


==> convRate/convRate_F1_S8 <==
Number of fluid steps= 1 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03437 &	 -0.0487523 \\
2 &			 1.11452 &	 -0.10767 \\
3 &			 1.0775 &	 0.0487346 \\
4 &			 0.651074 &	 0.726794 \\


==> convRate/convRate_F1_S9 <==
Number of fluid steps= 1 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03529 &	 -0.0500349 \\
2 &			 1.11643 &	 -0.108858 \\
3 &			 1.07757 &	 0.0511112 \\
4 &			 0.648741 &	 0.732067 \\


==> convRate/convRate_F2_S1 <==
Number of fluid steps= 2 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0247 &	 -0.0352016 \\
2 &			 1.06366 &	 -0.0538355 \\
3 &			 1.10668 &	 -0.0572011 \\
4 &			 1.12766 &	 -0.027094 \\


==> convRate/convRate_F2_S10 <==
Number of fluid steps= 2 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02989  &  \\
1 &			 1.09978 &	 -0.0947247 \\
2 &			 1.0691 &	 0.0408182 \\
3 &			 0.664408 &	 0.686255 \\
4 &			 0.268271 &	 1.30838 \\


==> convRate/convRate_F2_S11 <==
Number of fluid steps= 2 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03022  &  \\
1 &			 1.09814 &	 -0.0921095 \\
2 &			 1.06899 &	 0.0388136 \\
3 &			 0.664884 &	 0.685074 \\
4 &			 0.266073 &	 1.32128 \\


==> convRate/convRate_F2_S12 <==
Number of fluid steps= 2 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03067  &  \\
1 &			 1.10291 &	 -0.0977326 \\
2 &			 1.0684 &	 0.0458632 \\
3 &			 0.657758 &	 0.699823 \\
4 &			 0.259827 &	 1.34001 \\


==> convRate/convRate_F2_S13 <==
Number of fluid steps= 2 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03107  &  \\
1 &			 1.10134 &	 -0.0951176 \\
2 &			 1.06858 &	 0.043565 \\
3 &			 0.658866 &	 0.697638 \\
4 &			 0.258842 &	 1.34791 \\


==> convRate/convRate_F2_S14 <==
Number of fluid steps= 2 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03148  &  \\
1 &			 1.10535 &	 -0.0997874 \\
2 &			 1.06793 &	 0.0496862 \\
3 &			 0.653173 &	 0.70928 \\
4 &			 0.254184 &	 1.36159 \\


==> convRate/convRate_F2_S15 <==
Number of fluid steps= 2 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03196  &  \\
1 &			 1.10392 &	 -0.0972486 \\
2 &			 1.06829 &	 0.0473323 \\
3 &			 0.654607 &	 0.706602 \\
4 &			 0.253901 &	 1.36636 \\


==> convRate/convRate_F2_S16 <==
Number of fluid steps= 2 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03233  &  \\
1 &			 1.10731 &	 -0.101155 \\
2 &			 1.0676 &	 0.052688 \\
3 &			 0.649855 &	 0.716181 \\
4 &			 0.250218 &	 1.37693 \\


==> convRate/convRate_F2_S17 <==
Number of fluid steps= 2 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03288  &  \\
1 &			 1.10602 &	 -0.0987048 \\
2 &			 1.06809 &	 0.0503443 \\
3 &			 0.651454 &	 0.713298 \\
4 &			 0.25036 &	 1.37966 \\


==> convRate/convRate_F2_S18 <==
Number of fluid steps= 2 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03322  &  \\
1 &			 1.10891 &	 -0.101995 \\
2 &			 1.06736 &	 0.0550954 \\
3 &			 0.647364 &	 0.721398 \\
4 &			 0.247319 &	 1.3882 \\


==> convRate/convRate_F2_S19 <==
Number of fluid steps= 2 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03384  &  \\
1 &			 1.10777 &	 -0.0996454 \\
2 &			 1.06794 &	 0.0528278 \\
3 &			 0.649039 &	 0.718454 \\
4 &			 0.247726 &	 1.38956 \\


==> convRate/convRate_F2_S2 <==
Number of fluid steps= 2 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02422  &  \\
1 &			 1.06849 &	 -0.0610478 \\
2 &			 1.08069 &	 -0.0163793 \\
3 &			 0.805655 &	 0.423719 \\
4 &			 0.471993 &	 0.771397 \\


==> convRate/convRate_F2_S20 <==
Number of fluid steps= 2 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03414  &  \\
1 &			 1.11024 &	 -0.10244 \\
2 &			 1.06719 &	 0.0570545 \\
3 &			 0.645436 &	 0.725471 \\
4 &			 0.245132 &	 1.39672 \\


==> convRate/convRate_F2_S3 <==
Number of fluid steps= 2 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02415  &  \\
1 &			 1.0694 &	 -0.0623745 \\
2 &			 1.07651 &	 -0.00956014 \\
3 &			 0.773582 &	 0.476736 \\
4 &			 0.418724 &	 0.885555 \\


==> convRate/convRate_F2_S4 <==
Number of fluid steps= 2 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0271  &  \\
1 &			 1.08208 &	 -0.0752305 \\
2 &			 1.07524 &	 0.00914845 \\
3 &			 0.725441 &	 0.567729 \\
4 &			 0.352577 &	 1.04092 \\


==> convRate/convRate_F2_S5 <==
Number of fluid steps= 2 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02708  &  \\
1 &			 1.08129 &	 -0.0742049 \\
2 &			 1.07299 &	 0.0111169 \\
3 &			 0.715412 &	 0.58479 \\
4 &			 0.333159 &	 1.10256 \\


==> convRate/convRate_F2_S6 <==
Number of fluid steps= 2 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0283  &  \\
1 &			 1.09005 &	 -0.0841331 \\
2 &			 1.07201 &	 0.0240759 \\
3 &			 0.692031 &	 0.63141 \\
4 &			 0.305358 &	 1.18034 \\


==> convRate/convRate_F2_S7 <==
Number of fluid steps= 2 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02844  &  \\
1 &			 1.08872 &	 -0.0821753 \\
2 &			 1.07082 &	 0.023917 \\
3 &			 0.688582 &	 0.637016 \\
4 &			 0.296455 &	 1.21582 \\


==> convRate/convRate_F2_S8 <==
Number of fluid steps= 2 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02914  &  \\
1 &			 1.09565 &	 -0.0903478 \\
2 &			 1.07019 &	 0.0339201 \\
3 &			 0.674684 &	 0.665583 \\
4 &			 0.281762 &	 1.25973 \\


==> convRate/convRate_F2_S9 <==
Number of fluid steps= 2 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02937  &  \\
1 &			 1.09407 &	 -0.0879434 \\
2 &			 1.06966 &	 0.0325527 \\
3 &			 0.673907 &	 0.666531 \\
4 &			 0.277339 &	 1.2809 \\


==> convRate/convRate_F3_S1 <==
Number of fluid steps= 3 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02354 &	 -0.0335675 \\
2 &			 1.05762 &	 -0.0472539 \\
3 &			 1.10304 &	 -0.0606637 \\


==> convRate/convRate_F3_S10 <==
Number of fluid steps= 3 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05414  &  \\
1 &			 1.10473 &	 -0.0676273 \\
2 &			 0.882649 &	 0.323782 \\
3 &			 0.443573 &	 0.992668 \\
4 &			 0.181382 &	 1.29014 \\


==> convRate/convRate_F3_S11 <==
Number of fluid steps= 3 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05549  &  \\
1 &			 1.10699 &	 -0.0687293 \\
2 &			 0.878861 &	 0.332935 \\
3 &			 0.435511 &	 1.01293 \\
4 &			 0.174017 &	 1.32348 \\


==> convRate/convRate_F3_S12 <==
Number of fluid steps= 3 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0574  &  \\
1 &			 1.10439 &	 -0.0627285 \\
2 &			 0.865651 &	 0.351392 \\
3 &			 0.419359 &	 1.0456 \\
4 &			 0.16257 &	 1.36712 \\


==> convRate/convRate_F3_S13 <==
Number of fluid steps= 3 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05758  &  \\
1 &			 1.10652 &	 -0.0652627 \\
2 &			 0.870541 &	 0.346045 \\
3 &			 0.422064 &	 1.04445 \\
4 &			 0.1619 &	 1.38236 \\


==> convRate/convRate_F3_S14 <==
Number of fluid steps= 3 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05882  &  \\
1 &			 1.10809 &	 -0.0656177 \\
2 &			 0.86837 &	 0.351693 \\
3 &			 0.417401 &	 1.05688 \\
4 &			 0.157817 &	 1.40318 \\


==> convRate/convRate_F3_S15 <==
Number of fluid steps= 3 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06032  &  \\
1 &			 1.10536 &	 -0.0600166 \\
2 &			 0.858139 &	 0.365233 \\
3 &			 0.405899 &	 1.08009 \\
4 &			 0.150262 &	 1.43364 \\


==> convRate/convRate_F3_S16 <==
Number of fluid steps= 3 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0605  &  \\
1 &			 1.10742 &	 -0.0624579 \\
2 &			 0.862815 &	 0.360079 \\
3 &			 0.409059 &	 1.07674 \\
4 &			 0.150632 &	 1.44128 \\


==> convRate/convRate_F3_S17 <==
Number of fluid steps= 3 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06164  &  \\
1 &			 1.1086 &	 -0.0624443 \\
2 &			 0.861475 &	 0.363858 \\
3 &			 0.406094 &	 1.085 \\
4 &			 0.148135 &	 1.4549 \\


==> convRate/convRate_F3_S18 <==
Number of fluid steps= 3 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06287  &  \\
1 &			 1.10596 &	 -0.0573341 \\
2 &			 0.853126 &	 0.374468 \\
3 &			 0.397253 &	 1.1027 \\
4 &			 0.142653 &	 1.47755 \\


==> convRate/convRate_F3_S19 <==
Number of fluid steps= 3 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06303  &  \\
1 &			 1.1079 &	 -0.0596454 \\
2 &			 0.857502 &	 0.369616 \\
3 &			 0.4005 &	 1.09834 \\
4 &			 0.143526 &	 1.48049 \\


==> convRate/convRate_F3_S2 <==
Number of fluid steps= 3 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01313  &  \\
1 &			 1.06469 &	 -0.0716141 \\
2 &			 1.09962 &	 -0.0465716 \\
3 &			 1.03727 &	 0.0842136 \\
4 &			 0.981679 &	 0.0794682 \\


==> convRate/convRate_F3_S20 <==
Number of fluid steps= 3 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06407  &  \\
1 &			 1.10884 &	 -0.0594581 \\
2 &			 0.856635 &	 0.372299 \\
3 &			 0.398485 &	 1.10416 \\
4 &			 0.141888 &	 1.48977 \\


==> convRate/convRate_F3_S3 <==
Number of fluid steps= 3 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04252  &  \\
1 &			 1.09027 &	 -0.0646104 \\
2 &			 0.951307 &	 0.196703 \\
3 &			 0.596548 &	 0.673273 \\
4 &			 0.343489 &	 0.796374 \\


==> convRate/convRate_F3_S4 <==
Number of fluid steps= 3 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04247  &  \\
1 &			 1.09073 &	 -0.0652882 \\
2 &			 0.946816 &	 0.204138 \\
3 &			 0.576965 &	 0.7146 \\
4 &			 0.315791 &	 0.869514 \\


==> convRate/convRate_F3_S5 <==
Number of fluid steps= 3 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04502  &  \\
1 &			 1.09774 &	 -0.0710058 \\
2 &			 0.929583 &	 0.239881 \\
3 &			 0.535769 &	 0.794973 \\
4 &			 0.271903 &	 0.978519 \\


==> convRate/convRate_F3_S6 <==
Number of fluid steps= 3 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04967  &  \\
1 &			 1.09917 &	 -0.0664787 \\
2 &			 0.900469 &	 0.287666 \\
3 &			 0.486974 &	 0.886832 \\
4 &			 0.22842 &	 1.09216 \\


==> convRate/convRate_F3_S7 <==
Number of fluid steps= 3 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04977  &  \\
1 &			 1.10084 &	 -0.0685315 \\
2 &			 0.903779 &	 0.284563 \\
3 &			 0.483912 &	 0.901225 \\
4 &			 0.21979 &	 1.13862 \\


==> convRate/convRate_F3_S8 <==
Number of fluid steps= 3 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05132  &  \\
1 &			 1.10445 &	 -0.0711262 \\
2 &			 0.896367 &	 0.301167 \\
3 &			 0.467804 &	 0.938185 \\
4 &			 0.204279 &	 1.19536 \\


==> convRate/convRate_F3_S9 <==
Number of fluid steps= 3 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05397  &  \\
1 &			 1.10264 &	 -0.065128 \\
2 &			 0.877891 &	 0.328848 \\
3 &			 0.442289 &	 0.989052 \\
4 &			 0.184334 &	 1.26267 \\


==> convRate/convRate_F4_S1 <==
Number of fluid steps= 4 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02244 &	 -0.0320162 \\
2 &			 1.05271 &	 -0.0420919 \\
3 &			 1.09311 &	 -0.0543305 \\


==> convRate/convRate_F4_S10 <==
Number of fluid steps= 4 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06685  &  \\
1 &			 1.05 &	 0.022968 \\
2 &			 0.71699 &	 0.550364 \\
3 &			 0.341163 &	 1.07149 \\
4 &			 0.152242 &	 1.16409 \\


==> convRate/convRate_F4_S11 <==
Number of fluid steps= 4 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07054  &  \\
1 &			 1.05348 &	 0.0231758 \\
2 &			 0.713385 &	 0.56241 \\
3 &			 0.333678 &	 1.09622 \\
4 &			 0.144971 &	 1.20269 \\


==> convRate/convRate_F4_S12 <==
Number of fluid steps= 4 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07245  &  \\
1 &			 1.04401 &	 0.0387749 \\
2 &			 0.692166 &	 0.592946 \\
3 &			 0.313105 &	 1.14447 \\
4 &			 0.131393 &	 1.25276 \\


==> convRate/convRate_F4_S13 <==
Number of fluid steps= 4 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07295  &  \\
1 &			 1.04768 &	 0.0343847 \\
2 &			 0.699036 &	 0.583759 \\
3 &			 0.31579 &	 1.1464 \\
4 &			 0.130557 &	 1.27429 \\


==> convRate/convRate_F4_S14 <==
Number of fluid steps= 4 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07127  &  \\
1 &			 1.04302 &	 0.0385553 \\
2 &			 0.688734 &	 0.598748 \\
3 &			 0.30437 &	 1.17812 \\
4 &			 0.121974 &	 1.31925 \\


==> convRate/convRate_F4_S15 <==
Number of fluid steps= 4 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0744  &  \\
1 &			 1.0464 &	 0.0380968 \\
2 &			 0.68863 &	 0.603634 \\
3 &			 0.302521 &	 1.18669 \\
4 &			 0.120325 &	 1.3301 \\


==> convRate/convRate_F4_S16 <==
Number of fluid steps= 4 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07566  &  \\
1 &			 1.03863 &	 0.0505403 \\
2 &			 0.673546 &	 0.624833 \\
3 &			 0.289224 &	 1.21959 \\
4 &			 0.112203 &	 1.36608 \\


==> convRate/convRate_F4_S17 <==
Number of fluid steps= 4 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07617  &  \\
1 &			 1.042 &	 0.0465507 \\
2 &			 0.680021 &	 0.615704 \\
3 &			 0.292655 &	 1.21638 \\
4 &			 0.112658 &	 1.37725 \\


==> convRate/convRate_F4_S18 <==
Number of fluid steps= 4 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07423  &  \\
1 &			 1.03834 &	 0.049024 \\
2 &			 0.672678 &	 0.626291 \\
3 &			 0.284841 &	 1.23976 \\
4 &			 0.1067 &	 1.4166 \\


==> convRate/convRate_F4_S19 <==
Number of fluid steps= 4 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07694  &  \\
1 &			 1.04147 &	 0.0483166 \\
2 &			 0.67379 &	 0.62825 \\
3 &			 0.284958 &	 1.24155 \\
4 &			 0.106918 &	 1.41424 \\


==> convRate/convRate_F4_S2 <==
Number of fluid steps= 4 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02211  &  \\
1 &			 1.05944 &	 -0.0517514 \\
2 &			 1.10144 &	 -0.056089 \\
3 &			 1.12424 &	 -0.0295591 \\
4 &			 1.18376 &	 -0.0744266 \\


==> convRate/convRate_F4_S20 <==
Number of fluid steps= 4 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07784  &  \\
1 &			 1.0349 &	 0.0586517 \\
2 &			 0.662125 &	 0.644316 \\
3 &			 0.275323 &	 1.26598 \\
4 &			 0.101352 &	 1.44175 \\


==> convRate/convRate_F4_S3 <==
Number of fluid steps= 4 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04061  &  \\
1 &			 1.08993 &	 -0.066806 \\
2 &			 1.04319 &	 0.0632335 \\
3 &			 0.897305 &	 0.217332 \\
4 &			 0.814145 &	 0.140313 \\


==> convRate/convRate_F4_S4 <==
Number of fluid steps= 4 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05847  &  \\
1 &			 1.06556 &	 -0.00963145 \\
2 &			 0.806965 &	 0.401034 \\
3 &			 0.477817 &	 0.756048 \\
4 &			 0.274237 &	 0.801035 \\


==> convRate/convRate_F4_S5 <==
Number of fluid steps= 4 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05869  &  \\
1 &			 1.06748 &	 -0.0119288 \\
2 &			 0.807415 &	 0.402827 \\
3 &			 0.466344 &	 0.791916 \\
4 &			 0.258064 &	 0.853666 \\


==> convRate/convRate_F4_S6 <==
Number of fluid steps= 4 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0591  &  \\
1 &			 1.06043 &	 -0.00181058 \\
2 &			 0.775891 &	 0.450723 \\
3 &			 0.425638 &	 0.866227 \\
4 &			 0.227285 &	 0.905124 \\


==> convRate/convRate_F4_S7 <==
Number of fluid steps= 4 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0639  &  \\
1 &			 1.06385 &	 6.78038e-05 \\
2 &			 0.761163 &	 0.483017 \\
3 &			 0.39875 &	 0.932721 \\
4 &			 0.198898 &	 1.00346 \\


==> convRate/convRate_F4_S8 <==
Number of fluid steps= 4 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06753  &  \\
1 &			 1.0523 &	 0.0207306 \\
2 &			 0.726742 &	 0.534031 \\
3 &			 0.360135 &	 1.01291 \\
4 &			 0.170355 &	 1.07999 \\


==> convRate/convRate_F4_S9 <==
Number of fluid steps= 4 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.068  &  \\
1 &			 1.05601 &	 0.0162882 \\
2 &			 0.733139 &	 0.526465 \\
3 &			 0.360068 &	 1.02582 \\
4 &			 0.166162 &	 1.11568 \\


==> convRate/convRate_F5_S1 <==
Number of fluid steps= 5 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02143 &	 -0.0305903 \\
2 &			 1.04866 &	 -0.0379567 \\


==> convRate/convRate_F5_S10 <==
Number of fluid steps= 5 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0701  &  \\
1 &			 0.969327 &	 0.14269 \\
2 &			 0.596856 &	 0.699601 \\
3 &			 0.286723 &	 1.05773 \\
4 &			 0.136658 &	 1.06909 \\


==> convRate/convRate_F5_S11 <==
Number of fluid steps= 5 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07161  &  \\
1 &			 0.97506 &	 0.136217 \\
2 &			 0.60425 &	 0.690345 \\
3 &			 0.287735 &	 1.0704 \\
4 &			 0.1344 &	 1.09821 \\


==> convRate/convRate_F5_S12 <==
Number of fluid steps= 5 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07029  &  \\
1 &			 0.971898 &	 0.139125 \\
2 &			 0.593959 &	 0.710442 \\
3 &			 0.275873 &	 1.10636 \\
4 &			 0.125772 &	 1.13319 \\


==> convRate/convRate_F5_S13 <==
Number of fluid steps= 5 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07208  &  \\
1 &			 0.967564 &	 0.147984 \\
2 &			 0.584823 &	 0.726357 \\
3 &			 0.26601 &	 1.13652 \\
4 &			 0.118319 &	 1.1688 \\


==> convRate/convRate_F5_S14 <==
Number of fluid steps= 5 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0723  &  \\
1 &			 0.964902 &	 0.152254 \\
2 &			 0.575995 &	 0.744326 \\
3 &			 0.257087 &	 1.1638 \\
4 &			 0.11213 &	 1.19708 \\


==> convRate/convRate_F5_S15 <==
Number of fluid steps= 5 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0712  &  \\
1 &			 0.949946 &	 0.17331 \\
2 &			 0.555675 &	 0.773604 \\
3 &			 0.24079 &	 1.20647 \\
4 &			 0.102342 &	 1.23438 \\


==> convRate/convRate_F5_S16 <==
Number of fluid steps= 5 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07271  &  \\
1 &			 0.95523 &	 0.16734 \\
2 &			 0.56305 &	 0.762585 \\
3 &			 0.243703 &	 1.20814 \\
4 &			 0.102293 &	 1.25242 \\


==> convRate/convRate_F5_S17 <==
Number of fluid steps= 5 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07146  &  \\
1 &			 0.953827 &	 0.167778 \\
2 &			 0.557335 &	 0.775183 \\
3 &			 0.23713 &	 1.23287 \\
4 &			 0.097206 &	 1.28656 \\


==> convRate/convRate_F5_S18 <==
Number of fluid steps= 5 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07296  &  \\
1 &			 0.951244 &	 0.173709 \\
2 &			 0.552622 &	 0.783522 \\
3 &			 0.232373 &	 1.24985 \\
4 &			 0.0938374 &	 1.30821 \\


==> convRate/convRate_F5_S19 <==
Number of fluid steps= 5 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07249  &  \\
1 &			 0.949995 &	 0.174972 \\
2 &			 0.548008 &	 0.793723 \\
3 &			 0.228281 &	 1.26339 \\
4 &			 0.0914663 &	 1.3195 \\


==> convRate/convRate_F5_S2 <==
Number of fluid steps= 5 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01738  &  \\
1 &			 1.05626 &	 -0.0541064 \\
2 &			 1.10178 &	 -0.0608712 \\
3 &			 1.15591 &	 -0.0691929 \\


==> convRate/convRate_F5_S20 <==
Number of fluid steps= 5 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07122  &  \\
1 &			 0.938306 &	 0.191124 \\
2 &			 0.533577 &	 0.814362 \\
3 &			 0.217592 &	 1.29407 \\
4 &			 0.0854429 &	 1.34859 \\


==> convRate/convRate_F5_S3 <==
Number of fluid steps= 5 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02705  &  \\
1 &			 1.08496 &	 -0.0791354 \\
2 &			 1.0859 &	 -0.0012494 \\
3 &			 1.0672 &	 0.0250607 \\
4 &			 1.10536 &	 -0.0506857 \\


==> convRate/convRate_F5_S4 <==
Number of fluid steps= 5 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06455  &  \\
1 &			 1.08133 &	 -0.0225632 \\
2 &			 0.949449 &	 0.187644 \\
3 &			 0.771417 &	 0.29958 \\
4 &			 0.683357 &	 0.174871 \\


==> convRate/convRate_F5_S5 <==
Number of fluid steps= 5 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06545  &  \\
1 &			 1.00699 &	 0.0814135 \\
2 &			 0.693507 &	 0.538067 \\
3 &			 0.403654 &	 0.780791 \\
4 &			 0.229625 &	 0.813839 \\


==> convRate/convRate_F5_S6 <==
Number of fluid steps= 5 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06652  &  \\
1 &			 1.01123 &	 0.0767999 \\
2 &			 0.696872 &	 0.537146 \\
3 &			 0.396303 &	 0.81429 \\
4 &			 0.219097 &	 0.855034 \\


==> convRate/convRate_F5_S7 <==
Number of fluid steps= 5 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06569  &  \\
1 &			 1.00365 &	 0.0865316 \\
2 &			 0.672788 &	 0.577032 \\
3 &			 0.368056 &	 0.870227 \\
4 &			 0.199518 &	 0.883406 \\


==> convRate/convRate_F5_S8 <==
Number of fluid steps= 5 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06848  &  \\
1 &			 0.995372 &	 0.102252 \\
2 &			 0.650266 &	 0.614206 \\
3 &			 0.340737 &	 0.932371 \\
4 &			 0.175954 &	 0.95346 \\


==> convRate/convRate_F5_S9 <==
Number of fluid steps= 5 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07032  &  \\
1 &			 0.989864 &	 0.11274 \\
2 &			 0.630087 &	 0.651679 \\
3 &			 0.317005 &	 0.991045 \\
4 &			 0.15679 &	 1.01567 \\


==> convRate/convRate_F6_S1 <==
Number of fluid steps= 6 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0205 &	 -0.0292762 \\
2 &			 1.04525 &	 -0.0345719 \\


==> convRate/convRate_F6_S10 <==
Number of fluid steps= 6 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06056  &  \\
1 &			 0.9112 &	 0.218987 \\
2 &			 0.551638 &	 0.724046 \\
3 &			 0.282331 &	 0.966334 \\
4 &			 0.143288 &	 0.97847 \\


==> convRate/convRate_F6_S11 <==
Number of fluid steps= 6 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05914  &  \\
1 &			 0.904431 &	 0.227811 \\
2 &			 0.5346 &	 0.758551 \\
3 &			 0.263789 &	 1.01908 \\
4 &			 0.129376 &	 1.02781 \\


==> convRate/convRate_F6_S12 <==
Number of fluid steps= 6 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05435  &  \\
1 &			 0.879988 &	 0.260798 \\
2 &			 0.504881 &	 0.80154 \\
3 &			 0.239873 &	 1.07367 \\
4 &			 0.114482 &	 1.06715 \\


==> convRate/convRate_F6_S13 <==
Number of fluid steps= 6 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05739  &  \\
1 &			 0.886937 &	 0.253604 \\
2 &			 0.512224 &	 0.792057 \\
3 &			 0.241241 &	 1.0863 \\
4 &			 0.11318 &	 1.09186 \\


==> convRate/convRate_F6_S14 <==
Number of fluid steps= 6 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05564  &  \\
1 &			 0.882138 &	 0.259042 \\
2 &			 0.501674 &	 0.814254 \\
3 &			 0.231413 &	 1.11628 \\
4 &			 0.106829 &	 1.11517 \\


==> convRate/convRate_F6_S15 <==
Number of fluid steps= 6 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.053  &  \\
1 &			 0.874293 &	 0.268317 \\
2 &			 0.489667 &	 0.836316 \\
3 &			 0.22065 &	 1.15004 \\
4 &			 0.100417 &	 1.13576 \\


==> convRate/convRate_F6_S16 <==
Number of fluid steps= 6 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05497  &  \\
1 &			 0.87208 &	 0.27467 \\
2 &			 0.485333 &	 0.845486 \\
3 &			 0.215954 &	 1.16825 \\
4 &			 0.0959879 &	 1.1698 \\


==> convRate/convRate_F6_S17 <==
Number of fluid steps= 6 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05298  &  \\
1 &			 0.869493 &	 0.276232 \\
2 &			 0.478534 &	 0.861553 \\
3 &			 0.209245 &	 1.19343 \\
4 &			 0.0913981 &	 1.19496 \\


==> convRate/convRate_F6_S18 <==
Number of fluid steps= 6 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04895  &  \\
1 &			 0.852426 &	 0.299299 \\
2 &			 0.460449 &	 0.888533 \\
3 &			 0.196261 &	 1.23027 \\
4 &			 0.0840326 &	 1.22375 \\


==> convRate/convRate_F6_S19 <==
Number of fluid steps= 6 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05182  &  \\
1 &			 0.858539 &	 0.292932 \\
2 &			 0.467573 &	 0.876692 \\
3 &			 0.199032 &	 1.23219 \\
4 &			 0.0843018 &	 1.23937 \\


==> convRate/convRate_F6_S2 <==
Number of fluid steps= 6 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02031  &  \\
1 &			 1.05256 &	 -0.0448949 \\
2 &			 1.09785 &	 -0.0607785 \\


==> convRate/convRate_F6_S20 <==
Number of fluid steps= 6 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05054  &  \\
1 &			 0.855848 &	 0.295705 \\
2 &			 0.461185 &	 0.892009 \\
3 &			 0.193264 &	 1.25477 \\
4 &			 0.0803398 &	 1.26639 \\


==> convRate/convRate_F6_S3 <==
Number of fluid steps= 6 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03601  &  \\
1 &			 1.07879 &	 -0.0583761 \\
2 &			 1.10607 &	 -0.0360286 \\
3 &			 1.14948 &	 -0.0555387 \\
4 &			 1.23161 &	 -0.0995641 \\


==> convRate/convRate_F6_S4 <==
Number of fluid steps= 6 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05237  &  \\
1 &			 1.08074 &	 -0.0383775 \\
2 &			 1.02742 &	 0.0729934 \\
3 &			 0.97809 &	 0.0709869 \\
4 &			 0.997721 &	 -0.0286692 \\


==> convRate/convRate_F6_S5 <==
Number of fluid steps= 6 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07728  &  \\
1 &			 1.04434 &	 0.0448018 \\
2 &			 0.855717 &	 0.287386 \\
3 &			 0.67063 &	 0.351617 \\
4 &			 0.584997 &	 0.197088 \\


==> convRate/convRate_F6_S6 <==
Number of fluid steps= 6 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0599  &  \\
1 &			 0.936833 &	 0.178064 \\
2 &			 0.610213 &	 0.618479 \\
3 &			 0.352485 &	 0.791751 \\
4 &			 0.19803 &	 0.831843 \\


==> convRate/convRate_F6_S7 <==
Number of fluid steps= 6 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06246  &  \\
1 &			 0.943095 &	 0.171934 \\
2 &			 0.61465 &	 0.617638 \\
3 &			 0.347383 &	 0.823238 \\
4 &			 0.190639 &	 0.865684 \\


==> convRate/convRate_F6_S8 <==
Number of fluid steps= 6 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06001  &  \\
1 &			 0.932106 &	 0.185512 \\
2 &			 0.591838 &	 0.655292 \\
3 &			 0.32538 &	 0.863077 \\
4 &			 0.178121 &	 0.869268 \\


==> convRate/convRate_F6_S9 <==
Number of fluid steps= 6 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05828  &  \\
1 &			 0.917873 &	 0.205355 \\
2 &			 0.566563 &	 0.696058 \\
3 &			 0.301053 &	 0.912219 \\
4 &			 0.163456 &	 0.881115 \\


==> convRate/convRate_F7_S1 <==
Number of fluid steps= 7 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01965 &	 -0.028074 \\
2 &			 1.04234 &	 -0.0317519 \\


==> convRate/convRate_F7_S10 <==
Number of fluid steps= 7 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04132  &  \\
1 &			 0.85731 &	 0.280525 \\
2 &			 0.516389 &	 0.731359 \\
3 &			 0.276037 &	 0.903597 \\
4 &			 0.14954 &	 0.88433 \\


==> convRate/convRate_F7_S11 <==
Number of fluid steps= 7 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04072  &  \\
1 &			 0.844419 &	 0.301551 \\
2 &			 0.498466 &	 0.760464 \\
3 &			 0.257799 &	 0.951248 \\
4 &			 0.133972 &	 0.944315 \\


==> convRate/convRate_F7_S12 <==
Number of fluid steps= 7 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03817  &  \\
1 &			 0.834026 &	 0.315878 \\
2 &			 0.482387 &	 0.789901 \\
3 &			 0.242281 &	 0.99351 \\
4 &			 0.120704 &	 1.00521 \\


==> convRate/convRate_F7_S13 <==
Number of fluid steps= 7 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03319  &  \\
1 &			 0.824216 &	 0.326011 \\
2 &			 0.465121 &	 0.825416 \\
3 &			 0.226727 &	 1.03665 \\
4 &			 0.110134 &	 1.0417 \\


==> convRate/convRate_F7_S14 <==
Number of fluid steps= 7 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02457  &  \\
1 &			 0.799182 &	 0.358423 \\
2 &			 0.439299 &	 0.863321 \\
3 &			 0.207542 &	 1.0818 \\
4 &			 0.0986901 &	 1.07243 \\


==> convRate/convRate_F7_S15 <==
Number of fluid steps= 7 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02921  &  \\
1 &			 0.806631 &	 0.351557 \\
2 &			 0.44617 &	 0.854315 \\
3 &			 0.208989 &	 1.09417 \\
4 &			 0.0979118 &	 1.09387 \\


==> convRate/convRate_F7_S16 <==
Number of fluid steps= 7 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02692  &  \\
1 &			 0.804454 &	 0.352242 \\
2 &			 0.439236 &	 0.873014 \\
3 &			 0.202332 &	 1.11827 \\
4 &			 0.0934962 &	 1.11374 \\


==> convRate/convRate_F7_S17 <==
Number of fluid steps= 7 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02512  &  \\
1 &			 0.799361 &	 0.358874 \\
2 &			 0.430694 &	 0.892184 \\
3 &			 0.194558 &	 1.14646 \\
4 &			 0.0888379 &	 1.13095 \\


==> convRate/convRate_F7_S18 <==
Number of fluid steps= 7 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0251  &  \\
1 &			 0.792998 &	 0.370376 \\
2 &			 0.423794 &	 0.903954 \\
3 &			 0.188397 &	 1.16959 \\
4 &			 0.0843845 &	 1.15873 \\


==> convRate/convRate_F7_S19 <==
Number of fluid steps= 7 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0228  &  \\
1 &			 0.78797 &	 0.376311 \\
2 &			 0.417303 &	 0.917045 \\
3 &			 0.18334 &	 1.18657 \\
4 &			 0.0809267 &	 1.17983 \\


==> convRate/convRate_F7_S2 <==
Number of fluid steps= 7 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01765  &  \\
1 &			 1.05003 &	 -0.0451891 \\
2 &			 1.09381 &	 -0.0589316 \\


==> convRate/convRate_F7_S20 <==
Number of fluid steps= 7 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01881  &  \\
1 &			 0.783267 &	 0.379309 \\
2 &			 0.409321 &	 0.936271 \\
3 &			 0.177077 &	 1.20886 \\
4 &			 0.077155 &	 1.19855 \\


==> convRate/convRate_F7_S3 <==
Number of fluid steps= 7 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03735  &  \\
1 &			 1.07673 &	 -0.0537538 \\
2 &			 1.12013 &	 -0.0570097 \\
3 &			 1.18074 &	 -0.0760251 \\


==> convRate/convRate_F7_S4 <==
Number of fluid steps= 7 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03771  &  \\
1 &			 1.0842 &	 -0.0632276 \\
2 &			 1.08217 &	 0.00270376 \\
3 &			 1.10884 &	 -0.0351241 \\
4 &			 1.17941 &	 -0.0890141 \\


==> convRate/convRate_F7_S5 <==
Number of fluid steps= 7 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05271  &  \\
1 &			 1.05815 &	 -0.0074361 \\
2 &			 0.9621 &	 0.137285 \\
3 &			 0.893732 &	 0.106345 \\
4 &			 0.898769 &	 -0.00810808 \\


==> convRate/convRate_F7_S6 <==
Number of fluid steps= 7 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07649  &  \\
1 &			 0.993111 &	 0.116308 \\
2 &			 0.773487 &	 0.360578 \\
3 &			 0.591086 &	 0.388009 \\
4 &			 0.509931 &	 0.213066 \\


==> convRate/convRate_F7_S7 <==
Number of fluid steps= 7 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04279  &  \\
1 &			 0.869203 &	 0.262684 \\
2 &			 0.548601 &	 0.663936 \\
3 &			 0.314582 &	 0.802321 \\
4 &			 0.174311 &	 0.851773 \\


==> convRate/convRate_F7_S8 <==
Number of fluid steps= 7 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04717  &  \\
1 &			 0.87676 &	 0.256242 \\
2 &			 0.553189 &	 0.66441 \\
3 &			 0.310839 &	 0.831605 \\
4 &			 0.16884 &	 0.880511 \\


==> convRate/convRate_F7_S9 <==
Number of fluid steps= 7 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04374  &  \\
1 &			 0.869106 &	 0.264158 \\
2 &			 0.536449 &	 0.696091 \\
3 &			 0.294655 &	 0.864414 \\
4 &			 0.159632 &	 0.884277 \\


==> convRate/convRate_F8_S1 <==
Number of fluid steps= 8 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01887 &	 -0.02697 \\
2 &			 1.03984 &	 -0.0293916 \\


==> convRate/convRate_F8_S10 <==
Number of fluid steps= 8 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01895  &  \\
1 &			 0.80946 &	 0.332052 \\
2 &			 0.490888 &	 0.721566 \\
3 &			 0.269204 &	 0.866694 \\
4 &			 0.144672 &	 0.895914 \\


==> convRate/convRate_F8_S11 <==
Number of fluid steps= 8 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01754  &  \\
1 &			 0.799794 &	 0.347385 \\
2 &			 0.475459 &	 0.750308 \\
3 &			 0.255081 &	 0.898365 \\
4 &			 0.138291 &	 0.883248 \\


==> convRate/convRate_F8_S12 <==
Number of fluid steps= 8 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01028  &  \\
1 &			 0.782251 &	 0.369052 \\
2 &			 0.454001 &	 0.784936 \\
3 &			 0.238968 &	 0.925878 \\
4 &			 0.131515 &	 0.86159 \\


==> convRate/convRate_F8_S13 <==
Number of fluid steps= 8 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00902  &  \\
1 &			 0.776755 &	 0.377423 \\
2 &			 0.443231 &	 0.809401 \\
3 &			 0.224949 &	 0.978461 \\
4 &			 0.113794 &	 0.983173 \\


==> convRate/convRate_F8_S14 <==
Number of fluid steps= 8 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00388  &  \\
1 &			 0.763551 &	 0.39479 \\
2 &			 0.427351 &	 0.837303 \\
3 &			 0.211638 &	 1.01382 \\
4 &			 0.103972 &	 1.0254 \\


==> convRate/convRate_F8_S15 <==
Number of fluid steps= 8 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.998593  &  \\
1 &			 0.755253 &	 0.402937 \\
2 &			 0.413551 &	 0.868895 \\
3 &			 0.199521 &	 1.05152 \\
4 &			 0.0958871 &	 1.05713 \\


==> convRate/convRate_F8_S16 <==
Number of fluid steps= 8 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.987522  &  \\
1 &			 0.731477 &	 0.433 \\
2 &			 0.391347 &	 0.902364 \\
3 &			 0.183871 &	 1.08975 \\
4 &			 0.0868258 &	 1.0825 \\


==> convRate/convRate_F8_S17 <==
Number of fluid steps= 8 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.993457  &  \\
1 &			 0.738946 &	 0.426989 \\
2 &			 0.39762 &	 0.894079 \\
3 &			 0.185292 &	 1.10159 \\
4 &			 0.0863575 &	 1.10141 \\


==> convRate/convRate_F8_S18 <==
Number of fluid steps= 8 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.990056  &  \\
1 &			 0.735552 &	 0.428683 \\
2 &			 0.390743 &	 0.912607 \\
3 &			 0.179697 &	 1.12065 \\
4 &			 0.0829082 &	 1.11598 \\


==> convRate/convRate_F8_S19 <==
Number of fluid steps= 8 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.99006  &  \\
1 &			 0.732067 &	 0.43554 \\
2 &			 0.384982 &	 0.927185 \\
3 &			 0.174051 &	 1.14528 \\
4 &			 0.0795047 &	 1.1304 \\


==> convRate/convRate_F8_S2 <==
Number of fluid steps= 8 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01878  &  \\
1 &			 1.04724 &	 -0.0397496 \\
2 &			 1.08842 &	 -0.0556433 \\


==> convRate/convRate_F8_S20 <==
Number of fluid steps= 8 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.985187  &  \\
1 &			 0.722586 &	 0.447228 \\
2 &			 0.374185 &	 0.949418 \\
3 &			 0.166389 &	 1.16919 \\
4 &			 0.0760942 &	 1.1287 \\


==> convRate/convRate_F8_S3 <==
Number of fluid steps= 8 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0269  &  \\
1 &			 1.07348 &	 -0.0639996 \\
2 &			 1.12402 &	 -0.0663724 \\


==> convRate/convRate_F8_S4 <==
Number of fluid steps= 8 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04524  &  \\
1 &			 1.08116 &	 -0.0487458 \\
2 &			 1.11035 &	 -0.0384345 \\
3 &			 1.177 &	 -0.0840998 \\
4 &			 1.26551 &	 -0.104605 \\


==> convRate/convRate_F8_S5 <==
Number of fluid steps= 8 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05521  &  \\
1 &			 1.06809 &	 -0.0175031 \\
2 &			 1.03722 &	 0.0423113 \\
3 &			 1.04772 &	 -0.0145313 \\
4 &			 1.10469 &	 -0.0763884 \\


==> convRate/convRate_F8_S6 <==
Number of fluid steps= 8 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05713  &  \\
1 &			 1.01612 &	 0.057082 \\
2 &			 0.891119 &	 0.189381 \\
3 &			 0.812554 &	 0.133154 \\
4 &			 0.809252 &	 0.00587467 \\


==> convRate/convRate_F8_S7 <==
Number of fluid steps= 8 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06373  &  \\
1 &			 0.93844 &	 0.180796 \\
2 &			 0.704147 &	 0.414388 \\
3 &			 0.527677 &	 0.416222 \\
4 &			 0.451291 &	 0.225597 \\


==> convRate/convRate_F8_S8 <==
Number of fluid steps= 8 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01772  &  \\
1 &			 0.809936 &	 0.329461 \\
2 &			 0.501699 &	 0.690986 \\
3 &			 0.285094 &	 0.815384 \\
4 &			 0.15578 &	 0.871928 \\


==> convRate/convRate_F8_S9 <==
Number of fluid steps= 8 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0239  &  \\
1 &			 0.818104 &	 0.323719 \\
2 &			 0.506067 &	 0.692956 \\
3 &			 0.282242 &	 0.842396 \\
4 &			 0.151569 &	 0.896958 \\


==> convRate/convRate_F9_S1 <==
Number of fluid steps= 9 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01814 &	 -0.025936 \\
2 &			 1.03756 &	 -0.0272588 \\


==> convRate/convRate_F9_S10 <==
Number of fluid steps= 9 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.996409  &  \\
1 &			 0.768494 &	 0.374704 \\
2 &			 0.468876 &	 0.712828 \\
3 &			 0.259112 &	 0.855631 \\
4 &			 0.137533 &	 0.913798 \\


==> convRate/convRate_F9_S11 <==
Number of fluid steps= 9 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.991487  &  \\
1 &			 0.762557 &	 0.378749 \\
2 &			 0.457204 &	 0.738007 \\
3 &			 0.248886 &	 0.877353 \\
4 &			 0.131965 &	 0.91533 \\


==> convRate/convRate_F9_S12 <==
Number of fluid steps= 9 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98659  &  \\
1 &			 0.749421 &	 0.396674 \\
2 &			 0.441076 &	 0.764749 \\
3 &			 0.237173 &	 0.895087 \\
4 &			 0.129151 &	 0.876881 \\


==> convRate/convRate_F9_S13 <==
Number of fluid steps= 9 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98338  &  \\
1 &			 0.741018 &	 0.40824 \\
2 &			 0.427115 &	 0.794884 \\
3 &			 0.224538 &	 0.927665 \\
4 &			 0.122399 &	 0.875368 \\


==> convRate/convRate_F9_S14 <==
Number of fluid steps= 9 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98049  &  \\
1 &			 0.729277 &	 0.427036 \\
2 &			 0.413536 &	 0.818454 \\
3 &			 0.211498 &	 0.967369 \\
4 &			 0.11066 &	 0.93451 \\


==> convRate/convRate_F9_S15 <==
Number of fluid steps= 9 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.971526  &  \\
1 &			 0.716279 &	 0.439731 \\
2 &			 0.398958 &	 0.844285 \\
3 &			 0.199503 &	 0.999826 \\
4 &			 0.0990307 &	 1.01046 \\


==> convRate/convRate_F9_S16 <==
Number of fluid steps= 9 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.969115  &  \\
1 &			 0.70819 &	 0.452531 \\
2 &			 0.387807 &	 0.868798 \\
3 &			 0.189252 &	 1.03503 \\
4 &			 0.0915005 &	 1.04846 \\


==> convRate/convRate_F9_S17 <==
Number of fluid steps= 9 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.96114  &  \\
1 &			 0.698301 &	 0.460898 \\
2 &			 0.374302 &	 0.899646 \\
3 &			 0.178719 &	 1.06651 \\
4 &			 0.0849134 &	 1.07363 \\


==> convRate/convRate_F9_S18 <==
Number of fluid steps= 9 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.94899  &  \\
1 &			 0.676658 &	 0.487966 \\
2 &			 0.355242 &	 0.929625 \\
3 &			 0.165752 &	 1.09978 \\
4 &			 0.0775627 &	 1.09559 \\


==> convRate/convRate_F9_S19 <==
Number of fluid steps= 9 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.955776  &  \\
1 &			 0.683869 &	 0.482953 \\
2 &			 0.360918 &	 0.922049 \\
3 &			 0.167108 &	 1.11089 \\
4 &			 0.077289 &	 1.11245 \\


==> convRate/convRate_F9_S2 <==
Number of fluid steps= 9 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01704  &  \\
1 &			 1.04519 &	 -0.0393888 \\
2 &			 1.32409 &	 -0.341236 \\


==> convRate/convRate_F9_S20 <==
Number of fluid steps= 9 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.952715  &  \\
1 &			 0.682102 &	 0.482057 \\
2 &			 0.356073 &	 0.937814 \\
3 &			 0.16303 &	 1.12704 \\
4 &			 0.074695 &	 1.12605 \\


==> convRate/convRate_F9_S3 <==
Number of fluid steps= 9 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03108  &  \\
1 &			 1.06959 &	 -0.0529016 \\
2 &			 1.12214 &	 -0.0691948 \\


==> convRate/convRate_F9_S4 <==
Number of fluid steps= 9 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04951  &  \\
1 &			 1.08339 &	 -0.0458368 \\
2 &			 1.13211 &	 -0.0634615 \\
3 &			 1.94209 &	 -0.778596 \\


==> convRate/convRate_F9_S5 <==
Number of fluid steps= 9 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04145  &  \\
1 &			 1.07542 &	 -0.0463066 \\
2 &			 1.08836 &	 -0.0172556 \\
3 &			 1.14597 &	 -0.0744134 \\
4 &			 1.22691 &	 -0.0984601 \\


==> convRate/convRate_F9_S6 <==
Number of fluid steps= 9 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0521  &  \\
1 &			 1.03536 &	 0.0231393 \\
2 &			 0.981247 &	 0.0774442 \\
3 &			 0.97915 &	 0.00308645 \\
4 &			 1.02478 &	 -0.0657124 \\


==> convRate/convRate_F9_S7 <==
Number of fluid steps= 9 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0431  &  \\
1 &			 0.974984 &	 0.097427 \\
2 &			 0.830433 &	 0.231515 \\
3 &			 0.745298 &	 0.156046 \\
4 &			 0.735287 &	 0.0195099 \\


==> convRate/convRate_F9_S8 <==
Number of fluid steps= 9 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04248  &  \\
1 &			 0.886163 &	 0.234376 \\
2 &			 0.64617 &	 0.455658 \\
3 &			 0.476324 &	 0.439971 \\
4 &			 0.40443 &	 0.236053 \\


==> convRate/convRate_F9_S9 <==
Number of fluid steps= 9 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988738  &  \\
1 &			 0.760213 &	 0.379185 \\
2 &			 0.464844 &	 0.709657 \\
3 &			 0.261343 &	 0.830802 \\
4 &			 0.140871 &	 0.89157 \\


==> jagged_time_step/convRate/convRateAll0-4 <==

Number of fluid steps= 1 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02579 &	 -0.0367354 \\
2 &			 1.07106 &	 -0.0623039 \\
3 &			 1.08424 &	 -0.0176448 \\
4 &			 0.805303 &	 0.429081 \\
Number of fluid steps= 1 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02893 &	 -0.0411448 \\
2 &			 1.0859 &	 -0.0777464 \\
3 &			 1.08077 &	 0.00683172 \\
4 &			 0.725089 &	 0.57583 \\
Number of fluid steps= 1 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03021 &	 -0.0429384 \\
2 &			 1.09474 &	 -0.0876498 \\
3 &			 1.07887 &	 0.0210672 \\
4 &			 0.691975 &	 0.640729 \\
Number of fluid steps= 1 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03107 &	 -0.0441423 \\
2 &			 1.10104 &	 -0.0947246 \\
3 &			 1.07801 &	 0.0304963 \\
4 &			 0.674954 &	 0.675509 \\
Number of fluid steps= 1 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03185 &	 -0.0452333 \\
2 &			 1.10574 &	 -0.0997789 \\
3 &			 1.07764 &	 0.0371369 \\
4 &			 0.664974 &	 0.696505 \\
Number of fluid steps= 1 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03265 &	 -0.0463514 \\
2 &			 1.10936 &	 -0.103376 \\
3 &			 1.07749 &	 0.0420531 \\
4 &			 0.658577 &	 0.71025 \\
Number of fluid steps= 1 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03349 &	 -0.0475244 \\
2 &			 1.11221 &	 -0.105905 \\
3 &			 1.07747 &	 0.0457815 \\
4 &			 0.654208 &	 0.719826 \\
Number of fluid steps= 1 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03437 &	 -0.0487523 \\
2 &			 1.11452 &	 -0.10767 \\
3 &			 1.0775 &	 0.0487346 \\
4 &			 0.651074 &	 0.726794 \\
Number of fluid steps= 1 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03529 &	 -0.0500349 \\
2 &			 1.11643 &	 -0.108858 \\
3 &			 1.07757 &	 0.0511112 \\
4 &			 0.648741 &	 0.732067 \\
Number of fluid steps= 1 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03624 &	 -0.0513582 \\
2 &			 1.11802 &	 -0.109588 \\
3 &			 1.07765 &	 0.0530573 \\
4 &			 0.64695 &	 0.736163 \\
Number of fluid steps= 1 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03723 &	 -0.0527358 \\
2 &			 1.11937 &	 -0.109951 \\
3 &			 1.07774 &	 0.0546778 \\
4 &			 0.64554 &	 0.739431 \\
Number of fluid steps= 1 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03824 &	 -0.05414 \\
2 &			 1.12052 &	 -0.110028 \\
3 &			 1.07782 &	 0.0560521 \\
4 &			 0.644406 &	 0.742074 \\
Number of fluid steps= 1 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03927 &	 -0.0555705 \\
2 &			 1.12152 &	 -0.109885 \\
3 &			 1.07791 &	 0.0572186 \\
4 &			 0.64348 &	 0.74427 \\
Number of fluid steps= 1 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04032 &	 -0.0570274 \\
2 &			 1.12239 &	 -0.109547 \\
3 &			 1.07799 &	 0.0582303 \\
4 &			 0.64271 &	 0.746104 \\
Number of fluid steps= 1 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04139 &	 -0.0585105 \\
2 &			 1.12316 &	 -0.109053 \\
3 &			 1.07807 &	 0.0591126 \\
4 &			 0.642062 &	 0.747666 \\
Number of fluid steps= 1 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04247 &	 -0.0600059 \\
2 &			 1.12384 &	 -0.108431 \\
3 &			 1.07815 &	 0.0598787 \\
4 &			 0.641511 &	 0.749012 \\
Number of fluid steps= 1 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04356 &	 -0.0615136 \\
2 &			 1.12444 &	 -0.107693 \\
3 &			 1.07822 &	 0.0605551 \\
4 &			 0.641037 &	 0.750172 \\
Number of fluid steps= 1 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04465 &	 -0.0630197 \\
2 &			 1.12499 &	 -0.106893 \\
3 &			 1.07829 &	 0.0611669 \\
4 &			 0.640627 &	 0.751189 \\
Number of fluid steps= 1 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04575 &	 -0.064538 \\
2 &			 1.12548 &	 -0.106002 \\
3 &			 1.07835 &	 0.0617149 \\
4 &			 0.640267 &	 0.75208 \\
Number of fluid steps= 1 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04684 &	 -0.066041 \\
2 &			 1.12592 &	 -0.105063 \\
3 &			 1.07841 &	 0.0621985 \\
4 &			 0.639951 &	 0.752872 \\
Number of fluid steps= 2 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0247 &	 -0.0352016 \\
2 &			 1.06366 &	 -0.0538355 \\
3 &			 1.10668 &	 -0.0572011 \\
4 &			 1.12766 &	 -0.027094 \\
Number of fluid steps= 2 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02422  &  \\
1 &			 1.06849 &	 -0.0610478 \\
2 &			 1.08069 &	 -0.0163793 \\
3 &			 0.805655 &	 0.423719 \\
4 &			 0.471993 &	 0.771397 \\
Number of fluid steps= 2 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02415  &  \\
1 &			 1.0694 &	 -0.0623745 \\
2 &			 1.07651 &	 -0.00956014 \\
3 &			 0.773582 &	 0.476736 \\
4 &			 0.418724 &	 0.885555 \\
Number of fluid steps= 2 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0271  &  \\
1 &			 1.08208 &	 -0.0752305 \\
2 &			 1.07524 &	 0.00914845 \\
3 &			 0.725441 &	 0.567729 \\
4 &			 0.352577 &	 1.04092 \\
Number of fluid steps= 2 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02708  &  \\
1 &			 1.08129 &	 -0.0742049 \\
2 &			 1.07299 &	 0.0111169 \\
3 &			 0.715412 &	 0.58479 \\
4 &			 0.333159 &	 1.10256 \\
Number of fluid steps= 2 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0283  &  \\
1 &			 1.09005 &	 -0.0841331 \\
2 &			 1.07201 &	 0.0240759 \\
3 &			 0.692031 &	 0.63141 \\
4 &			 0.305358 &	 1.18034 \\
Number of fluid steps= 2 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02844  &  \\
1 &			 1.08872 &	 -0.0821753 \\
2 &			 1.07082 &	 0.023917 \\
3 &			 0.688582 &	 0.637016 \\
4 &			 0.296455 &	 1.21582 \\
Number of fluid steps= 2 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02914  &  \\
1 &			 1.09565 &	 -0.0903478 \\
2 &			 1.07019 &	 0.0339201 \\
3 &			 0.674684 &	 0.665583 \\
4 &			 0.281762 &	 1.25973 \\
Number of fluid steps= 2 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02937  &  \\
1 &			 1.09407 &	 -0.0879434 \\
2 &			 1.06966 &	 0.0325527 \\
3 &			 0.673907 &	 0.666531 \\
4 &			 0.277339 &	 1.2809 \\
Number of fluid steps= 2 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02989  &  \\
1 &			 1.09978 &	 -0.0947247 \\
2 &			 1.0691 &	 0.0408182 \\
3 &			 0.664408 &	 0.686255 \\
4 &			 0.268271 &	 1.30838 \\
Number of fluid steps= 2 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03022  &  \\
1 &			 1.09814 &	 -0.0921095 \\
2 &			 1.06899 &	 0.0388136 \\
3 &			 0.664884 &	 0.685074 \\
4 &			 0.266073 &	 1.32128 \\
Number of fluid steps= 2 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03067  &  \\
1 &			 1.10291 &	 -0.0977326 \\
2 &			 1.0684 &	 0.0458632 \\
3 &			 0.657758 &	 0.699823 \\
4 &			 0.259827 &	 1.34001 \\
Number of fluid steps= 2 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03107  &  \\
1 &			 1.10134 &	 -0.0951176 \\
2 &			 1.06858 &	 0.043565 \\
3 &			 0.658866 &	 0.697638 \\
4 &			 0.258842 &	 1.34791 \\
Number of fluid steps= 2 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03148  &  \\
1 &			 1.10535 &	 -0.0997874 \\
2 &			 1.06793 &	 0.0496862 \\
3 &			 0.653173 &	 0.70928 \\
4 &			 0.254184 &	 1.36159 \\
Number of fluid steps= 2 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03196  &  \\
1 &			 1.10392 &	 -0.0972486 \\
2 &			 1.06829 &	 0.0473323 \\
3 &			 0.654607 &	 0.706602 \\
4 &			 0.253901 &	 1.36636 \\
Number of fluid steps= 2 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03233  &  \\
1 &			 1.10731 &	 -0.101155 \\
2 &			 1.0676 &	 0.052688 \\
3 &			 0.649855 &	 0.716181 \\
4 &			 0.250218 &	 1.37693 \\
Number of fluid steps= 2 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03288  &  \\
1 &			 1.10602 &	 -0.0987048 \\
2 &			 1.06809 &	 0.0503443 \\
3 &			 0.651454 &	 0.713298 \\
4 &			 0.25036 &	 1.37966 \\
Number of fluid steps= 2 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03322  &  \\
1 &			 1.10891 &	 -0.101995 \\
2 &			 1.06736 &	 0.0550954 \\
3 &			 0.647364 &	 0.721398 \\
4 &			 0.247319 &	 1.3882 \\
Number of fluid steps= 2 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03384  &  \\
1 &			 1.10777 &	 -0.0996454 \\
2 &			 1.06794 &	 0.0528278 \\
3 &			 0.649039 &	 0.718454 \\
4 &			 0.247726 &	 1.38956 \\
Number of fluid steps= 2 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03414  &  \\
1 &			 1.11024 &	 -0.10244 \\
2 &			 1.06719 &	 0.0570545 \\
3 &			 0.645436 &	 0.725471 \\
4 &			 0.245132 &	 1.39672 \\
Number of fluid steps= 3 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02354 &	 -0.0335675 \\
2 &			 1.05762 &	 -0.0472539 \\
3 &			 1.10304 &	 -0.0606637 \\
Number of fluid steps= 3 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01313  &  \\
1 &			 1.06469 &	 -0.0716141 \\
2 &			 1.09962 &	 -0.0465716 \\
3 &			 1.03727 &	 0.0842136 \\
4 &			 0.981679 &	 0.0794682 \\
Number of fluid steps= 3 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04252  &  \\
1 &			 1.09027 &	 -0.0646104 \\
2 &			 0.951307 &	 0.196703 \\
3 &			 0.596548 &	 0.673273 \\
4 &			 0.343489 &	 0.796374 \\
Number of fluid steps= 3 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04247  &  \\
1 &			 1.09073 &	 -0.0652882 \\
2 &			 0.946816 &	 0.204138 \\
3 &			 0.576965 &	 0.7146 \\
4 &			 0.315791 &	 0.869514 \\
Number of fluid steps= 3 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04502  &  \\
1 &			 1.09774 &	 -0.0710058 \\
2 &			 0.929583 &	 0.239881 \\
3 &			 0.535769 &	 0.794973 \\
4 &			 0.271903 &	 0.978519 \\
Number of fluid steps= 3 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04967  &  \\
1 &			 1.09917 &	 -0.0664787 \\
2 &			 0.900469 &	 0.287666 \\
3 &			 0.486974 &	 0.886832 \\
4 &			 0.22842 &	 1.09216 \\
Number of fluid steps= 3 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04977  &  \\
1 &			 1.10084 &	 -0.0685315 \\
2 &			 0.903779 &	 0.284563 \\
3 &			 0.483912 &	 0.901225 \\
4 &			 0.21979 &	 1.13862 \\
Number of fluid steps= 3 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05132  &  \\
1 &			 1.10445 &	 -0.0711262 \\
2 &			 0.896367 &	 0.301167 \\
3 &			 0.467804 &	 0.938185 \\
4 &			 0.204279 &	 1.19536 \\
Number of fluid steps= 3 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05397  &  \\
1 &			 1.10264 &	 -0.065128 \\
2 &			 0.877891 &	 0.328848 \\
3 &			 0.442289 &	 0.989052 \\
4 &			 0.184334 &	 1.26267 \\
Number of fluid steps= 3 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05414  &  \\
1 &			 1.10473 &	 -0.0676273 \\
2 &			 0.882649 &	 0.323782 \\
3 &			 0.443573 &	 0.992668 \\
4 &			 0.181382 &	 1.29014 \\
Number of fluid steps= 3 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05549  &  \\
1 &			 1.10699 &	 -0.0687293 \\
2 &			 0.878861 &	 0.332935 \\
3 &			 0.435511 &	 1.01293 \\
4 &			 0.174017 &	 1.32348 \\
Number of fluid steps= 3 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0574  &  \\
1 &			 1.10439 &	 -0.0627285 \\
2 &			 0.865651 &	 0.351392 \\
3 &			 0.419359 &	 1.0456 \\
4 &			 0.16257 &	 1.36712 \\
Number of fluid steps= 3 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05758  &  \\
1 &			 1.10652 &	 -0.0652627 \\
2 &			 0.870541 &	 0.346045 \\
3 &			 0.422064 &	 1.04445 \\
4 &			 0.1619 &	 1.38236 \\
Number of fluid steps= 3 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05882  &  \\
1 &			 1.10809 &	 -0.0656177 \\
2 &			 0.86837 &	 0.351693 \\
3 &			 0.417401 &	 1.05688 \\
4 &			 0.157817 &	 1.40318 \\
Number of fluid steps= 3 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06032  &  \\
1 &			 1.10536 &	 -0.0600166 \\
2 &			 0.858139 &	 0.365233 \\
3 &			 0.405899 &	 1.08009 \\
4 &			 0.150262 &	 1.43364 \\
Number of fluid steps= 3 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0605  &  \\
1 &			 1.10742 &	 -0.0624579 \\
2 &			 0.862815 &	 0.360079 \\
3 &			 0.409059 &	 1.07674 \\
4 &			 0.150632 &	 1.44128 \\
Number of fluid steps= 3 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06164  &  \\
1 &			 1.1086 &	 -0.0624443 \\
2 &			 0.861475 &	 0.363858 \\
3 &			 0.406094 &	 1.085 \\
4 &			 0.148135 &	 1.4549 \\
Number of fluid steps= 3 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06287  &  \\
1 &			 1.10596 &	 -0.0573341 \\
2 &			 0.853126 &	 0.374468 \\
3 &			 0.397253 &	 1.1027 \\
4 &			 0.142653 &	 1.47755 \\
Number of fluid steps= 3 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06303  &  \\
1 &			 1.1079 &	 -0.0596454 \\
2 &			 0.857502 &	 0.369616 \\
3 &			 0.4005 &	 1.09834 \\
4 &			 0.143526 &	 1.48049 \\
Number of fluid steps= 3 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06407  &  \\
1 &			 1.10884 &	 -0.0594581 \\
2 &			 0.856635 &	 0.372299 \\
3 &			 0.398485 &	 1.10416 \\
4 &			 0.141888 &	 1.48977 \\
Number of fluid steps= 4 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02244 &	 -0.0320162 \\
2 &			 1.05271 &	 -0.0420919 \\
3 &			 1.09311 &	 -0.0543305 \\
Number of fluid steps= 4 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02211  &  \\
1 &			 1.05944 &	 -0.0517514 \\
2 &			 1.10144 &	 -0.056089 \\
3 &			 1.12424 &	 -0.0295591 \\
4 &			 1.18376 &	 -0.0744266 \\
Number of fluid steps= 4 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04061  &  \\
1 &			 1.08993 &	 -0.066806 \\
2 &			 1.04319 &	 0.0632335 \\
3 &			 0.897305 &	 0.217332 \\
4 &			 0.814145 &	 0.140313 \\
Number of fluid steps= 4 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05847  &  \\
1 &			 1.06556 &	 -0.00963145 \\
2 &			 0.806965 &	 0.401034 \\
3 &			 0.477817 &	 0.756048 \\
4 &			 0.274237 &	 0.801035 \\
Number of fluid steps= 4 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05869  &  \\
1 &			 1.06748 &	 -0.0119288 \\
2 &			 0.807415 &	 0.402827 \\
3 &			 0.466344 &	 0.791916 \\
4 &			 0.258064 &	 0.853666 \\
Number of fluid steps= 4 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0591  &  \\
1 &			 1.06043 &	 -0.00181058 \\
2 &			 0.775891 &	 0.450723 \\
3 &			 0.425638 &	 0.866227 \\
4 &			 0.227285 &	 0.905124 \\
Number of fluid steps= 4 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0639  &  \\
1 &			 1.06385 &	 6.78038e-05 \\
2 &			 0.761163 &	 0.483017 \\
3 &			 0.39875 &	 0.932721 \\
4 &			 0.198898 &	 1.00346 \\
Number of fluid steps= 4 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06753  &  \\
1 &			 1.0523 &	 0.0207306 \\
2 &			 0.726742 &	 0.534031 \\
3 &			 0.360135 &	 1.01291 \\
4 &			 0.170355 &	 1.07999 \\
Number of fluid steps= 4 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.068  &  \\
1 &			 1.05601 &	 0.0162882 \\
2 &			 0.733139 &	 0.526465 \\
3 &			 0.360068 &	 1.02582 \\
4 &			 0.166162 &	 1.11568 \\
Number of fluid steps= 4 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06685  &  \\
1 &			 1.05 &	 0.022968 \\
2 &			 0.71699 &	 0.550364 \\
3 &			 0.341163 &	 1.07149 \\
4 &			 0.152242 &	 1.16409 \\
Number of fluid steps= 4 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07054  &  \\
1 &			 1.05348 &	 0.0231758 \\
2 &			 0.713385 &	 0.56241 \\
3 &			 0.333678 &	 1.09622 \\
4 &			 0.144971 &	 1.20269 \\
Number of fluid steps= 4 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07245  &  \\
1 &			 1.04401 &	 0.0387749 \\
2 &			 0.692166 &	 0.592946 \\
3 &			 0.313105 &	 1.14447 \\
4 &			 0.131393 &	 1.25276 \\
Number of fluid steps= 4 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07295  &  \\
1 &			 1.04768 &	 0.0343847 \\
2 &			 0.699036 &	 0.583759 \\
3 &			 0.31579 &	 1.1464 \\
4 &			 0.130557 &	 1.27429 \\
Number of fluid steps= 4 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07127  &  \\
1 &			 1.04302 &	 0.0385553 \\
2 &			 0.688734 &	 0.598748 \\
3 &			 0.30437 &	 1.17812 \\
4 &			 0.121974 &	 1.31925 \\
Number of fluid steps= 4 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0744  &  \\
1 &			 1.0464 &	 0.0380968 \\
2 &			 0.68863 &	 0.603634 \\
3 &			 0.302521 &	 1.18669 \\
4 &			 0.120325 &	 1.3301 \\
Number of fluid steps= 4 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07566  &  \\
1 &			 1.03863 &	 0.0505403 \\
2 &			 0.673546 &	 0.624833 \\
3 &			 0.289224 &	 1.21959 \\
4 &			 0.112203 &	 1.36608 \\
Number of fluid steps= 4 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07617  &  \\
1 &			 1.042 &	 0.0465507 \\
2 &			 0.680021 &	 0.615704 \\
3 &			 0.292655 &	 1.21638 \\
4 &			 0.112658 &	 1.37725 \\
Number of fluid steps= 4 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07423  &  \\
1 &			 1.03834 &	 0.049024 \\
2 &			 0.672678 &	 0.626291 \\
3 &			 0.284841 &	 1.23976 \\
4 &			 0.1067 &	 1.4166 \\
Number of fluid steps= 4 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07694  &  \\
1 &			 1.04147 &	 0.0483166 \\
2 &			 0.67379 &	 0.62825 \\
3 &			 0.284958 &	 1.24155 \\
4 &			 0.106918 &	 1.41424 \\
Number of fluid steps= 4 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07784  &  \\
1 &			 1.0349 &	 0.0586517 \\
2 &			 0.662125 &	 0.644316 \\
3 &			 0.275323 &	 1.26598 \\
4 &			 0.101352 &	 1.44175 \\
Number of fluid steps= 5 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02143 &	 -0.0305903 \\
2 &			 1.04866 &	 -0.0379567 \\
Number of fluid steps= 5 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01738  &  \\
1 &			 1.05626 &	 -0.0541064 \\
2 &			 1.10178 &	 -0.0608712 \\
3 &			 1.15591 &	 -0.0691929 \\
Number of fluid steps= 5 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02705  &  \\
1 &			 1.08496 &	 -0.0791354 \\
2 &			 1.0859 &	 -0.0012494 \\
3 &			 1.0672 &	 0.0250607 \\
4 &			 1.10536 &	 -0.0506857 \\
Number of fluid steps= 5 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06455  &  \\
1 &			 1.08133 &	 -0.0225632 \\
2 &			 0.949449 &	 0.187644 \\
3 &			 0.771417 &	 0.29958 \\
4 &			 0.683357 &	 0.174871 \\
Number of fluid steps= 5 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06545  &  \\
1 &			 1.00699 &	 0.0814135 \\
2 &			 0.693507 &	 0.538067 \\
3 &			 0.403654 &	 0.780791 \\
4 &			 0.229625 &	 0.813839 \\
Number of fluid steps= 5 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06652  &  \\
1 &			 1.01123 &	 0.0767999 \\
2 &			 0.696872 &	 0.537146 \\
3 &			 0.396303 &	 0.81429 \\
4 &			 0.219097 &	 0.855034 \\
Number of fluid steps= 5 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06569  &  \\
1 &			 1.00365 &	 0.0865316 \\
2 &			 0.672788 &	 0.577032 \\
3 &			 0.368056 &	 0.870227 \\
4 &			 0.199518 &	 0.883406 \\
Number of fluid steps= 5 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06848  &  \\
1 &			 0.995372 &	 0.102252 \\
2 &			 0.650266 &	 0.614206 \\
3 &			 0.340737 &	 0.932371 \\
4 &			 0.175954 &	 0.95346 \\
Number of fluid steps= 5 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07032  &  \\
1 &			 0.989864 &	 0.11274 \\
2 &			 0.630087 &	 0.651679 \\
3 &			 0.317005 &	 0.991045 \\
4 &			 0.15679 &	 1.01567 \\
Number of fluid steps= 5 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0701  &  \\
1 &			 0.969327 &	 0.14269 \\
2 &			 0.596856 &	 0.699601 \\
3 &			 0.286723 &	 1.05773 \\
4 &			 0.136658 &	 1.06909 \\
Number of fluid steps= 5 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07161  &  \\
1 &			 0.97506 &	 0.136217 \\
2 &			 0.60425 &	 0.690345 \\
3 &			 0.287735 &	 1.0704 \\
4 &			 0.1344 &	 1.09821 \\
Number of fluid steps= 5 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07029  &  \\
1 &			 0.971898 &	 0.139125 \\
2 &			 0.593959 &	 0.710442 \\
3 &			 0.275873 &	 1.10636 \\
4 &			 0.125772 &	 1.13319 \\
Number of fluid steps= 5 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07208  &  \\
1 &			 0.967564 &	 0.147984 \\
2 &			 0.584823 &	 0.726357 \\
3 &			 0.26601 &	 1.13652 \\
4 &			 0.118319 &	 1.1688 \\
Number of fluid steps= 5 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0723  &  \\
1 &			 0.964902 &	 0.152254 \\
2 &			 0.575995 &	 0.744326 \\
3 &			 0.257087 &	 1.1638 \\
4 &			 0.11213 &	 1.19708 \\
Number of fluid steps= 5 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0712  &  \\
1 &			 0.949946 &	 0.17331 \\
2 &			 0.555675 &	 0.773604 \\
3 &			 0.24079 &	 1.20647 \\
4 &			 0.102342 &	 1.23438 \\
Number of fluid steps= 5 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07271  &  \\
1 &			 0.95523 &	 0.16734 \\
2 &			 0.56305 &	 0.762585 \\
3 &			 0.243703 &	 1.20814 \\
4 &			 0.102293 &	 1.25242 \\
Number of fluid steps= 5 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07146  &  \\
1 &			 0.953827 &	 0.167778 \\
2 &			 0.557335 &	 0.775183 \\
3 &			 0.23713 &	 1.23287 \\
4 &			 0.097206 &	 1.28656 \\
Number of fluid steps= 5 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07296  &  \\
1 &			 0.951244 &	 0.173709 \\
2 &			 0.552622 &	 0.783522 \\
3 &			 0.232373 &	 1.24985 \\
4 &			 0.0938374 &	 1.30821 \\
Number of fluid steps= 5 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07249  &  \\
1 &			 0.949995 &	 0.174972 \\
2 &			 0.548008 &	 0.793723 \\
3 &			 0.228281 &	 1.26339 \\
4 &			 0.0914663 &	 1.3195 \\
Number of fluid steps= 5 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07122  &  \\
1 &			 0.938306 &	 0.191124 \\
2 &			 0.533577 &	 0.814362 \\
3 &			 0.217592 &	 1.29407 \\
4 &			 0.0854429 &	 1.34859 \\
Number of fluid steps= 6 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0205 &	 -0.0292762 \\
2 &			 1.04525 &	 -0.0345719 \\
Number of fluid steps= 6 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02031  &  \\
1 &			 1.05256 &	 -0.0448949 \\
2 &			 1.09785 &	 -0.0607785 \\
Number of fluid steps= 6 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03601  &  \\
1 &			 1.07879 &	 -0.0583761 \\
2 &			 1.10607 &	 -0.0360286 \\
3 &			 1.14948 &	 -0.0555387 \\
4 &			 1.23161 &	 -0.0995641 \\
Number of fluid steps= 6 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05237  &  \\
1 &			 1.08074 &	 -0.0383775 \\
2 &			 1.02742 &	 0.0729934 \\
3 &			 0.97809 &	 0.0709869 \\
4 &			 0.997721 &	 -0.0286692 \\
Number of fluid steps= 6 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07728  &  \\
1 &			 1.04434 &	 0.0448018 \\
2 &			 0.855717 &	 0.287386 \\
3 &			 0.67063 &	 0.351617 \\
4 &			 0.584997 &	 0.197088 \\
Number of fluid steps= 6 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0599  &  \\
1 &			 0.936833 &	 0.178064 \\
2 &			 0.610213 &	 0.618479 \\
3 &			 0.352485 &	 0.791751 \\
4 &			 0.19803 &	 0.831843 \\
Number of fluid steps= 6 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06246  &  \\
1 &			 0.943095 &	 0.171934 \\
2 &			 0.61465 &	 0.617638 \\
3 &			 0.347383 &	 0.823238 \\
4 &			 0.190639 &	 0.865684 \\
Number of fluid steps= 6 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06001  &  \\
1 &			 0.932106 &	 0.185512 \\
2 &			 0.591838 &	 0.655292 \\
3 &			 0.32538 &	 0.863077 \\
4 &			 0.178121 &	 0.869268 \\
Number of fluid steps= 6 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05828  &  \\
1 &			 0.917873 &	 0.205355 \\
2 &			 0.566563 &	 0.696058 \\
3 &			 0.301053 &	 0.912219 \\
4 &			 0.163456 &	 0.881115 \\
Number of fluid steps= 6 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06056  &  \\
1 &			 0.9112 &	 0.218987 \\
2 &			 0.551638 &	 0.724046 \\
3 &			 0.282331 &	 0.966334 \\
4 &			 0.143288 &	 0.97847 \\
Number of fluid steps= 6 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05914  &  \\
1 &			 0.904431 &	 0.227811 \\
2 &			 0.5346 &	 0.758551 \\
3 &			 0.263789 &	 1.01908 \\
4 &			 0.129376 &	 1.02781 \\
Number of fluid steps= 6 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05435  &  \\
1 &			 0.879988 &	 0.260798 \\
2 &			 0.504881 &	 0.80154 \\
3 &			 0.239873 &	 1.07367 \\
4 &			 0.114482 &	 1.06715 \\
Number of fluid steps= 6 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05739  &  \\
1 &			 0.886937 &	 0.253604 \\
2 &			 0.512224 &	 0.792057 \\
3 &			 0.241241 &	 1.0863 \\
4 &			 0.11318 &	 1.09186 \\
Number of fluid steps= 6 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05564  &  \\
1 &			 0.882138 &	 0.259042 \\
2 &			 0.501674 &	 0.814254 \\
3 &			 0.231413 &	 1.11628 \\
4 &			 0.106829 &	 1.11517 \\
Number of fluid steps= 6 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.053  &  \\
1 &			 0.874293 &	 0.268317 \\
2 &			 0.489667 &	 0.836316 \\
3 &			 0.22065 &	 1.15004 \\
4 &			 0.100417 &	 1.13576 \\
Number of fluid steps= 6 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05497  &  \\
1 &			 0.87208 &	 0.27467 \\
2 &			 0.485333 &	 0.845486 \\
3 &			 0.215954 &	 1.16825 \\
4 &			 0.0959879 &	 1.1698 \\
Number of fluid steps= 6 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05298  &  \\
1 &			 0.869493 &	 0.276232 \\
2 &			 0.478534 &	 0.861553 \\
3 &			 0.209245 &	 1.19343 \\
4 &			 0.0913981 &	 1.19496 \\
Number of fluid steps= 6 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04895  &  \\
1 &			 0.852426 &	 0.299299 \\
2 &			 0.460449 &	 0.888533 \\
3 &			 0.196261 &	 1.23027 \\
4 &			 0.0840326 &	 1.22375 \\
Number of fluid steps= 6 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05182  &  \\
1 &			 0.858539 &	 0.292932 \\
2 &			 0.467573 &	 0.876692 \\
3 &			 0.199032 &	 1.23219 \\
4 &			 0.0843018 &	 1.23937 \\
Number of fluid steps= 6 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05054  &  \\
1 &			 0.855848 &	 0.295705 \\
2 &			 0.461185 &	 0.892009 \\
3 &			 0.193264 &	 1.25477 \\
4 &			 0.0803398 &	 1.26639 \\
Number of fluid steps= 7 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01965 &	 -0.028074 \\
2 &			 1.04234 &	 -0.0317519 \\
Number of fluid steps= 7 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01765  &  \\
1 &			 1.05003 &	 -0.0451891 \\
2 &			 1.09381 &	 -0.0589316 \\
Number of fluid steps= 7 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03735  &  \\
1 &			 1.07673 &	 -0.0537538 \\
2 &			 1.12013 &	 -0.0570097 \\
3 &			 1.18074 &	 -0.0760251 \\
Number of fluid steps= 7 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03771  &  \\
1 &			 1.0842 &	 -0.0632276 \\
2 &			 1.08217 &	 0.00270376 \\
3 &			 1.10884 &	 -0.0351241 \\
4 &			 1.17941 &	 -0.0890141 \\
Number of fluid steps= 7 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05271  &  \\
1 &			 1.05815 &	 -0.0074361 \\
2 &			 0.9621 &	 0.137285 \\
3 &			 0.893732 &	 0.106345 \\
4 &			 0.898769 &	 -0.00810808 \\
Number of fluid steps= 7 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07649  &  \\
1 &			 0.993111 &	 0.116308 \\
2 &			 0.773487 &	 0.360578 \\
3 &			 0.591086 &	 0.388009 \\
4 &			 0.509931 &	 0.213066 \\
Number of fluid steps= 7 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04279  &  \\
1 &			 0.869203 &	 0.262684 \\
2 &			 0.548601 &	 0.663936 \\
3 &			 0.314582 &	 0.802321 \\
4 &			 0.174311 &	 0.851773 \\
Number of fluid steps= 7 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04717  &  \\
1 &			 0.87676 &	 0.256242 \\
2 &			 0.553189 &	 0.66441 \\
3 &			 0.310839 &	 0.831605 \\
4 &			 0.16884 &	 0.880511 \\
Number of fluid steps= 7 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04374  &  \\
1 &			 0.869106 &	 0.264158 \\
2 &			 0.536449 &	 0.696091 \\
3 &			 0.294655 &	 0.864414 \\
4 &			 0.159632 &	 0.884277 \\
Number of fluid steps= 7 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04132  &  \\
1 &			 0.85731 &	 0.280525 \\
2 &			 0.516389 &	 0.731359 \\
3 &			 0.276037 &	 0.903597 \\
4 &			 0.14954 &	 0.88433 \\
Number of fluid steps= 7 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04072  &  \\
1 &			 0.844419 &	 0.301551 \\
2 &			 0.498466 &	 0.760464 \\
3 &			 0.257799 &	 0.951248 \\
4 &			 0.133972 &	 0.944315 \\
Number of fluid steps= 7 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03817  &  \\
1 &			 0.834026 &	 0.315878 \\
2 &			 0.482387 &	 0.789901 \\
3 &			 0.242281 &	 0.99351 \\
4 &			 0.120704 &	 1.00521 \\
Number of fluid steps= 7 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03319  &  \\
1 &			 0.824216 &	 0.326011 \\
2 &			 0.465121 &	 0.825416 \\
3 &			 0.226727 &	 1.03665 \\
4 &			 0.110134 &	 1.0417 \\
Number of fluid steps= 7 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02457  &  \\
1 &			 0.799182 &	 0.358423 \\
2 &			 0.439299 &	 0.863321 \\
3 &			 0.207542 &	 1.0818 \\
4 &			 0.0986901 &	 1.07243 \\
Number of fluid steps= 7 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02921  &  \\
1 &			 0.806631 &	 0.351557 \\
2 &			 0.44617 &	 0.854315 \\
3 &			 0.208989 &	 1.09417 \\
4 &			 0.0979118 &	 1.09387 \\
Number of fluid steps= 7 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02692  &  \\
1 &			 0.804454 &	 0.352242 \\
2 &			 0.439236 &	 0.873014 \\
3 &			 0.202332 &	 1.11827 \\
4 &			 0.0934962 &	 1.11374 \\
Number of fluid steps= 7 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02512  &  \\
1 &			 0.799361 &	 0.358874 \\
2 &			 0.430694 &	 0.892184 \\
3 &			 0.194558 &	 1.14646 \\
4 &			 0.0888379 &	 1.13095 \\
Number of fluid steps= 7 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0251  &  \\
1 &			 0.792998 &	 0.370376 \\
2 &			 0.423794 &	 0.903954 \\
3 &			 0.188397 &	 1.16959 \\
4 &			 0.0843845 &	 1.15873 \\
Number of fluid steps= 7 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0228  &  \\
1 &			 0.78797 &	 0.376311 \\
2 &			 0.417303 &	 0.917045 \\
3 &			 0.18334 &	 1.18657 \\
4 &			 0.0809267 &	 1.17983 \\
Number of fluid steps= 7 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01881  &  \\
1 &			 0.783267 &	 0.379309 \\
2 &			 0.409321 &	 0.936271 \\
3 &			 0.177077 &	 1.20886 \\
4 &			 0.077155 &	 1.19855 \\
Number of fluid steps= 8 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01887 &	 -0.02697 \\
2 &			 1.03984 &	 -0.0293916 \\
Number of fluid steps= 8 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01878  &  \\
1 &			 1.04724 &	 -0.0397496 \\
2 &			 1.08842 &	 -0.0556433 \\
Number of fluid steps= 8 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0269  &  \\
1 &			 1.07348 &	 -0.0639996 \\
2 &			 1.12402 &	 -0.0663724 \\
Number of fluid steps= 8 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04524  &  \\
1 &			 1.08116 &	 -0.0487458 \\
2 &			 1.11035 &	 -0.0384345 \\
3 &			 1.177 &	 -0.0840998 \\
4 &			 1.26551 &	 -0.104605 \\
Number of fluid steps= 8 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05521  &  \\
1 &			 1.06809 &	 -0.0175031 \\
2 &			 1.03722 &	 0.0423113 \\
3 &			 1.04772 &	 -0.0145313 \\
4 &			 1.10469 &	 -0.0763884 \\
Number of fluid steps= 8 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05713  &  \\
1 &			 1.01612 &	 0.057082 \\
2 &			 0.891119 &	 0.189381 \\
3 &			 0.812554 &	 0.133154 \\
4 &			 0.809252 &	 0.00587467 \\
Number of fluid steps= 8 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06373  &  \\
1 &			 0.93844 &	 0.180796 \\
2 &			 0.704147 &	 0.414388 \\
3 &			 0.527677 &	 0.416222 \\
4 &			 0.451291 &	 0.225597 \\
Number of fluid steps= 8 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01772  &  \\
1 &			 0.809936 &	 0.329461 \\
2 &			 0.501699 &	 0.690986 \\
3 &			 0.285094 &	 0.815384 \\
4 &			 0.15578 &	 0.871928 \\
Number of fluid steps= 8 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0239  &  \\
1 &			 0.818104 &	 0.323719 \\
2 &			 0.506067 &	 0.692956 \\
3 &			 0.282242 &	 0.842396 \\
4 &			 0.151569 &	 0.896958 \\
Number of fluid steps= 8 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01895  &  \\
1 &			 0.80946 &	 0.332052 \\
2 &			 0.490888 &	 0.721566 \\
3 &			 0.269204 &	 0.866694 \\
4 &			 0.144672 &	 0.895914 \\
Number of fluid steps= 8 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01754  &  \\
1 &			 0.799794 &	 0.347385 \\
2 &			 0.475459 &	 0.750308 \\
3 &			 0.255081 &	 0.898365 \\
4 &			 0.138291 &	 0.883248 \\
Number of fluid steps= 8 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01028  &  \\
1 &			 0.782251 &	 0.369052 \\
2 &			 0.454001 &	 0.784936 \\
3 &			 0.238968 &	 0.925878 \\
4 &			 0.131515 &	 0.86159 \\
Number of fluid steps= 8 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00902  &  \\
1 &			 0.776755 &	 0.377423 \\
2 &			 0.443231 &	 0.809401 \\
3 &			 0.224949 &	 0.978461 \\
4 &			 0.113794 &	 0.983173 \\
Number of fluid steps= 8 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00388  &  \\
1 &			 0.763551 &	 0.39479 \\
2 &			 0.427351 &	 0.837303 \\
3 &			 0.211638 &	 1.01382 \\
4 &			 0.103972 &	 1.0254 \\
Number of fluid steps= 8 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.998593  &  \\
1 &			 0.755253 &	 0.402937 \\
2 &			 0.413551 &	 0.868895 \\
3 &			 0.199521 &	 1.05152 \\
4 &			 0.0958871 &	 1.05713 \\
Number of fluid steps= 8 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.987522  &  \\
1 &			 0.731477 &	 0.433 \\
2 &			 0.391347 &	 0.902364 \\
3 &			 0.183871 &	 1.08975 \\
4 &			 0.0868258 &	 1.0825 \\
Number of fluid steps= 8 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.993457  &  \\
1 &			 0.738946 &	 0.426989 \\
2 &			 0.39762 &	 0.894079 \\
3 &			 0.185292 &	 1.10159 \\
4 &			 0.0863575 &	 1.10141 \\
Number of fluid steps= 8 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.990056  &  \\
1 &			 0.735552 &	 0.428683 \\
2 &			 0.390743 &	 0.912607 \\
3 &			 0.179697 &	 1.12065 \\
4 &			 0.0829082 &	 1.11598 \\
Number of fluid steps= 8 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.99006  &  \\
1 &			 0.732067 &	 0.43554 \\
2 &			 0.384982 &	 0.927185 \\
3 &			 0.174051 &	 1.14528 \\
4 &			 0.0795047 &	 1.1304 \\
Number of fluid steps= 8 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.985187  &  \\
1 &			 0.722586 &	 0.447228 \\
2 &			 0.374185 &	 0.949418 \\
3 &			 0.166389 &	 1.16919 \\
4 &			 0.0760942 &	 1.1287 \\
Number of fluid steps= 9 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01814 &	 -0.025936 \\
2 &			 1.03756 &	 -0.0272588 \\
Number of fluid steps= 9 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01704  &  \\
1 &			 1.04519 &	 -0.0393888 \\
2 &			 1.32409 &	 -0.341236 \\
Number of fluid steps= 9 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03108  &  \\
1 &			 1.06959 &	 -0.0529016 \\
2 &			 1.12214 &	 -0.0691948 \\
Number of fluid steps= 9 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04951  &  \\
1 &			 1.08339 &	 -0.0458368 \\
2 &			 1.13211 &	 -0.0634615 \\
3 &			 1.94209 &	 -0.778596 \\
Number of fluid steps= 9 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04145  &  \\
1 &			 1.07542 &	 -0.0463066 \\
2 &			 1.08836 &	 -0.0172556 \\
3 &			 1.14597 &	 -0.0744134 \\
4 &			 1.22691 &	 -0.0984601 \\
Number of fluid steps= 9 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0521  &  \\
1 &			 1.03536 &	 0.0231393 \\
2 &			 0.981247 &	 0.0774442 \\
3 &			 0.97915 &	 0.00308645 \\
4 &			 1.02478 &	 -0.0657124 \\
Number of fluid steps= 9 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0431  &  \\
1 &			 0.974984 &	 0.097427 \\
2 &			 0.830433 &	 0.231515 \\
3 &			 0.745298 &	 0.156046 \\
4 &			 0.735287 &	 0.0195099 \\
Number of fluid steps= 9 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04248  &  \\
1 &			 0.886163 &	 0.234376 \\
2 &			 0.64617 &	 0.455658 \\
3 &			 0.476324 &	 0.439971 \\
4 &			 0.40443 &	 0.236053 \\
Number of fluid steps= 9 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988738  &  \\
1 &			 0.760213 &	 0.379185 \\
2 &			 0.464844 &	 0.709657 \\
3 &			 0.261343 &	 0.830802 \\
4 &			 0.140871 &	 0.89157 \\
Number of fluid steps= 9 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.996409  &  \\
1 &			 0.768494 &	 0.374704 \\
2 &			 0.468876 &	 0.712828 \\
3 &			 0.259112 &	 0.855631 \\
4 &			 0.137533 &	 0.913798 \\
Number of fluid steps= 9 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.991487  &  \\
1 &			 0.762557 &	 0.378749 \\
2 &			 0.457204 &	 0.738007 \\
3 &			 0.248886 &	 0.877353 \\
4 &			 0.131965 &	 0.91533 \\
Number of fluid steps= 9 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98659  &  \\
1 &			 0.749421 &	 0.396674 \\
2 &			 0.441076 &	 0.764749 \\
3 &			 0.237173 &	 0.895087 \\
4 &			 0.129151 &	 0.876881 \\
Number of fluid steps= 9 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98338  &  \\
1 &			 0.741018 &	 0.40824 \\
2 &			 0.427115 &	 0.794884 \\
3 &			 0.224538 &	 0.927665 \\
4 &			 0.122399 &	 0.875368 \\
Number of fluid steps= 9 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98049  &  \\
1 &			 0.729277 &	 0.427036 \\
2 &			 0.413536 &	 0.818454 \\
3 &			 0.211498 &	 0.967369 \\
4 &			 0.11066 &	 0.93451 \\
Number of fluid steps= 9 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.971526  &  \\
1 &			 0.716279 &	 0.439731 \\
2 &			 0.398958 &	 0.844285 \\
3 &			 0.199503 &	 0.999826 \\
4 &			 0.0990307 &	 1.01046 \\
Number of fluid steps= 9 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.969115  &  \\
1 &			 0.70819 &	 0.452531 \\
2 &			 0.387807 &	 0.868798 \\
3 &			 0.189252 &	 1.03503 \\
4 &			 0.0915005 &	 1.04846 \\
Number of fluid steps= 9 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.96114  &  \\
1 &			 0.698301 &	 0.460898 \\
2 &			 0.374302 &	 0.899646 \\
3 &			 0.178719 &	 1.06651 \\
4 &			 0.0849134 &	 1.07363 \\
Number of fluid steps= 9 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.94899  &  \\
1 &			 0.676658 &	 0.487966 \\
2 &			 0.355242 &	 0.929625 \\
3 &			 0.165752 &	 1.09978 \\
4 &			 0.0775627 &	 1.09559 \\
Number of fluid steps= 9 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.955776  &  \\
1 &			 0.683869 &	 0.482953 \\
2 &			 0.360918 &	 0.922049 \\
3 &			 0.167108 &	 1.11089 \\
4 &			 0.077289 &	 1.11245 \\
Number of fluid steps= 9 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.952715  &  \\
1 &			 0.682102 &	 0.482057 \\
2 &			 0.356073 &	 0.937814 \\
3 &			 0.16303 &	 1.12704 \\
4 &			 0.074695 &	 1.12605 \\
Number of fluid steps= 10 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01747 &	 -0.0249863 \\
2 &			 1.03448 &	 -0.0239195 \\
Number of fluid steps= 10 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01747  &  \\
1 &			 1.04299 &	 -0.0357391 \\
Number of fluid steps= 10 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03229  &  \\
1 &			 1.06745 &	 -0.0483202 \\
Number of fluid steps= 10 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04127  &  \\
1 &			 1.08176 &	 -0.0550363 \\
2 &			 1.14185 &	 -0.0779927 \\
Number of fluid steps= 10 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04718  &  \\
1 &			 1.07637 &	 -0.0396646 \\
2 &			 1.11834 &	 -0.0551848 \\
3 &			 1.20162 &	 -0.103622 \\
4 &			 1.2899 &	 -0.102278 \\
Number of fluid steps= 10 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05023  &  \\
1 &			 1.05285 &	 -0.0035946 \\
2 &			 1.05043 &	 0.00331988 \\
3 &			 1.09813 &	 -0.0640688 \\
4 &			 1.16997 &	 -0.0914227 \\
Number of fluid steps= 10 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03856  &  \\
1 &			 1.00426 &	 0.0484517 \\
2 &			 0.931997 &	 0.107736 \\
3 &			 0.918279 &	 0.0213928 \\
4 &			 0.952381 &	 -0.0526063 \\
Number of fluid steps= 10 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02922  &  \\
1 &			 0.927246 &	 0.150527 \\
2 &			 0.77149 &	 0.265305 \\
3 &			 0.683711 &	 0.174261 \\
4 &			 0.670378 &	 0.0284118 \\
Number of fluid steps= 10 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01647  &  \\
1 &			 0.838747 &	 0.27726 \\
2 &			 0.597536 &	 0.48921 \\
3 &			 0.434059 &	 0.461134 \\
4 &			 0.36622 &	 0.245181 \\
Number of fluid steps= 10 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.959089  &  \\
1 &			 0.719217 &	 0.415238 \\
2 &			 0.435036 &	 0.725292 \\
3 &			 0.241714 &	 0.847834 \\
4 &			 0.128601 &	 0.910399 \\
Number of fluid steps= 10 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.967829  &  \\
1 &			 0.727302 &	 0.412198 \\
2 &			 0.438723 &	 0.729244 \\
3 &			 0.239936 &	 0.870661 \\
4 &			 0.125891 &	 0.930474 \\
Number of fluid steps= 10 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.961614  &  \\
1 &			 0.720729 &	 0.416001 \\
2 &			 0.427986 &	 0.751893 \\
3 &			 0.231341 &	 0.887543 \\
4 &			 0.12139 &	 0.930371 \\
Number of fluid steps= 10 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.959136  &  \\
1 &			 0.713101 &	 0.427629 \\
2 &			 0.416416 &	 0.776081 \\
3 &			 0.222066 &	 0.907037 \\
4 &			 0.118842 &	 0.901944 \\
Number of fluid steps= 10 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.954215  &  \\
1 &			 0.701572 &	 0.443723 \\
2 &			 0.402736 &	 0.800757 \\
3 &			 0.211865 &	 0.926689 \\
4 &			 0.115411 &	 0.876365 \\
Number of fluid steps= 10 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.94638  &  \\
1 &			 0.687342 &	 0.461391 \\
2 &			 0.387244 &	 0.827785 \\
3 &			 0.201331 &	 0.943674 \\
4 &			 0.112633 &	 0.83794 \\
Number of fluid steps= 10 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.942618  &  \\
1 &			 0.680601 &	 0.469864 \\
2 &			 0.377357 &	 0.850879 \\
3 &			 0.189333 &	 0.995004 \\
4 &			 0.0960739 &	 0.978709 \\
Number of fluid steps= 10 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.939048  &  \\
1 &			 0.671703 &	 0.483375 \\
2 &			 0.367244 &	 0.871085 \\
3 &			 0.180258 &	 1.02668 \\
4 &			 0.0876815 &	 1.03972 \\
Number of fluid steps= 10 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.931372  &  \\
1 &			 0.660522 &	 0.495751 \\
2 &			 0.354811 &	 0.896556 \\
3 &			 0.170893 &	 1.05396 \\
4 &			 0.0815292 &	 1.0677 \\
Number of fluid steps= 10 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.924888  &  \\
1 &			 0.652048 &	 0.504301 \\
2 &			 0.343674 &	 0.923937 \\
3 &			 0.162299 &	 1.08239 \\
4 &			 0.0762001 &	 1.09079 \\
Number of fluid steps= 10 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.912745  &  \\
1 &			 0.632842 &	 0.528367 \\
2 &			 0.327276 &	 0.951338 \\
3 &			 0.151401 &	 1.11213 \\
4 &			 0.0701174 &	 1.11053 \\
Number of fluid steps= 11 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01685 &	 -0.0241069 \\
2 &			 1.02658 &	 -0.0137392 \\
Number of fluid steps= 11 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01621  &  \\
1 &			 1.0413 &	 -0.0351872 \\
2 &			 76.7888 &	 -6.20444 \\
Number of fluid steps= 11 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02494  &  \\
1 &			 1.06492 &	 -0.0552056 \\
Number of fluid steps= 11 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03319  &  \\
1 &			 1.0812 &	 -0.0655278 \\
2 &			 3.3849 &	 -1.64648 \\
Number of fluid steps= 11 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05309  &  \\
1 &			 1.08309 &	 -0.0405244 \\
2 &			 1.14307 &	 -0.0777606 \\
3 &			 1.22156 &	 -0.095811 \\
Number of fluid steps= 11 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03854  &  \\
1 &			 1.06639 &	 -0.0381784 \\
2 &			 1.09936 &	 -0.0439287 \\
3 &			 1.1766 &	 -0.09796 \\
4 &			 1.25956 &	 -0.0982959 \\
Number of fluid steps= 11 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04471  &  \\
1 &			 1.0272 &	 0.0243854 \\
2 &			 1.0103 &	 0.0239334 \\
3 &			 1.04711 &	 -0.0516293 \\
4 &			 1.10858 &	 -0.0822999 \\
Number of fluid steps= 11 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02954  &  \\
1 &			 0.966671 &	 0.090903 \\
2 &			 0.880921 &	 0.134012 \\
3 &			 0.858817 &	 0.0366619 \\
4 &			 0.884628 &	 -0.0427202 \\
Number of fluid steps= 11 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00681  &  \\
1 &			 0.887464 &	 0.182031 \\
2 &			 0.723113 &	 0.295467 \\
3 &			 0.633216 &	 0.191523 \\
4 &			 0.616715 &	 0.0380938 \\
Number of fluid steps= 11 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988727  &  \\
1 &			 0.796843 &	 0.311277 \\
2 &			 0.556423 &	 0.518113 \\
3 &			 0.398747 &	 0.480708 \\
4 &			 0.334514 &	 0.253407 \\
Number of fluid steps= 11 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.930938  &  \\
1 &			 0.685526 &	 0.441474 \\
2 &			 0.410332 &	 0.74042 \\
3 &			 0.225169 &	 0.865783 \\
4 &			 0.118317 &	 0.928351 \\
Number of fluid steps= 11 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.940298  &  \\
1 &			 0.693247 &	 0.439749 \\
2 &			 0.413706 &	 0.744764 \\
3 &			 0.223735 &	 0.886815 \\
4 &			 0.116077 &	 0.946709 \\
Number of fluid steps= 11 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.934987  &  \\
1 &			 0.688349 &	 0.441806 \\
2 &			 0.405053 &	 0.76503 \\
3 &			 0.216679 &	 0.902551 \\
4 &			 0.112278 &	 0.948484 \\
Number of fluid steps= 11 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.932972  &  \\
1 &			 0.680535 &	 0.455164 \\
2 &			 0.394796 &	 0.785562 \\
3 &			 0.208923 &	 0.918136 \\
4 &			 0.110353 &	 0.920845 \\
Number of fluid steps= 11 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.929097  &  \\
1 &			 0.671495 &	 0.468453 \\
2 &			 0.383514 &	 0.808097 \\
3 &			 0.200796 &	 0.933549 \\
4 &			 0.109152 &	 0.879392 \\
Number of fluid steps= 11 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.922041  &  \\
1 &			 0.661257 &	 0.47962 \\
2 &			 0.370704 &	 0.834943 \\
3 &			 0.19149 &	 0.952999 \\
4 &			 0.10577 &	 0.856339 \\
Number of fluid steps= 11 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.918788  &  \\
1 &			 0.651984 &	 0.494895 \\
2 &			 0.360373 &	 0.855346 \\
3 &			 0.181609 &	 0.988655 \\
4 &			 0.0962007 &	 0.916716 \\
Number of fluid steps= 11 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.91093  &  \\
1 &			 0.642447 &	 0.503763 \\
2 &			 0.349654 &	 0.877649 \\
3 &			 0.172072 &	 1.02292 \\
4 &			 0.0848686 &	 1.01971 \\
Number of fluid steps= 11 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905112  &  \\
1 &			 0.633218 &	 0.515394 \\
2 &			 0.339808 &	 0.897982 \\
3 &			 0.164144 &	 1.04976 \\
4 &			 0.0785654 &	 1.063 \\
Number of fluid steps= 11 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.900334  &  \\
1 &			 0.623821 &	 0.529328 \\
2 &			 0.329904 &	 0.919086 \\
3 &			 0.156614 &	 1.07483 \\
4 &			 0.0736241 &	 1.08896 \\
Number of fluid steps= 12 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01626 &	 -0.0232695 \\
2 &			 1.01081 &	 0.00775771 \\
Number of fluid steps= 12 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01633  &  \\
1 &			 1.03951 &	 -0.0325347 \\
Number of fluid steps= 12 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02725  &  \\
1 &			 1.06208 &	 -0.0481051 \\
Number of fluid steps= 12 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0367  &  \\
1 &			 1.07847 &	 -0.0569876 \\
Number of fluid steps= 12 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04126  &  \\
1 &			 1.08518 &	 -0.059604 \\
2 &			 1.15056 &	 -0.0844019 \\
Number of fluid steps= 12 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04295  &  \\
1 &			 1.07052 &	 -0.0376418 \\
2 &			 1.12848 &	 -0.0760691 \\
3 &			 1.2225 &	 -0.115454 \\
4 &			 1.30809 &	 -0.0976273 \\
Number of fluid steps= 12 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04042  &  \\
1 &			 1.04522 &	 -0.0066406 \\
2 &			 1.06902 &	 -0.0324822 \\
3 &			 1.13895 &	 -0.0914156 \\
4 &			 1.21509 &	 -0.0933588 \\
Number of fluid steps= 12 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02666  &  \\
1 &			 0.991724 &	 0.0499479 \\
2 &			 0.963195 &	 0.0421108 \\
3 &			 0.991558 &	 -0.0418693 \\
4 &			 1.04506 &	 -0.0758167 \\
Number of fluid steps= 12 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00886  &  \\
1 &			 0.925521 &	 0.124388 \\
2 &			 0.830125 &	 0.156937 \\
3 &			 0.802394 &	 0.0490178 \\
4 &			 0.822533 &	 -0.0357627 \\
Number of fluid steps= 12 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.985703  &  \\
1 &			 0.845729 &	 0.220958 \\
2 &			 0.676972 &	 0.321099 \\
3 &			 0.586915 &	 0.205945 \\
4 &			 0.569162 &	 0.0443122 \\
Number of fluid steps= 12 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.961361  &  \\
1 &			 0.760243 &	 0.338618 \\
2 &			 0.521347 &	 0.544217 \\
3 &			 0.368847 &	 0.499221 \\
4 &			 0.30781 &	 0.260982 \\
Number of fluid steps= 12 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905489  &  \\
1 &			 0.657705 &	 0.461256 \\
2 &			 0.389443 &	 0.756028 \\
3 &			 0.211005 &	 0.884135 \\
4 &			 0.109568 &	 0.945451 \\
Number of fluid steps= 12 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.915061  &  \\
1 &			 0.664989 &	 0.460537 \\
2 &			 0.392544 &	 0.760476 \\
3 &			 0.209838 &	 0.903578 \\
4 &			 0.107687 &	 0.962432 \\
Number of fluid steps= 12 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.908666  &  \\
1 &			 0.659611 &	 0.462135 \\
2 &			 0.384459 &	 0.778786 \\
3 &			 0.203719 &	 0.916249 \\
4 &			 0.104493 &	 0.963174 \\
Number of fluid steps= 12 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905614  &  \\
1 &			 0.652037 &	 0.473942 \\
2 &			 0.375181 &	 0.797367 \\
3 &			 0.197168 &	 0.928161 \\
4 &			 0.103143 &	 0.93478 \\
Number of fluid steps= 12 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.901228  &  \\
1 &			 0.643375 &	 0.486232 \\
2 &			 0.364999 &	 0.817767 \\
3 &			 0.190855 &	 0.935416 \\
4 &			 0.10432 &	 0.871461 \\
Number of fluid steps= 12 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.899464  &  \\
1 &			 0.636632 &	 0.498606 \\
2 &			 0.355608 &	 0.840172 \\
3 &			 0.183002 &	 0.958428 \\
4 &			 0.100673 &	 0.862183 \\
Number of fluid steps= 12 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.890098  &  \\
1 &			 0.624113 &	 0.512157 \\
2 &			 0.343243 &	 0.862577 \\
3 &			 0.175868 &	 0.964737 \\
4 &			 0.100378 &	 0.80905 \\
Number of fluid steps= 12 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.887852  &  \\
1 &			 0.618843 &	 0.520746 \\
2 &			 0.335395 &	 0.883712 \\
3 &			 0.165428 &	 1.01966 \\
4 &			 0.0844785 &	 0.969547 \\
Number of fluid steps= 12 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.87936  &  \\
1 &			 0.608048 &	 0.532269 \\
2 &			 0.325365 &	 0.902126 \\
3 &			 0.157657 &	 1.04527 \\
4 &			 0.0762797 &	 1.04742 \\
Number of fluid steps= 13 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0157 &	 -0.0224743 \\
2 &			 1.0992 &	 -0.11398 \\
Number of fluid steps= 13 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01537  &  \\
1 &			 1.03808 &	 -0.0319121 \\
Number of fluid steps= 13 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02817  &  \\
1 &			 1.0601 &	 -0.0441215 \\
Number of fluid steps= 13 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03937  &  \\
1 &			 1.07767 &	 -0.0522061 \\
2 &			 156457 &	 -17.1475 \\
Number of fluid steps= 13 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04221  &  \\
1 &			 1.08601 &	 -0.0593914 \\
2 &			 9.76022 &	 -3.16788 \\
Number of fluid steps= 13 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05009  &  \\
1 &			 1.08063 &	 -0.0413597 \\
2 &			 1.15369 &	 -0.094383 \\
3 &			 4.21531 &	 -1.86938 \\
Number of fluid steps= 13 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03143  &  \\
1 &			 1.05948 &	 -0.0387104 \\
2 &			 1.11206 &	 -0.0698783 \\
3 &			 1.20156 &	 -0.111674 \\
4 &			 1.28325 &	 -0.0948936 \\
Number of fluid steps= 13 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02692  &  \\
1 &			 1.02022 &	 0.00944351 \\
2 &			 1.03455 &	 -0.0201231 \\
3 &			 1.09621 &	 -0.0835208 \\
4 &			 1.16471 &	 -0.0874466 \\
Number of fluid steps= 13 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00882  &  \\
1 &			 0.964166 &	 0.0653153 \\
2 &			 0.924486 &	 0.0606301 \\
3 &			 0.943134 &	 -0.0288113 \\
4 &			 0.987477 &	 -0.0662844 \\
Number of fluid steps= 13 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988269  &  \\
1 &			 0.893477 &	 0.145473 \\
2 &			 0.789133 &	 0.179162 \\
3 &			 0.755422 &	 0.0629857 \\
4 &			 0.769488 &	 -0.026616 \\
Number of fluid steps= 13 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.962504  &  \\
1 &			 0.812372 &	 0.244652 \\
2 &			 0.63917 &	 0.345941 \\
3 &			 0.548593 &	 0.220463 \\
4 &			 0.529267 &	 0.0517405 \\
Number of fluid steps= 13 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.935677  &  \\
1 &			 0.728404 &	 0.361272 \\
2 &			 0.491142 &	 0.568599 \\
3 &			 0.343228 &	 0.516973 \\
4 &			 0.285023 &	 0.268089 \\
Number of fluid steps= 13 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.883247  &  \\
1 &			 0.634523 &	 0.477144 \\
2 &			 0.371483 &	 0.772376 \\
3 &			 0.198724 &	 0.90253 \\
4 &			 0.102032 &	 0.961744 \\
Number of fluid steps= 13 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.892698  &  \\
1 &			 0.641355 &	 0.477049 \\
2 &			 0.374353 &	 0.776724 \\
3 &			 0.197769 &	 0.920583 \\
4 &			 0.100433 &	 0.977583 \\
Number of fluid steps= 13 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.88769  &  \\
1 &			 0.636962 &	 0.478849 \\
2 &			 0.367596 &	 0.793086 \\
3 &			 0.192581 &	 0.932656 \\
4 &			 0.0976608 &	 0.979614 \\
Number of fluid steps= 13 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.885135  &  \\
1 &			 0.630871 &	 0.488552 \\
2 &			 0.359692 &	 0.810583 \\
3 &			 0.18688 &	 0.94465 \\
4 &			 0.0962398 &	 0.957407 \\
Number of fluid steps= 13 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.881561  &  \\
1 &			 0.62366 &	 0.499301 \\
2 &			 0.350873 &	 0.829811 \\
3 &			 0.181309 &	 0.952498 \\
4 &			 0.0971324 &	 0.900426 \\
Number of fluid steps= 13 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.877876  &  \\
1 &			 0.616054 &	 0.51096 \\
2 &			 0.341971 &	 0.849183 \\
3 &			 0.175172 &	 0.965102 \\
4 &			 0.0962421 &	 0.864032 \\
Number of fluid steps= 13 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.872218  &  \\
1 &			 0.607077 &	 0.522809 \\
2 &			 0.331847 &	 0.871361 \\
3 &			 0.168436 &	 0.978318 \\
4 &			 0.094789 &	 0.829409 \\
Number of fluid steps= 13 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.86958  &  \\
1 &			 0.600155 &	 0.534984 \\
2 &			 0.323861 &	 0.88996 \\
3 &			 0.1606 &	 1.0119 \\
4 &			 0.0866142 &	 0.890796 \\
Number of fluid steps= 14 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01516 &	 -0.0217071 \\
2 &			 2.0784 &	 -1.03377 \\
Number of fluid steps= 14 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01534  &  \\
1 &			 1.03659 &	 -0.0298825 \\
Number of fluid steps= 14 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02277  &  \\
1 &			 1.05832 &	 -0.0492942 \\
Number of fluid steps= 14 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03398  &  \\
1 &			 1.07563 &	 -0.0569736 \\
Number of fluid steps= 14 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03433  &  \\
1 &			 1.08636 &	 -0.0708057 \\
Number of fluid steps= 14 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04135  &  \\
1 &			 1.08448 &	 -0.0585484 \\
2 &			 1.16076 &	 -0.0980663 \\
Number of fluid steps= 14 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03514  &  \\
1 &			 1.06575 &	 -0.0420432 \\
2 &			 1.13934 &	 -0.0963293 \\
3 &			 1.24001 &	 -0.122153 \\
4 &			 1.32212 &	 -0.0925014 \\
Number of fluid steps= 14 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02895  &  \\
1 &			 1.03801 &	 -0.0126475 \\
2 &			 1.08534 &	 -0.0643267 \\
3 &			 1.16976 &	 -0.108066 \\
4 &			 1.24671 &	 -0.0919134 \\
Number of fluid steps= 14 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01724  &  \\
1 &			 0.992953 &	 0.0348628 \\
2 &			 0.998329 &	 -0.0077899 \\
3 &			 1.05167 &	 -0.0750948 \\
4 &			 1.11263 &	 -0.0812918 \\
Number of fluid steps= 14 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.994591  &  \\
1 &			 0.930527 &	 0.0960554 \\
2 &			 0.882343 &	 0.0767084 \\
3 &			 0.893959 &	 -0.0188691 \\
4 &			 0.931804 &	 -0.0598179 \\
Number of fluid steps= 14 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.970229  &  \\
1 &			 0.86009 &	 0.173838 \\
2 &			 0.748917 &	 0.199682 \\
3 &			 0.711153 &	 0.0746459 \\
4 &			 0.721084 &	 -0.0200074 \\
Number of fluid steps= 14 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.941464  &  \\
1 &			 0.778391 &	 0.274411 \\
2 &			 0.603033 &	 0.368258 \\
3 &			 0.513078 &	 0.233059 \\
4 &			 0.493381 &	 0.056476 \\
Number of fluid steps= 14 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.91236  &  \\
1 &			 0.700693 &	 0.380821 \\
2 &			 0.4649 &	 0.591862 \\
3 &			 0.321047 &	 0.534136 \\
4 &			 0.265361 &	 0.274828 \\
Number of fluid steps= 14 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.864263  &  \\
1 &			 0.614989 &	 0.49091 \\
2 &			 0.355832 &	 0.789364 \\
3 &			 0.187963 &	 0.920748 \\
4 &			 0.0954705 &	 0.977322 \\
Number of fluid steps= 14 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.873342  &  \\
1 &			 0.621385 &	 0.491059 \\
2 &			 0.358507 &	 0.793486 \\
3 &			 0.187179 &	 0.937583 \\
4 &			 0.0940963 &	 0.992209 \\
Number of fluid steps= 14 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.867408  &  \\
1 &			 0.616659 &	 0.492238 \\
2 &			 0.35212 &	 0.808406 \\
3 &			 0.182575 &	 0.947578 \\
4 &			 0.0917029 &	 0.99345 \\
Number of fluid steps= 14 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.867234  &  \\
1 &			 0.611876 &	 0.503182 \\
2 &			 0.345718 &	 0.823644 \\
3 &			 0.177768 &	 0.9596 \\
4 &			 0.090404 &	 0.975537 \\
Number of fluid steps= 14 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.862673  &  \\
1 &			 0.605135 &	 0.511557 \\
2 &			 0.337761 &	 0.841254 \\
3 &			 0.173006 &	 0.965181 \\
4 &			 0.0914484 &	 0.919792 \\
Number of fluid steps= 14 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.861162  &  \\
1 &			 0.599081 &	 0.523534 \\
2 &			 0.330282 &	 0.859053 \\
3 &			 0.16822 &	 0.973349 \\
4 &			 0.0924786 &	 0.863158 \\
Number of fluid steps= 14 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.854726  &  \\
1 &			 0.590573 &	 0.533347 \\
2 &			 0.321171 &	 0.878774 \\
3 &			 0.162322 &	 0.984483 \\
4 &			 0.091044 &	 0.834223 \\
Number of fluid steps= 15 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01463 &	 -0.0209537 \\
Number of fluid steps= 15 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01456  &  \\
1 &			 1.03537 &	 -0.0292922 \\
Number of fluid steps= 15 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0242  &  \\
1 &			 1.05591 &	 -0.0439894 \\
Number of fluid steps= 15 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02883  &  \\
1 &			 1.07421 &	 -0.0622714 \\
Number of fluid steps= 15 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0371  &  \\
1 &			 1.08472 &	 -0.0647677 \\
Number of fluid steps= 15 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03915  &  \\
1 &			 1.08717 &	 -0.0651736 \\
2 &			 943.971 &	 -9.76202 \\
Number of fluid steps= 15 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04326  &  \\
1 &			 1.07811 &	 -0.0474056 \\
2 &			 1.16385 &	 -0.110401 \\
3 &			 1.31889 &	 -0.180419 \\
Number of fluid steps= 15 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02251  &  \\
1 &			 1.05492 &	 -0.0450186 \\
2 &			 1.12492 &	 -0.0926888 \\
3 &			 1.22203 &	 -0.119457 \\
4 &			 1.30117 &	 -0.0905298 \\
Number of fluid steps= 15 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01512  &  \\
1 &			 1.01447 &	 0.00092408 \\
2 &			 1.05521 &	 -0.0568039 \\
3 &			 1.13329 &	 -0.102987 \\
4 &			 1.20458 &	 -0.0880131 \\
Number of fluid steps= 15 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.995738  &  \\
1 &			 0.960593 &	 0.0518409 \\
2 &			 0.958117 &	 0.00372345 \\
3 &			 1.00483 &	 -0.0686777 \\
Number of fluid steps= 15 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 15 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 16 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 17 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 18 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 19 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
Number of fluid steps= 20 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv


==> jagged_time_step/convRate/convRate_F10_S1 <==
Number of fluid steps= 10 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01747 &	 -0.0249863 \\
2 &			 1.03448 &	 -0.0239195 \\


==> jagged_time_step/convRate/convRate_F10_S10 <==
Number of fluid steps= 10 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.959089  &  \\
1 &			 0.719217 &	 0.415238 \\
2 &			 0.435036 &	 0.725292 \\
3 &			 0.241714 &	 0.847834 \\
4 &			 0.128601 &	 0.910399 \\


==> jagged_time_step/convRate/convRate_F10_S11 <==
Number of fluid steps= 10 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.967829  &  \\
1 &			 0.727302 &	 0.412198 \\
2 &			 0.438723 &	 0.729244 \\
3 &			 0.239936 &	 0.870661 \\
4 &			 0.125891 &	 0.930474 \\


==> jagged_time_step/convRate/convRate_F10_S12 <==
Number of fluid steps= 10 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.961614  &  \\
1 &			 0.720729 &	 0.416001 \\
2 &			 0.427986 &	 0.751893 \\
3 &			 0.231341 &	 0.887543 \\
4 &			 0.12139 &	 0.930371 \\


==> jagged_time_step/convRate/convRate_F10_S13 <==
Number of fluid steps= 10 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.959136  &  \\
1 &			 0.713101 &	 0.427629 \\
2 &			 0.416416 &	 0.776081 \\
3 &			 0.222066 &	 0.907037 \\
4 &			 0.118842 &	 0.901944 \\


==> jagged_time_step/convRate/convRate_F10_S14 <==
Number of fluid steps= 10 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.954215  &  \\
1 &			 0.701572 &	 0.443723 \\
2 &			 0.402736 &	 0.800757 \\
3 &			 0.211865 &	 0.926689 \\
4 &			 0.115411 &	 0.876365 \\


==> jagged_time_step/convRate/convRate_F10_S15 <==
Number of fluid steps= 10 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.94638  &  \\
1 &			 0.687342 &	 0.461391 \\
2 &			 0.387244 &	 0.827785 \\
3 &			 0.201331 &	 0.943674 \\
4 &			 0.112633 &	 0.83794 \\


==> jagged_time_step/convRate/convRate_F10_S16 <==
Number of fluid steps= 10 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.942618  &  \\
1 &			 0.680601 &	 0.469864 \\
2 &			 0.377357 &	 0.850879 \\
3 &			 0.189333 &	 0.995004 \\
4 &			 0.0960739 &	 0.978709 \\


==> jagged_time_step/convRate/convRate_F10_S17 <==
Number of fluid steps= 10 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.939048  &  \\
1 &			 0.671703 &	 0.483375 \\
2 &			 0.367244 &	 0.871085 \\
3 &			 0.180258 &	 1.02668 \\
4 &			 0.0876815 &	 1.03972 \\


==> jagged_time_step/convRate/convRate_F10_S18 <==
Number of fluid steps= 10 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.931372  &  \\
1 &			 0.660522 &	 0.495751 \\
2 &			 0.354811 &	 0.896556 \\
3 &			 0.170893 &	 1.05396 \\
4 &			 0.0815292 &	 1.0677 \\


==> jagged_time_step/convRate/convRate_F10_S19 <==
Number of fluid steps= 10 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.924888  &  \\
1 &			 0.652048 &	 0.504301 \\
2 &			 0.343674 &	 0.923937 \\
3 &			 0.162299 &	 1.08239 \\
4 &			 0.0762001 &	 1.09079 \\


==> jagged_time_step/convRate/convRate_F10_S2 <==
Number of fluid steps= 10 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01747  &  \\
1 &			 1.04299 &	 -0.0357391 \\


==> jagged_time_step/convRate/convRate_F10_S20 <==
Number of fluid steps= 10 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.912745  &  \\
1 &			 0.632842 &	 0.528367 \\
2 &			 0.327276 &	 0.951338 \\
3 &			 0.151401 &	 1.11213 \\
4 &			 0.0701174 &	 1.11053 \\


==> jagged_time_step/convRate/convRate_F10_S3 <==
Number of fluid steps= 10 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03229  &  \\
1 &			 1.06745 &	 -0.0483202 \\


==> jagged_time_step/convRate/convRate_F10_S4 <==
Number of fluid steps= 10 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04127  &  \\
1 &			 1.08176 &	 -0.0550363 \\
2 &			 1.14185 &	 -0.0779927 \\


==> jagged_time_step/convRate/convRate_F10_S5 <==
Number of fluid steps= 10 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04718  &  \\
1 &			 1.07637 &	 -0.0396646 \\
2 &			 1.11834 &	 -0.0551848 \\
3 &			 1.20162 &	 -0.103622 \\
4 &			 1.2899 &	 -0.102278 \\


==> jagged_time_step/convRate/convRate_F10_S6 <==
Number of fluid steps= 10 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05023  &  \\
1 &			 1.05285 &	 -0.0035946 \\
2 &			 1.05043 &	 0.00331988 \\
3 &			 1.09813 &	 -0.0640688 \\
4 &			 1.16997 &	 -0.0914227 \\


==> jagged_time_step/convRate/convRate_F10_S7 <==
Number of fluid steps= 10 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03856  &  \\
1 &			 1.00426 &	 0.0484517 \\
2 &			 0.931997 &	 0.107736 \\
3 &			 0.918279 &	 0.0213928 \\
4 &			 0.952381 &	 -0.0526063 \\


==> jagged_time_step/convRate/convRate_F10_S8 <==
Number of fluid steps= 10 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02922  &  \\
1 &			 0.927246 &	 0.150527 \\
2 &			 0.77149 &	 0.265305 \\
3 &			 0.683711 &	 0.174261 \\
4 &			 0.670378 &	 0.0284118 \\


==> jagged_time_step/convRate/convRate_F10_S9 <==
Number of fluid steps= 10 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01647  &  \\
1 &			 0.838747 &	 0.27726 \\
2 &			 0.597536 &	 0.48921 \\
3 &			 0.434059 &	 0.461134 \\
4 &			 0.36622 &	 0.245181 \\


==> jagged_time_step/convRate/convRate_F11_S1 <==
Number of fluid steps= 11 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01685 &	 -0.0241069 \\
2 &			 1.02658 &	 -0.0137392 \\


==> jagged_time_step/convRate/convRate_F11_S10 <==
Number of fluid steps= 11 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988727  &  \\
1 &			 0.796843 &	 0.311277 \\
2 &			 0.556423 &	 0.518113 \\
3 &			 0.398747 &	 0.480708 \\
4 &			 0.334514 &	 0.253407 \\


==> jagged_time_step/convRate/convRate_F11_S11 <==
Number of fluid steps= 11 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.930938  &  \\
1 &			 0.685526 &	 0.441474 \\
2 &			 0.410332 &	 0.74042 \\
3 &			 0.225169 &	 0.865783 \\
4 &			 0.118317 &	 0.928351 \\


==> jagged_time_step/convRate/convRate_F11_S12 <==
Number of fluid steps= 11 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.940298  &  \\
1 &			 0.693247 &	 0.439749 \\
2 &			 0.413706 &	 0.744764 \\
3 &			 0.223735 &	 0.886815 \\
4 &			 0.116077 &	 0.946709 \\


==> jagged_time_step/convRate/convRate_F11_S13 <==
Number of fluid steps= 11 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.934987  &  \\
1 &			 0.688349 &	 0.441806 \\
2 &			 0.405053 &	 0.76503 \\
3 &			 0.216679 &	 0.902551 \\
4 &			 0.112278 &	 0.948484 \\


==> jagged_time_step/convRate/convRate_F11_S14 <==
Number of fluid steps= 11 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.932972  &  \\
1 &			 0.680535 &	 0.455164 \\
2 &			 0.394796 &	 0.785562 \\
3 &			 0.208923 &	 0.918136 \\
4 &			 0.110353 &	 0.920845 \\


==> jagged_time_step/convRate/convRate_F11_S15 <==
Number of fluid steps= 11 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.929097  &  \\
1 &			 0.671495 &	 0.468453 \\
2 &			 0.383514 &	 0.808097 \\
3 &			 0.200796 &	 0.933549 \\
4 &			 0.109152 &	 0.879392 \\


==> jagged_time_step/convRate/convRate_F11_S16 <==
Number of fluid steps= 11 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.922041  &  \\
1 &			 0.661257 &	 0.47962 \\
2 &			 0.370704 &	 0.834943 \\
3 &			 0.19149 &	 0.952999 \\
4 &			 0.10577 &	 0.856339 \\


==> jagged_time_step/convRate/convRate_F11_S17 <==
Number of fluid steps= 11 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.918788  &  \\
1 &			 0.651984 &	 0.494895 \\
2 &			 0.360373 &	 0.855346 \\
3 &			 0.181609 &	 0.988655 \\
4 &			 0.0962007 &	 0.916716 \\


==> jagged_time_step/convRate/convRate_F11_S18 <==
Number of fluid steps= 11 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.91093  &  \\
1 &			 0.642447 &	 0.503763 \\
2 &			 0.349654 &	 0.877649 \\
3 &			 0.172072 &	 1.02292 \\
4 &			 0.0848686 &	 1.01971 \\


==> jagged_time_step/convRate/convRate_F11_S19 <==
Number of fluid steps= 11 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905112  &  \\
1 &			 0.633218 &	 0.515394 \\
2 &			 0.339808 &	 0.897982 \\
3 &			 0.164144 &	 1.04976 \\
4 &			 0.0785654 &	 1.063 \\


==> jagged_time_step/convRate/convRate_F11_S2 <==
Number of fluid steps= 11 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01621  &  \\
1 &			 1.0413 &	 -0.0351872 \\
2 &			 76.7888 &	 -6.20444 \\


==> jagged_time_step/convRate/convRate_F11_S20 <==
Number of fluid steps= 11 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.900334  &  \\
1 &			 0.623821 &	 0.529328 \\
2 &			 0.329904 &	 0.919086 \\
3 &			 0.156614 &	 1.07483 \\
4 &			 0.0736241 &	 1.08896 \\


==> jagged_time_step/convRate/convRate_F11_S3 <==
Number of fluid steps= 11 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02494  &  \\
1 &			 1.06492 &	 -0.0552056 \\


==> jagged_time_step/convRate/convRate_F11_S4 <==
Number of fluid steps= 11 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03319  &  \\
1 &			 1.0812 &	 -0.0655278 \\
2 &			 3.3849 &	 -1.64648 \\


==> jagged_time_step/convRate/convRate_F11_S5 <==
Number of fluid steps= 11 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05309  &  \\
1 &			 1.08309 &	 -0.0405244 \\
2 &			 1.14307 &	 -0.0777606 \\
3 &			 1.22156 &	 -0.095811 \\


==> jagged_time_step/convRate/convRate_F11_S6 <==
Number of fluid steps= 11 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03854  &  \\
1 &			 1.06639 &	 -0.0381784 \\
2 &			 1.09936 &	 -0.0439287 \\
3 &			 1.1766 &	 -0.09796 \\
4 &			 1.25956 &	 -0.0982959 \\


==> jagged_time_step/convRate/convRate_F11_S7 <==
Number of fluid steps= 11 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04471  &  \\
1 &			 1.0272 &	 0.0243854 \\
2 &			 1.0103 &	 0.0239334 \\
3 &			 1.04711 &	 -0.0516293 \\
4 &			 1.10858 &	 -0.0822999 \\


==> jagged_time_step/convRate/convRate_F11_S8 <==
Number of fluid steps= 11 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02954  &  \\
1 &			 0.966671 &	 0.090903 \\
2 &			 0.880921 &	 0.134012 \\
3 &			 0.858817 &	 0.0366619 \\
4 &			 0.884628 &	 -0.0427202 \\


==> jagged_time_step/convRate/convRate_F11_S9 <==
Number of fluid steps= 11 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00681  &  \\
1 &			 0.887464 &	 0.182031 \\
2 &			 0.723113 &	 0.295467 \\
3 &			 0.633216 &	 0.191523 \\
4 &			 0.616715 &	 0.0380938 \\


==> jagged_time_step/convRate/convRate_F12_S1 <==
Number of fluid steps= 12 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01626 &	 -0.0232695 \\
2 &			 1.01081 &	 0.00775771 \\


==> jagged_time_step/convRate/convRate_F12_S10 <==
Number of fluid steps= 12 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.985703  &  \\
1 &			 0.845729 &	 0.220958 \\
2 &			 0.676972 &	 0.321099 \\
3 &			 0.586915 &	 0.205945 \\
4 &			 0.569162 &	 0.0443122 \\


==> jagged_time_step/convRate/convRate_F12_S11 <==
Number of fluid steps= 12 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.961361  &  \\
1 &			 0.760243 &	 0.338618 \\
2 &			 0.521347 &	 0.544217 \\
3 &			 0.368847 &	 0.499221 \\
4 &			 0.30781 &	 0.260982 \\


==> jagged_time_step/convRate/convRate_F12_S12 <==
Number of fluid steps= 12 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905489  &  \\
1 &			 0.657705 &	 0.461256 \\
2 &			 0.389443 &	 0.756028 \\
3 &			 0.211005 &	 0.884135 \\
4 &			 0.109568 &	 0.945451 \\


==> jagged_time_step/convRate/convRate_F12_S13 <==
Number of fluid steps= 12 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.915061  &  \\
1 &			 0.664989 &	 0.460537 \\
2 &			 0.392544 &	 0.760476 \\
3 &			 0.209838 &	 0.903578 \\
4 &			 0.107687 &	 0.962432 \\


==> jagged_time_step/convRate/convRate_F12_S14 <==
Number of fluid steps= 12 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.908666  &  \\
1 &			 0.659611 &	 0.462135 \\
2 &			 0.384459 &	 0.778786 \\
3 &			 0.203719 &	 0.916249 \\
4 &			 0.104493 &	 0.963174 \\


==> jagged_time_step/convRate/convRate_F12_S15 <==
Number of fluid steps= 12 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.905614  &  \\
1 &			 0.652037 &	 0.473942 \\
2 &			 0.375181 &	 0.797367 \\
3 &			 0.197168 &	 0.928161 \\
4 &			 0.103143 &	 0.93478 \\


==> jagged_time_step/convRate/convRate_F12_S16 <==
Number of fluid steps= 12 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.901228  &  \\
1 &			 0.643375 &	 0.486232 \\
2 &			 0.364999 &	 0.817767 \\
3 &			 0.190855 &	 0.935416 \\
4 &			 0.10432 &	 0.871461 \\


==> jagged_time_step/convRate/convRate_F12_S17 <==
Number of fluid steps= 12 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.899464  &  \\
1 &			 0.636632 &	 0.498606 \\
2 &			 0.355608 &	 0.840172 \\
3 &			 0.183002 &	 0.958428 \\
4 &			 0.100673 &	 0.862183 \\


==> jagged_time_step/convRate/convRate_F12_S18 <==
Number of fluid steps= 12 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.890098  &  \\
1 &			 0.624113 &	 0.512157 \\
2 &			 0.343243 &	 0.862577 \\
3 &			 0.175868 &	 0.964737 \\
4 &			 0.100378 &	 0.80905 \\


==> jagged_time_step/convRate/convRate_F12_S19 <==
Number of fluid steps= 12 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.887852  &  \\
1 &			 0.618843 &	 0.520746 \\
2 &			 0.335395 &	 0.883712 \\
3 &			 0.165428 &	 1.01966 \\
4 &			 0.0844785 &	 0.969547 \\


==> jagged_time_step/convRate/convRate_F12_S2 <==
Number of fluid steps= 12 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01633  &  \\
1 &			 1.03951 &	 -0.0325347 \\


==> jagged_time_step/convRate/convRate_F12_S20 <==
Number of fluid steps= 12 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.87936  &  \\
1 &			 0.608048 &	 0.532269 \\
2 &			 0.325365 &	 0.902126 \\
3 &			 0.157657 &	 1.04527 \\
4 &			 0.0762797 &	 1.04742 \\


==> jagged_time_step/convRate/convRate_F12_S3 <==
Number of fluid steps= 12 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02725  &  \\
1 &			 1.06208 &	 -0.0481051 \\


==> jagged_time_step/convRate/convRate_F12_S4 <==
Number of fluid steps= 12 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0367  &  \\
1 &			 1.07847 &	 -0.0569876 \\


==> jagged_time_step/convRate/convRate_F12_S5 <==
Number of fluid steps= 12 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04126  &  \\
1 &			 1.08518 &	 -0.059604 \\
2 &			 1.15056 &	 -0.0844019 \\


==> jagged_time_step/convRate/convRate_F12_S6 <==
Number of fluid steps= 12 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04295  &  \\
1 &			 1.07052 &	 -0.0376418 \\
2 &			 1.12848 &	 -0.0760691 \\
3 &			 1.2225 &	 -0.115454 \\
4 &			 1.30809 &	 -0.0976273 \\


==> jagged_time_step/convRate/convRate_F12_S7 <==
Number of fluid steps= 12 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04042  &  \\
1 &			 1.04522 &	 -0.0066406 \\
2 &			 1.06902 &	 -0.0324822 \\
3 &			 1.13895 &	 -0.0914156 \\
4 &			 1.21509 &	 -0.0933588 \\


==> jagged_time_step/convRate/convRate_F12_S8 <==
Number of fluid steps= 12 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02666  &  \\
1 &			 0.991724 &	 0.0499479 \\
2 &			 0.963195 &	 0.0421108 \\
3 &			 0.991558 &	 -0.0418693 \\
4 &			 1.04506 &	 -0.0758167 \\


==> jagged_time_step/convRate/convRate_F12_S9 <==
Number of fluid steps= 12 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00886  &  \\
1 &			 0.925521 &	 0.124388 \\
2 &			 0.830125 &	 0.156937 \\
3 &			 0.802394 &	 0.0490178 \\
4 &			 0.822533 &	 -0.0357627 \\


==> jagged_time_step/convRate/convRate_F13_S1 <==
Number of fluid steps= 13 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0157 &	 -0.0224743 \\
2 &			 1.0992 &	 -0.11398 \\


==> jagged_time_step/convRate/convRate_F13_S10 <==
Number of fluid steps= 13 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988269  &  \\
1 &			 0.893477 &	 0.145473 \\
2 &			 0.789133 &	 0.179162 \\
3 &			 0.755422 &	 0.0629857 \\
4 &			 0.769488 &	 -0.026616 \\


==> jagged_time_step/convRate/convRate_F13_S11 <==
Number of fluid steps= 13 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.962504  &  \\
1 &			 0.812372 &	 0.244652 \\
2 &			 0.63917 &	 0.345941 \\
3 &			 0.548593 &	 0.220463 \\
4 &			 0.529267 &	 0.0517405 \\


==> jagged_time_step/convRate/convRate_F13_S12 <==
Number of fluid steps= 13 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.935677  &  \\
1 &			 0.728404 &	 0.361272 \\
2 &			 0.491142 &	 0.568599 \\
3 &			 0.343228 &	 0.516973 \\
4 &			 0.285023 &	 0.268089 \\


==> jagged_time_step/convRate/convRate_F13_S13 <==
Number of fluid steps= 13 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.883247  &  \\
1 &			 0.634523 &	 0.477144 \\
2 &			 0.371483 &	 0.772376 \\
3 &			 0.198724 &	 0.90253 \\
4 &			 0.102032 &	 0.961744 \\


==> jagged_time_step/convRate/convRate_F13_S14 <==
Number of fluid steps= 13 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.892698  &  \\
1 &			 0.641355 &	 0.477049 \\
2 &			 0.374353 &	 0.776724 \\
3 &			 0.197769 &	 0.920583 \\
4 &			 0.100433 &	 0.977583 \\


==> jagged_time_step/convRate/convRate_F13_S15 <==
Number of fluid steps= 13 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.88769  &  \\
1 &			 0.636962 &	 0.478849 \\
2 &			 0.367596 &	 0.793086 \\
3 &			 0.192581 &	 0.932656 \\
4 &			 0.0976608 &	 0.979614 \\


==> jagged_time_step/convRate/convRate_F13_S16 <==
Number of fluid steps= 13 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.885135  &  \\
1 &			 0.630871 &	 0.488552 \\
2 &			 0.359692 &	 0.810583 \\
3 &			 0.18688 &	 0.94465 \\
4 &			 0.0962398 &	 0.957407 \\


==> jagged_time_step/convRate/convRate_F13_S17 <==
Number of fluid steps= 13 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.881561  &  \\
1 &			 0.62366 &	 0.499301 \\
2 &			 0.350873 &	 0.829811 \\
3 &			 0.181309 &	 0.952498 \\
4 &			 0.0971324 &	 0.900426 \\


==> jagged_time_step/convRate/convRate_F13_S18 <==
Number of fluid steps= 13 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.877876  &  \\
1 &			 0.616054 &	 0.51096 \\
2 &			 0.341971 &	 0.849183 \\
3 &			 0.175172 &	 0.965102 \\
4 &			 0.0962421 &	 0.864032 \\


==> jagged_time_step/convRate/convRate_F13_S19 <==
Number of fluid steps= 13 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.872218  &  \\
1 &			 0.607077 &	 0.522809 \\
2 &			 0.331847 &	 0.871361 \\
3 &			 0.168436 &	 0.978318 \\
4 &			 0.094789 &	 0.829409 \\


==> jagged_time_step/convRate/convRate_F13_S2 <==
Number of fluid steps= 13 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01537  &  \\
1 &			 1.03808 &	 -0.0319121 \\


==> jagged_time_step/convRate/convRate_F13_S20 <==
Number of fluid steps= 13 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.86958  &  \\
1 &			 0.600155 &	 0.534984 \\
2 &			 0.323861 &	 0.88996 \\
3 &			 0.1606 &	 1.0119 \\
4 &			 0.0866142 &	 0.890796 \\


==> jagged_time_step/convRate/convRate_F13_S3 <==
Number of fluid steps= 13 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02817  &  \\
1 &			 1.0601 &	 -0.0441215 \\


==> jagged_time_step/convRate/convRate_F13_S4 <==
Number of fluid steps= 13 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03937  &  \\
1 &			 1.07767 &	 -0.0522061 \\
2 &			 156457 &	 -17.1475 \\


==> jagged_time_step/convRate/convRate_F13_S5 <==
Number of fluid steps= 13 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04221  &  \\
1 &			 1.08601 &	 -0.0593914 \\
2 &			 9.76022 &	 -3.16788 \\


==> jagged_time_step/convRate/convRate_F13_S6 <==
Number of fluid steps= 13 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05009  &  \\
1 &			 1.08063 &	 -0.0413597 \\
2 &			 1.15369 &	 -0.094383 \\
3 &			 4.21531 &	 -1.86938 \\


==> jagged_time_step/convRate/convRate_F13_S7 <==
Number of fluid steps= 13 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03143  &  \\
1 &			 1.05948 &	 -0.0387104 \\
2 &			 1.11206 &	 -0.0698783 \\
3 &			 1.20156 &	 -0.111674 \\
4 &			 1.28325 &	 -0.0948936 \\


==> jagged_time_step/convRate/convRate_F13_S8 <==
Number of fluid steps= 13 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02692  &  \\
1 &			 1.02022 &	 0.00944351 \\
2 &			 1.03455 &	 -0.0201231 \\
3 &			 1.09621 &	 -0.0835208 \\
4 &			 1.16471 &	 -0.0874466 \\


==> jagged_time_step/convRate/convRate_F13_S9 <==
Number of fluid steps= 13 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00882  &  \\
1 &			 0.964166 &	 0.0653153 \\
2 &			 0.924486 &	 0.0606301 \\
3 &			 0.943134 &	 -0.0288113 \\
4 &			 0.987477 &	 -0.0662844 \\


==> jagged_time_step/convRate/convRate_F14_S1 <==
Number of fluid steps= 14 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01516 &	 -0.0217071 \\
2 &			 2.0784 &	 -1.03377 \\


==> jagged_time_step/convRate/convRate_F14_S10 <==
Number of fluid steps= 14 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.994591  &  \\
1 &			 0.930527 &	 0.0960554 \\
2 &			 0.882343 &	 0.0767084 \\
3 &			 0.893959 &	 -0.0188691 \\
4 &			 0.931804 &	 -0.0598179 \\


==> jagged_time_step/convRate/convRate_F14_S11 <==
Number of fluid steps= 14 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.970229  &  \\
1 &			 0.86009 &	 0.173838 \\
2 &			 0.748917 &	 0.199682 \\
3 &			 0.711153 &	 0.0746459 \\
4 &			 0.721084 &	 -0.0200074 \\


==> jagged_time_step/convRate/convRate_F14_S12 <==
Number of fluid steps= 14 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.941464  &  \\
1 &			 0.778391 &	 0.274411 \\
2 &			 0.603033 &	 0.368258 \\
3 &			 0.513078 &	 0.233059 \\
4 &			 0.493381 &	 0.056476 \\


==> jagged_time_step/convRate/convRate_F14_S13 <==
Number of fluid steps= 14 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.91236  &  \\
1 &			 0.700693 &	 0.380821 \\
2 &			 0.4649 &	 0.591862 \\
3 &			 0.321047 &	 0.534136 \\
4 &			 0.265361 &	 0.274828 \\


==> jagged_time_step/convRate/convRate_F14_S14 <==
Number of fluid steps= 14 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.864263  &  \\
1 &			 0.614989 &	 0.49091 \\
2 &			 0.355832 &	 0.789364 \\
3 &			 0.187963 &	 0.920748 \\
4 &			 0.0954705 &	 0.977322 \\


==> jagged_time_step/convRate/convRate_F14_S15 <==
Number of fluid steps= 14 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.873342  &  \\
1 &			 0.621385 &	 0.491059 \\
2 &			 0.358507 &	 0.793486 \\
3 &			 0.187179 &	 0.937583 \\
4 &			 0.0940963 &	 0.992209 \\


==> jagged_time_step/convRate/convRate_F14_S16 <==
Number of fluid steps= 14 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.867408  &  \\
1 &			 0.616659 &	 0.492238 \\
2 &			 0.35212 &	 0.808406 \\
3 &			 0.182575 &	 0.947578 \\
4 &			 0.0917029 &	 0.99345 \\


==> jagged_time_step/convRate/convRate_F14_S17 <==
Number of fluid steps= 14 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.867234  &  \\
1 &			 0.611876 &	 0.503182 \\
2 &			 0.345718 &	 0.823644 \\
3 &			 0.177768 &	 0.9596 \\
4 &			 0.090404 &	 0.975537 \\


==> jagged_time_step/convRate/convRate_F14_S18 <==
Number of fluid steps= 14 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.862673  &  \\
1 &			 0.605135 &	 0.511557 \\
2 &			 0.337761 &	 0.841254 \\
3 &			 0.173006 &	 0.965181 \\
4 &			 0.0914484 &	 0.919792 \\


==> jagged_time_step/convRate/convRate_F14_S19 <==
Number of fluid steps= 14 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.861162  &  \\
1 &			 0.599081 &	 0.523534 \\
2 &			 0.330282 &	 0.859053 \\
3 &			 0.16822 &	 0.973349 \\
4 &			 0.0924786 &	 0.863158 \\


==> jagged_time_step/convRate/convRate_F14_S2 <==
Number of fluid steps= 14 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01534  &  \\
1 &			 1.03659 &	 -0.0298825 \\


==> jagged_time_step/convRate/convRate_F14_S20 <==
Number of fluid steps= 14 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.854726  &  \\
1 &			 0.590573 &	 0.533347 \\
2 &			 0.321171 &	 0.878774 \\
3 &			 0.162322 &	 0.984483 \\
4 &			 0.091044 &	 0.834223 \\


==> jagged_time_step/convRate/convRate_F14_S3 <==
Number of fluid steps= 14 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02277  &  \\
1 &			 1.05832 &	 -0.0492942 \\


==> jagged_time_step/convRate/convRate_F14_S4 <==
Number of fluid steps= 14 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03398  &  \\
1 &			 1.07563 &	 -0.0569736 \\


==> jagged_time_step/convRate/convRate_F14_S5 <==
Number of fluid steps= 14 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03433  &  \\
1 &			 1.08636 &	 -0.0708057 \\


==> jagged_time_step/convRate/convRate_F14_S6 <==
Number of fluid steps= 14 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04135  &  \\
1 &			 1.08448 &	 -0.0585484 \\
2 &			 1.16076 &	 -0.0980663 \\


==> jagged_time_step/convRate/convRate_F14_S7 <==
Number of fluid steps= 14 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03514  &  \\
1 &			 1.06575 &	 -0.0420432 \\
2 &			 1.13934 &	 -0.0963293 \\
3 &			 1.24001 &	 -0.122153 \\
4 &			 1.32212 &	 -0.0925014 \\


==> jagged_time_step/convRate/convRate_F14_S8 <==
Number of fluid steps= 14 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02895  &  \\
1 &			 1.03801 &	 -0.0126475 \\
2 &			 1.08534 &	 -0.0643267 \\
3 &			 1.16976 &	 -0.108066 \\
4 &			 1.24671 &	 -0.0919134 \\


==> jagged_time_step/convRate/convRate_F14_S9 <==
Number of fluid steps= 14 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01724  &  \\
1 &			 0.992953 &	 0.0348628 \\
2 &			 0.998329 &	 -0.0077899 \\
3 &			 1.05167 &	 -0.0750948 \\
4 &			 1.11263 &	 -0.0812918 \\


==> jagged_time_step/convRate/convRate_F15_S1 <==
Number of fluid steps= 15 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01463 &	 -0.0209537 \\


==> jagged_time_step/convRate/convRate_F15_S10 <==
Number of fluid steps= 15 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.995738  &  \\
1 &			 0.960593 &	 0.0518409 \\
2 &			 0.958117 &	 0.00372345 \\
3 &			 1.00483 &	 -0.0686777 \\


==> jagged_time_step/convRate/convRate_F15_S2 <==
Number of fluid steps= 15 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01456  &  \\
1 &			 1.03537 &	 -0.0292922 \\


==> jagged_time_step/convRate/convRate_F15_S3 <==
Number of fluid steps= 15 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0242  &  \\
1 &			 1.05591 &	 -0.0439894 \\


==> jagged_time_step/convRate/convRate_F15_S4 <==
Number of fluid steps= 15 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02883  &  \\
1 &			 1.07421 &	 -0.0622714 \\


==> jagged_time_step/convRate/convRate_F15_S5 <==
Number of fluid steps= 15 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0371  &  \\
1 &			 1.08472 &	 -0.0647677 \\


==> jagged_time_step/convRate/convRate_F15_S6 <==
Number of fluid steps= 15 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03915  &  \\
1 &			 1.08717 &	 -0.0651736 \\
2 &			 943.971 &	 -9.76202 \\


==> jagged_time_step/convRate/convRate_F15_S7 <==
Number of fluid steps= 15 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04326  &  \\
1 &			 1.07811 &	 -0.0474056 \\
2 &			 1.16385 &	 -0.110401 \\
3 &			 1.31889 &	 -0.180419 \\


==> jagged_time_step/convRate/convRate_F15_S8 <==
Number of fluid steps= 15 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02251  &  \\
1 &			 1.05492 &	 -0.0450186 \\
2 &			 1.12492 &	 -0.0926888 \\
3 &			 1.22203 &	 -0.119457 \\
4 &			 1.30117 &	 -0.0905298 \\


==> jagged_time_step/convRate/convRate_F15_S9 <==
Number of fluid steps= 15 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01512  &  \\
1 &			 1.01447 &	 0.00092408 \\
2 &			 1.05521 &	 -0.0568039 \\
3 &			 1.13329 &	 -0.102987 \\
4 &			 1.20458 &	 -0.0880131 \\


==> jagged_time_step/convRate/convRate_F1_S1 <==
Number of fluid steps= 1 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02579 &	 -0.0367354 \\
2 &			 1.07106 &	 -0.0623039 \\
3 &			 1.08424 &	 -0.0176448 \\
4 &			 0.805303 &	 0.429081 \\


==> jagged_time_step/convRate/convRate_F1_S10 <==
Number of fluid steps= 1 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03624 &	 -0.0513582 \\
2 &			 1.11802 &	 -0.109588 \\
3 &			 1.07765 &	 0.0530573 \\
4 &			 0.64695 &	 0.736163 \\


==> jagged_time_step/convRate/convRate_F1_S11 <==
Number of fluid steps= 1 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03723 &	 -0.0527358 \\
2 &			 1.11937 &	 -0.109951 \\
3 &			 1.07774 &	 0.0546778 \\
4 &			 0.64554 &	 0.739431 \\


==> jagged_time_step/convRate/convRate_F1_S12 <==
Number of fluid steps= 1 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03824 &	 -0.05414 \\
2 &			 1.12052 &	 -0.110028 \\
3 &			 1.07782 &	 0.0560521 \\
4 &			 0.644406 &	 0.742074 \\


==> jagged_time_step/convRate/convRate_F1_S13 <==
Number of fluid steps= 1 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03927 &	 -0.0555705 \\
2 &			 1.12152 &	 -0.109885 \\
3 &			 1.07791 &	 0.0572186 \\
4 &			 0.64348 &	 0.74427 \\


==> jagged_time_step/convRate/convRate_F1_S14 <==
Number of fluid steps= 1 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04032 &	 -0.0570274 \\
2 &			 1.12239 &	 -0.109547 \\
3 &			 1.07799 &	 0.0582303 \\
4 &			 0.64271 &	 0.746104 \\


==> jagged_time_step/convRate/convRate_F1_S15 <==
Number of fluid steps= 1 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04139 &	 -0.0585105 \\
2 &			 1.12316 &	 -0.109053 \\
3 &			 1.07807 &	 0.0591126 \\
4 &			 0.642062 &	 0.747666 \\


==> jagged_time_step/convRate/convRate_F1_S16 <==
Number of fluid steps= 1 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04247 &	 -0.0600059 \\
2 &			 1.12384 &	 -0.108431 \\
3 &			 1.07815 &	 0.0598787 \\
4 &			 0.641511 &	 0.749012 \\


==> jagged_time_step/convRate/convRate_F1_S17 <==
Number of fluid steps= 1 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04356 &	 -0.0615136 \\
2 &			 1.12444 &	 -0.107693 \\
3 &			 1.07822 &	 0.0605551 \\
4 &			 0.641037 &	 0.750172 \\


==> jagged_time_step/convRate/convRate_F1_S18 <==
Number of fluid steps= 1 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04465 &	 -0.0630197 \\
2 &			 1.12499 &	 -0.106893 \\
3 &			 1.07829 &	 0.0611669 \\
4 &			 0.640627 &	 0.751189 \\


==> jagged_time_step/convRate/convRate_F1_S19 <==
Number of fluid steps= 1 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04575 &	 -0.064538 \\
2 &			 1.12548 &	 -0.106002 \\
3 &			 1.07835 &	 0.0617149 \\
4 &			 0.640267 &	 0.75208 \\


==> jagged_time_step/convRate/convRate_F1_S2 <==
Number of fluid steps= 1 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02893 &	 -0.0411448 \\
2 &			 1.0859 &	 -0.0777464 \\
3 &			 1.08077 &	 0.00683172 \\
4 &			 0.725089 &	 0.57583 \\


==> jagged_time_step/convRate/convRate_F1_S20 <==
Number of fluid steps= 1 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.04684 &	 -0.066041 \\
2 &			 1.12592 &	 -0.105063 \\
3 &			 1.07841 &	 0.0621985 \\
4 &			 0.639951 &	 0.752872 \\


==> jagged_time_step/convRate/convRate_F1_S3 <==
Number of fluid steps= 1 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03021 &	 -0.0429384 \\
2 &			 1.09474 &	 -0.0876498 \\
3 &			 1.07887 &	 0.0210672 \\
4 &			 0.691975 &	 0.640729 \\


==> jagged_time_step/convRate/convRate_F1_S4 <==
Number of fluid steps= 1 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03107 &	 -0.0441423 \\
2 &			 1.10104 &	 -0.0947246 \\
3 &			 1.07801 &	 0.0304963 \\
4 &			 0.674954 &	 0.675509 \\


==> jagged_time_step/convRate/convRate_F1_S5 <==
Number of fluid steps= 1 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03185 &	 -0.0452333 \\
2 &			 1.10574 &	 -0.0997789 \\
3 &			 1.07764 &	 0.0371369 \\
4 &			 0.664974 &	 0.696505 \\


==> jagged_time_step/convRate/convRate_F1_S6 <==
Number of fluid steps= 1 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03265 &	 -0.0463514 \\
2 &			 1.10936 &	 -0.103376 \\
3 &			 1.07749 &	 0.0420531 \\
4 &			 0.658577 &	 0.71025 \\


==> jagged_time_step/convRate/convRate_F1_S7 <==
Number of fluid steps= 1 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03349 &	 -0.0475244 \\
2 &			 1.11221 &	 -0.105905 \\
3 &			 1.07747 &	 0.0457815 \\
4 &			 0.654208 &	 0.719826 \\


==> jagged_time_step/convRate/convRate_F1_S8 <==
Number of fluid steps= 1 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03437 &	 -0.0487523 \\
2 &			 1.11452 &	 -0.10767 \\
3 &			 1.0775 &	 0.0487346 \\
4 &			 0.651074 &	 0.726794 \\


==> jagged_time_step/convRate/convRate_F1_S9 <==
Number of fluid steps= 1 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.03529 &	 -0.0500349 \\
2 &			 1.11643 &	 -0.108858 \\
3 &			 1.07757 &	 0.0511112 \\
4 &			 0.648741 &	 0.732067 \\


==> jagged_time_step/convRate/convRate_F2_S1 <==
Number of fluid steps= 2 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0247 &	 -0.0352016 \\
2 &			 1.06366 &	 -0.0538355 \\
3 &			 1.10668 &	 -0.0572011 \\
4 &			 1.12766 &	 -0.027094 \\


==> jagged_time_step/convRate/convRate_F2_S10 <==
Number of fluid steps= 2 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02989  &  \\
1 &			 1.09978 &	 -0.0947247 \\
2 &			 1.0691 &	 0.0408182 \\
3 &			 0.664408 &	 0.686255 \\
4 &			 0.268271 &	 1.30838 \\


==> jagged_time_step/convRate/convRate_F2_S11 <==
Number of fluid steps= 2 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03022  &  \\
1 &			 1.09814 &	 -0.0921095 \\
2 &			 1.06899 &	 0.0388136 \\
3 &			 0.664884 &	 0.685074 \\
4 &			 0.266073 &	 1.32128 \\


==> jagged_time_step/convRate/convRate_F2_S12 <==
Number of fluid steps= 2 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03067  &  \\
1 &			 1.10291 &	 -0.0977326 \\
2 &			 1.0684 &	 0.0458632 \\
3 &			 0.657758 &	 0.699823 \\
4 &			 0.259827 &	 1.34001 \\


==> jagged_time_step/convRate/convRate_F2_S13 <==
Number of fluid steps= 2 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03107  &  \\
1 &			 1.10134 &	 -0.0951176 \\
2 &			 1.06858 &	 0.043565 \\
3 &			 0.658866 &	 0.697638 \\
4 &			 0.258842 &	 1.34791 \\


==> jagged_time_step/convRate/convRate_F2_S14 <==
Number of fluid steps= 2 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03148  &  \\
1 &			 1.10535 &	 -0.0997874 \\
2 &			 1.06793 &	 0.0496862 \\
3 &			 0.653173 &	 0.70928 \\
4 &			 0.254184 &	 1.36159 \\


==> jagged_time_step/convRate/convRate_F2_S15 <==
Number of fluid steps= 2 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03196  &  \\
1 &			 1.10392 &	 -0.0972486 \\
2 &			 1.06829 &	 0.0473323 \\
3 &			 0.654607 &	 0.706602 \\
4 &			 0.253901 &	 1.36636 \\


==> jagged_time_step/convRate/convRate_F2_S16 <==
Number of fluid steps= 2 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03233  &  \\
1 &			 1.10731 &	 -0.101155 \\
2 &			 1.0676 &	 0.052688 \\
3 &			 0.649855 &	 0.716181 \\
4 &			 0.250218 &	 1.37693 \\


==> jagged_time_step/convRate/convRate_F2_S17 <==
Number of fluid steps= 2 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03288  &  \\
1 &			 1.10602 &	 -0.0987048 \\
2 &			 1.06809 &	 0.0503443 \\
3 &			 0.651454 &	 0.713298 \\
4 &			 0.25036 &	 1.37966 \\


==> jagged_time_step/convRate/convRate_F2_S18 <==
Number of fluid steps= 2 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03322  &  \\
1 &			 1.10891 &	 -0.101995 \\
2 &			 1.06736 &	 0.0550954 \\
3 &			 0.647364 &	 0.721398 \\
4 &			 0.247319 &	 1.3882 \\


==> jagged_time_step/convRate/convRate_F2_S19 <==
Number of fluid steps= 2 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03384  &  \\
1 &			 1.10777 &	 -0.0996454 \\
2 &			 1.06794 &	 0.0528278 \\
3 &			 0.649039 &	 0.718454 \\
4 &			 0.247726 &	 1.38956 \\


==> jagged_time_step/convRate/convRate_F2_S2 <==
Number of fluid steps= 2 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02422  &  \\
1 &			 1.06849 &	 -0.0610478 \\
2 &			 1.08069 &	 -0.0163793 \\
3 &			 0.805655 &	 0.423719 \\
4 &			 0.471993 &	 0.771397 \\


==> jagged_time_step/convRate/convRate_F2_S20 <==
Number of fluid steps= 2 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03414  &  \\
1 &			 1.11024 &	 -0.10244 \\
2 &			 1.06719 &	 0.0570545 \\
3 &			 0.645436 &	 0.725471 \\
4 &			 0.245132 &	 1.39672 \\


==> jagged_time_step/convRate/convRate_F2_S3 <==
Number of fluid steps= 2 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02415  &  \\
1 &			 1.0694 &	 -0.0623745 \\
2 &			 1.07651 &	 -0.00956014 \\
3 &			 0.773582 &	 0.476736 \\
4 &			 0.418724 &	 0.885555 \\


==> jagged_time_step/convRate/convRate_F2_S4 <==
Number of fluid steps= 2 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0271  &  \\
1 &			 1.08208 &	 -0.0752305 \\
2 &			 1.07524 &	 0.00914845 \\
3 &			 0.725441 &	 0.567729 \\
4 &			 0.352577 &	 1.04092 \\


==> jagged_time_step/convRate/convRate_F2_S5 <==
Number of fluid steps= 2 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02708  &  \\
1 &			 1.08129 &	 -0.0742049 \\
2 &			 1.07299 &	 0.0111169 \\
3 &			 0.715412 &	 0.58479 \\
4 &			 0.333159 &	 1.10256 \\


==> jagged_time_step/convRate/convRate_F2_S6 <==
Number of fluid steps= 2 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0283  &  \\
1 &			 1.09005 &	 -0.0841331 \\
2 &			 1.07201 &	 0.0240759 \\
3 &			 0.692031 &	 0.63141 \\
4 &			 0.305358 &	 1.18034 \\


==> jagged_time_step/convRate/convRate_F2_S7 <==
Number of fluid steps= 2 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02844  &  \\
1 &			 1.08872 &	 -0.0821753 \\
2 &			 1.07082 &	 0.023917 \\
3 &			 0.688582 &	 0.637016 \\
4 &			 0.296455 &	 1.21582 \\


==> jagged_time_step/convRate/convRate_F2_S8 <==
Number of fluid steps= 2 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02914  &  \\
1 &			 1.09565 &	 -0.0903478 \\
2 &			 1.07019 &	 0.0339201 \\
3 &			 0.674684 &	 0.665583 \\
4 &			 0.281762 &	 1.25973 \\


==> jagged_time_step/convRate/convRate_F2_S9 <==
Number of fluid steps= 2 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02937  &  \\
1 &			 1.09407 &	 -0.0879434 \\
2 &			 1.06966 &	 0.0325527 \\
3 &			 0.673907 &	 0.666531 \\
4 &			 0.277339 &	 1.2809 \\


==> jagged_time_step/convRate/convRate_F3_S1 <==
Number of fluid steps= 3 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02354 &	 -0.0335675 \\
2 &			 1.05762 &	 -0.0472539 \\
3 &			 1.10304 &	 -0.0606637 \\


==> jagged_time_step/convRate/convRate_F3_S10 <==
Number of fluid steps= 3 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05414  &  \\
1 &			 1.10473 &	 -0.0676273 \\
2 &			 0.882649 &	 0.323782 \\
3 &			 0.443573 &	 0.992668 \\
4 &			 0.181382 &	 1.29014 \\


==> jagged_time_step/convRate/convRate_F3_S11 <==
Number of fluid steps= 3 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05549  &  \\
1 &			 1.10699 &	 -0.0687293 \\
2 &			 0.878861 &	 0.332935 \\
3 &			 0.435511 &	 1.01293 \\
4 &			 0.174017 &	 1.32348 \\


==> jagged_time_step/convRate/convRate_F3_S12 <==
Number of fluid steps= 3 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0574  &  \\
1 &			 1.10439 &	 -0.0627285 \\
2 &			 0.865651 &	 0.351392 \\
3 &			 0.419359 &	 1.0456 \\
4 &			 0.16257 &	 1.36712 \\


==> jagged_time_step/convRate/convRate_F3_S13 <==
Number of fluid steps= 3 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05758  &  \\
1 &			 1.10652 &	 -0.0652627 \\
2 &			 0.870541 &	 0.346045 \\
3 &			 0.422064 &	 1.04445 \\
4 &			 0.1619 &	 1.38236 \\


==> jagged_time_step/convRate/convRate_F3_S14 <==
Number of fluid steps= 3 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05882  &  \\
1 &			 1.10809 &	 -0.0656177 \\
2 &			 0.86837 &	 0.351693 \\
3 &			 0.417401 &	 1.05688 \\
4 &			 0.157817 &	 1.40318 \\


==> jagged_time_step/convRate/convRate_F3_S15 <==
Number of fluid steps= 3 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06032  &  \\
1 &			 1.10536 &	 -0.0600166 \\
2 &			 0.858139 &	 0.365233 \\
3 &			 0.405899 &	 1.08009 \\
4 &			 0.150262 &	 1.43364 \\


==> jagged_time_step/convRate/convRate_F3_S16 <==
Number of fluid steps= 3 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0605  &  \\
1 &			 1.10742 &	 -0.0624579 \\
2 &			 0.862815 &	 0.360079 \\
3 &			 0.409059 &	 1.07674 \\
4 &			 0.150632 &	 1.44128 \\


==> jagged_time_step/convRate/convRate_F3_S17 <==
Number of fluid steps= 3 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06164  &  \\
1 &			 1.1086 &	 -0.0624443 \\
2 &			 0.861475 &	 0.363858 \\
3 &			 0.406094 &	 1.085 \\
4 &			 0.148135 &	 1.4549 \\


==> jagged_time_step/convRate/convRate_F3_S18 <==
Number of fluid steps= 3 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06287  &  \\
1 &			 1.10596 &	 -0.0573341 \\
2 &			 0.853126 &	 0.374468 \\
3 &			 0.397253 &	 1.1027 \\
4 &			 0.142653 &	 1.47755 \\


==> jagged_time_step/convRate/convRate_F3_S19 <==
Number of fluid steps= 3 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06303  &  \\
1 &			 1.1079 &	 -0.0596454 \\
2 &			 0.857502 &	 0.369616 \\
3 &			 0.4005 &	 1.09834 \\
4 &			 0.143526 &	 1.48049 \\


==> jagged_time_step/convRate/convRate_F3_S2 <==
Number of fluid steps= 3 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01313  &  \\
1 &			 1.06469 &	 -0.0716141 \\
2 &			 1.09962 &	 -0.0465716 \\
3 &			 1.03727 &	 0.0842136 \\
4 &			 0.981679 &	 0.0794682 \\


==> jagged_time_step/convRate/convRate_F3_S20 <==
Number of fluid steps= 3 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06407  &  \\
1 &			 1.10884 &	 -0.0594581 \\
2 &			 0.856635 &	 0.372299 \\
3 &			 0.398485 &	 1.10416 \\
4 &			 0.141888 &	 1.48977 \\


==> jagged_time_step/convRate/convRate_F3_S3 <==
Number of fluid steps= 3 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04252  &  \\
1 &			 1.09027 &	 -0.0646104 \\
2 &			 0.951307 &	 0.196703 \\
3 &			 0.596548 &	 0.673273 \\
4 &			 0.343489 &	 0.796374 \\


==> jagged_time_step/convRate/convRate_F3_S4 <==
Number of fluid steps= 3 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04247  &  \\
1 &			 1.09073 &	 -0.0652882 \\
2 &			 0.946816 &	 0.204138 \\
3 &			 0.576965 &	 0.7146 \\
4 &			 0.315791 &	 0.869514 \\


==> jagged_time_step/convRate/convRate_F3_S5 <==
Number of fluid steps= 3 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04502  &  \\
1 &			 1.09774 &	 -0.0710058 \\
2 &			 0.929583 &	 0.239881 \\
3 &			 0.535769 &	 0.794973 \\
4 &			 0.271903 &	 0.978519 \\


==> jagged_time_step/convRate/convRate_F3_S6 <==
Number of fluid steps= 3 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04967  &  \\
1 &			 1.09917 &	 -0.0664787 \\
2 &			 0.900469 &	 0.287666 \\
3 &			 0.486974 &	 0.886832 \\
4 &			 0.22842 &	 1.09216 \\


==> jagged_time_step/convRate/convRate_F3_S7 <==
Number of fluid steps= 3 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04977  &  \\
1 &			 1.10084 &	 -0.0685315 \\
2 &			 0.903779 &	 0.284563 \\
3 &			 0.483912 &	 0.901225 \\
4 &			 0.21979 &	 1.13862 \\


==> jagged_time_step/convRate/convRate_F3_S8 <==
Number of fluid steps= 3 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05132  &  \\
1 &			 1.10445 &	 -0.0711262 \\
2 &			 0.896367 &	 0.301167 \\
3 &			 0.467804 &	 0.938185 \\
4 &			 0.204279 &	 1.19536 \\


==> jagged_time_step/convRate/convRate_F3_S9 <==
Number of fluid steps= 3 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05397  &  \\
1 &			 1.10264 &	 -0.065128 \\
2 &			 0.877891 &	 0.328848 \\
3 &			 0.442289 &	 0.989052 \\
4 &			 0.184334 &	 1.26267 \\


==> jagged_time_step/convRate/convRate_F4_S1 <==
Number of fluid steps= 4 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02244 &	 -0.0320162 \\
2 &			 1.05271 &	 -0.0420919 \\
3 &			 1.09311 &	 -0.0543305 \\


==> jagged_time_step/convRate/convRate_F4_S10 <==
Number of fluid steps= 4 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06685  &  \\
1 &			 1.05 &	 0.022968 \\
2 &			 0.71699 &	 0.550364 \\
3 &			 0.341163 &	 1.07149 \\
4 &			 0.152242 &	 1.16409 \\


==> jagged_time_step/convRate/convRate_F4_S11 <==
Number of fluid steps= 4 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07054  &  \\
1 &			 1.05348 &	 0.0231758 \\
2 &			 0.713385 &	 0.56241 \\
3 &			 0.333678 &	 1.09622 \\
4 &			 0.144971 &	 1.20269 \\


==> jagged_time_step/convRate/convRate_F4_S12 <==
Number of fluid steps= 4 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07245  &  \\
1 &			 1.04401 &	 0.0387749 \\
2 &			 0.692166 &	 0.592946 \\
3 &			 0.313105 &	 1.14447 \\
4 &			 0.131393 &	 1.25276 \\


==> jagged_time_step/convRate/convRate_F4_S13 <==
Number of fluid steps= 4 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07295  &  \\
1 &			 1.04768 &	 0.0343847 \\
2 &			 0.699036 &	 0.583759 \\
3 &			 0.31579 &	 1.1464 \\
4 &			 0.130557 &	 1.27429 \\


==> jagged_time_step/convRate/convRate_F4_S14 <==
Number of fluid steps= 4 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07127  &  \\
1 &			 1.04302 &	 0.0385553 \\
2 &			 0.688734 &	 0.598748 \\
3 &			 0.30437 &	 1.17812 \\
4 &			 0.121974 &	 1.31925 \\


==> jagged_time_step/convRate/convRate_F4_S15 <==
Number of fluid steps= 4 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0744  &  \\
1 &			 1.0464 &	 0.0380968 \\
2 &			 0.68863 &	 0.603634 \\
3 &			 0.302521 &	 1.18669 \\
4 &			 0.120325 &	 1.3301 \\


==> jagged_time_step/convRate/convRate_F4_S16 <==
Number of fluid steps= 4 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07566  &  \\
1 &			 1.03863 &	 0.0505403 \\
2 &			 0.673546 &	 0.624833 \\
3 &			 0.289224 &	 1.21959 \\
4 &			 0.112203 &	 1.36608 \\


==> jagged_time_step/convRate/convRate_F4_S17 <==
Number of fluid steps= 4 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07617  &  \\
1 &			 1.042 &	 0.0465507 \\
2 &			 0.680021 &	 0.615704 \\
3 &			 0.292655 &	 1.21638 \\
4 &			 0.112658 &	 1.37725 \\


==> jagged_time_step/convRate/convRate_F4_S18 <==
Number of fluid steps= 4 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07423  &  \\
1 &			 1.03834 &	 0.049024 \\
2 &			 0.672678 &	 0.626291 \\
3 &			 0.284841 &	 1.23976 \\
4 &			 0.1067 &	 1.4166 \\


==> jagged_time_step/convRate/convRate_F4_S19 <==
Number of fluid steps= 4 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07694  &  \\
1 &			 1.04147 &	 0.0483166 \\
2 &			 0.67379 &	 0.62825 \\
3 &			 0.284958 &	 1.24155 \\
4 &			 0.106918 &	 1.41424 \\


==> jagged_time_step/convRate/convRate_F4_S2 <==
Number of fluid steps= 4 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02211  &  \\
1 &			 1.05944 &	 -0.0517514 \\
2 &			 1.10144 &	 -0.056089 \\
3 &			 1.12424 &	 -0.0295591 \\
4 &			 1.18376 &	 -0.0744266 \\


==> jagged_time_step/convRate/convRate_F4_S20 <==
Number of fluid steps= 4 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07784  &  \\
1 &			 1.0349 &	 0.0586517 \\
2 &			 0.662125 &	 0.644316 \\
3 &			 0.275323 &	 1.26598 \\
4 &			 0.101352 &	 1.44175 \\


==> jagged_time_step/convRate/convRate_F4_S3 <==
Number of fluid steps= 4 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04061  &  \\
1 &			 1.08993 &	 -0.066806 \\
2 &			 1.04319 &	 0.0632335 \\
3 &			 0.897305 &	 0.217332 \\
4 &			 0.814145 &	 0.140313 \\


==> jagged_time_step/convRate/convRate_F4_S4 <==
Number of fluid steps= 4 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05847  &  \\
1 &			 1.06556 &	 -0.00963145 \\
2 &			 0.806965 &	 0.401034 \\
3 &			 0.477817 &	 0.756048 \\
4 &			 0.274237 &	 0.801035 \\


==> jagged_time_step/convRate/convRate_F4_S5 <==
Number of fluid steps= 4 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05869  &  \\
1 &			 1.06748 &	 -0.0119288 \\
2 &			 0.807415 &	 0.402827 \\
3 &			 0.466344 &	 0.791916 \\
4 &			 0.258064 &	 0.853666 \\


==> jagged_time_step/convRate/convRate_F4_S6 <==
Number of fluid steps= 4 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0591  &  \\
1 &			 1.06043 &	 -0.00181058 \\
2 &			 0.775891 &	 0.450723 \\
3 &			 0.425638 &	 0.866227 \\
4 &			 0.227285 &	 0.905124 \\


==> jagged_time_step/convRate/convRate_F4_S7 <==
Number of fluid steps= 4 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0639  &  \\
1 &			 1.06385 &	 6.78038e-05 \\
2 &			 0.761163 &	 0.483017 \\
3 &			 0.39875 &	 0.932721 \\
4 &			 0.198898 &	 1.00346 \\


==> jagged_time_step/convRate/convRate_F4_S8 <==
Number of fluid steps= 4 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06753  &  \\
1 &			 1.0523 &	 0.0207306 \\
2 &			 0.726742 &	 0.534031 \\
3 &			 0.360135 &	 1.01291 \\
4 &			 0.170355 &	 1.07999 \\


==> jagged_time_step/convRate/convRate_F4_S9 <==
Number of fluid steps= 4 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.068  &  \\
1 &			 1.05601 &	 0.0162882 \\
2 &			 0.733139 &	 0.526465 \\
3 &			 0.360068 &	 1.02582 \\
4 &			 0.166162 &	 1.11568 \\


==> jagged_time_step/convRate/convRate_F5_S1 <==
Number of fluid steps= 5 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.02143 &	 -0.0305903 \\
2 &			 1.04866 &	 -0.0379567 \\


==> jagged_time_step/convRate/convRate_F5_S10 <==
Number of fluid steps= 5 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0701  &  \\
1 &			 0.969327 &	 0.14269 \\
2 &			 0.596856 &	 0.699601 \\
3 &			 0.286723 &	 1.05773 \\
4 &			 0.136658 &	 1.06909 \\


==> jagged_time_step/convRate/convRate_F5_S11 <==
Number of fluid steps= 5 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07161  &  \\
1 &			 0.97506 &	 0.136217 \\
2 &			 0.60425 &	 0.690345 \\
3 &			 0.287735 &	 1.0704 \\
4 &			 0.1344 &	 1.09821 \\


==> jagged_time_step/convRate/convRate_F5_S12 <==
Number of fluid steps= 5 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07029  &  \\
1 &			 0.971898 &	 0.139125 \\
2 &			 0.593959 &	 0.710442 \\
3 &			 0.275873 &	 1.10636 \\
4 &			 0.125772 &	 1.13319 \\


==> jagged_time_step/convRate/convRate_F5_S13 <==
Number of fluid steps= 5 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07208  &  \\
1 &			 0.967564 &	 0.147984 \\
2 &			 0.584823 &	 0.726357 \\
3 &			 0.26601 &	 1.13652 \\
4 &			 0.118319 &	 1.1688 \\


==> jagged_time_step/convRate/convRate_F5_S14 <==
Number of fluid steps= 5 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0723  &  \\
1 &			 0.964902 &	 0.152254 \\
2 &			 0.575995 &	 0.744326 \\
3 &			 0.257087 &	 1.1638 \\
4 &			 0.11213 &	 1.19708 \\


==> jagged_time_step/convRate/convRate_F5_S15 <==
Number of fluid steps= 5 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0712  &  \\
1 &			 0.949946 &	 0.17331 \\
2 &			 0.555675 &	 0.773604 \\
3 &			 0.24079 &	 1.20647 \\
4 &			 0.102342 &	 1.23438 \\


==> jagged_time_step/convRate/convRate_F5_S16 <==
Number of fluid steps= 5 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07271  &  \\
1 &			 0.95523 &	 0.16734 \\
2 &			 0.56305 &	 0.762585 \\
3 &			 0.243703 &	 1.20814 \\
4 &			 0.102293 &	 1.25242 \\


==> jagged_time_step/convRate/convRate_F5_S17 <==
Number of fluid steps= 5 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07146  &  \\
1 &			 0.953827 &	 0.167778 \\
2 &			 0.557335 &	 0.775183 \\
3 &			 0.23713 &	 1.23287 \\
4 &			 0.097206 &	 1.28656 \\


==> jagged_time_step/convRate/convRate_F5_S18 <==
Number of fluid steps= 5 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07296  &  \\
1 &			 0.951244 &	 0.173709 \\
2 &			 0.552622 &	 0.783522 \\
3 &			 0.232373 &	 1.24985 \\
4 &			 0.0938374 &	 1.30821 \\


==> jagged_time_step/convRate/convRate_F5_S19 <==
Number of fluid steps= 5 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07249  &  \\
1 &			 0.949995 &	 0.174972 \\
2 &			 0.548008 &	 0.793723 \\
3 &			 0.228281 &	 1.26339 \\
4 &			 0.0914663 &	 1.3195 \\


==> jagged_time_step/convRate/convRate_F5_S2 <==
Number of fluid steps= 5 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01738  &  \\
1 &			 1.05626 &	 -0.0541064 \\
2 &			 1.10178 &	 -0.0608712 \\
3 &			 1.15591 &	 -0.0691929 \\


==> jagged_time_step/convRate/convRate_F5_S20 <==
Number of fluid steps= 5 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07122  &  \\
1 &			 0.938306 &	 0.191124 \\
2 &			 0.533577 &	 0.814362 \\
3 &			 0.217592 &	 1.29407 \\
4 &			 0.0854429 &	 1.34859 \\


==> jagged_time_step/convRate/convRate_F5_S3 <==
Number of fluid steps= 5 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02705  &  \\
1 &			 1.08496 &	 -0.0791354 \\
2 &			 1.0859 &	 -0.0012494 \\
3 &			 1.0672 &	 0.0250607 \\
4 &			 1.10536 &	 -0.0506857 \\


==> jagged_time_step/convRate/convRate_F5_S4 <==
Number of fluid steps= 5 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06455  &  \\
1 &			 1.08133 &	 -0.0225632 \\
2 &			 0.949449 &	 0.187644 \\
3 &			 0.771417 &	 0.29958 \\
4 &			 0.683357 &	 0.174871 \\


==> jagged_time_step/convRate/convRate_F5_S5 <==
Number of fluid steps= 5 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06545  &  \\
1 &			 1.00699 &	 0.0814135 \\
2 &			 0.693507 &	 0.538067 \\
3 &			 0.403654 &	 0.780791 \\
4 &			 0.229625 &	 0.813839 \\


==> jagged_time_step/convRate/convRate_F5_S6 <==
Number of fluid steps= 5 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06652  &  \\
1 &			 1.01123 &	 0.0767999 \\
2 &			 0.696872 &	 0.537146 \\
3 &			 0.396303 &	 0.81429 \\
4 &			 0.219097 &	 0.855034 \\


==> jagged_time_step/convRate/convRate_F5_S7 <==
Number of fluid steps= 5 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06569  &  \\
1 &			 1.00365 &	 0.0865316 \\
2 &			 0.672788 &	 0.577032 \\
3 &			 0.368056 &	 0.870227 \\
4 &			 0.199518 &	 0.883406 \\


==> jagged_time_step/convRate/convRate_F5_S8 <==
Number of fluid steps= 5 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06848  &  \\
1 &			 0.995372 &	 0.102252 \\
2 &			 0.650266 &	 0.614206 \\
3 &			 0.340737 &	 0.932371 \\
4 &			 0.175954 &	 0.95346 \\


==> jagged_time_step/convRate/convRate_F5_S9 <==
Number of fluid steps= 5 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07032  &  \\
1 &			 0.989864 &	 0.11274 \\
2 &			 0.630087 &	 0.651679 \\
3 &			 0.317005 &	 0.991045 \\
4 &			 0.15679 &	 1.01567 \\


==> jagged_time_step/convRate/convRate_F6_S1 <==
Number of fluid steps= 6 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.0205 &	 -0.0292762 \\
2 &			 1.04525 &	 -0.0345719 \\


==> jagged_time_step/convRate/convRate_F6_S10 <==
Number of fluid steps= 6 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06056  &  \\
1 &			 0.9112 &	 0.218987 \\
2 &			 0.551638 &	 0.724046 \\
3 &			 0.282331 &	 0.966334 \\
4 &			 0.143288 &	 0.97847 \\


==> jagged_time_step/convRate/convRate_F6_S11 <==
Number of fluid steps= 6 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05914  &  \\
1 &			 0.904431 &	 0.227811 \\
2 &			 0.5346 &	 0.758551 \\
3 &			 0.263789 &	 1.01908 \\
4 &			 0.129376 &	 1.02781 \\


==> jagged_time_step/convRate/convRate_F6_S12 <==
Number of fluid steps= 6 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05435  &  \\
1 &			 0.879988 &	 0.260798 \\
2 &			 0.504881 &	 0.80154 \\
3 &			 0.239873 &	 1.07367 \\
4 &			 0.114482 &	 1.06715 \\


==> jagged_time_step/convRate/convRate_F6_S13 <==
Number of fluid steps= 6 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05739  &  \\
1 &			 0.886937 &	 0.253604 \\
2 &			 0.512224 &	 0.792057 \\
3 &			 0.241241 &	 1.0863 \\
4 &			 0.11318 &	 1.09186 \\


==> jagged_time_step/convRate/convRate_F6_S14 <==
Number of fluid steps= 6 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05564  &  \\
1 &			 0.882138 &	 0.259042 \\
2 &			 0.501674 &	 0.814254 \\
3 &			 0.231413 &	 1.11628 \\
4 &			 0.106829 &	 1.11517 \\


==> jagged_time_step/convRate/convRate_F6_S15 <==
Number of fluid steps= 6 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.053  &  \\
1 &			 0.874293 &	 0.268317 \\
2 &			 0.489667 &	 0.836316 \\
3 &			 0.22065 &	 1.15004 \\
4 &			 0.100417 &	 1.13576 \\


==> jagged_time_step/convRate/convRate_F6_S16 <==
Number of fluid steps= 6 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05497  &  \\
1 &			 0.87208 &	 0.27467 \\
2 &			 0.485333 &	 0.845486 \\
3 &			 0.215954 &	 1.16825 \\
4 &			 0.0959879 &	 1.1698 \\


==> jagged_time_step/convRate/convRate_F6_S17 <==
Number of fluid steps= 6 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05298  &  \\
1 &			 0.869493 &	 0.276232 \\
2 &			 0.478534 &	 0.861553 \\
3 &			 0.209245 &	 1.19343 \\
4 &			 0.0913981 &	 1.19496 \\


==> jagged_time_step/convRate/convRate_F6_S18 <==
Number of fluid steps= 6 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04895  &  \\
1 &			 0.852426 &	 0.299299 \\
2 &			 0.460449 &	 0.888533 \\
3 &			 0.196261 &	 1.23027 \\
4 &			 0.0840326 &	 1.22375 \\


==> jagged_time_step/convRate/convRate_F6_S19 <==
Number of fluid steps= 6 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05182  &  \\
1 &			 0.858539 &	 0.292932 \\
2 &			 0.467573 &	 0.876692 \\
3 &			 0.199032 &	 1.23219 \\
4 &			 0.0843018 &	 1.23937 \\


==> jagged_time_step/convRate/convRate_F6_S2 <==
Number of fluid steps= 6 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02031  &  \\
1 &			 1.05256 &	 -0.0448949 \\
2 &			 1.09785 &	 -0.0607785 \\


==> jagged_time_step/convRate/convRate_F6_S20 <==
Number of fluid steps= 6 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05054  &  \\
1 &			 0.855848 &	 0.295705 \\
2 &			 0.461185 &	 0.892009 \\
3 &			 0.193264 &	 1.25477 \\
4 &			 0.0803398 &	 1.26639 \\


==> jagged_time_step/convRate/convRate_F6_S3 <==
Number of fluid steps= 6 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03601  &  \\
1 &			 1.07879 &	 -0.0583761 \\
2 &			 1.10607 &	 -0.0360286 \\
3 &			 1.14948 &	 -0.0555387 \\
4 &			 1.23161 &	 -0.0995641 \\


==> jagged_time_step/convRate/convRate_F6_S4 <==
Number of fluid steps= 6 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05237  &  \\
1 &			 1.08074 &	 -0.0383775 \\
2 &			 1.02742 &	 0.0729934 \\
3 &			 0.97809 &	 0.0709869 \\
4 &			 0.997721 &	 -0.0286692 \\


==> jagged_time_step/convRate/convRate_F6_S5 <==
Number of fluid steps= 6 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07728  &  \\
1 &			 1.04434 &	 0.0448018 \\
2 &			 0.855717 &	 0.287386 \\
3 &			 0.67063 &	 0.351617 \\
4 &			 0.584997 &	 0.197088 \\


==> jagged_time_step/convRate/convRate_F6_S6 <==
Number of fluid steps= 6 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0599  &  \\
1 &			 0.936833 &	 0.178064 \\
2 &			 0.610213 &	 0.618479 \\
3 &			 0.352485 &	 0.791751 \\
4 &			 0.19803 &	 0.831843 \\


==> jagged_time_step/convRate/convRate_F6_S7 <==
Number of fluid steps= 6 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06246  &  \\
1 &			 0.943095 &	 0.171934 \\
2 &			 0.61465 &	 0.617638 \\
3 &			 0.347383 &	 0.823238 \\
4 &			 0.190639 &	 0.865684 \\


==> jagged_time_step/convRate/convRate_F6_S8 <==
Number of fluid steps= 6 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06001  &  \\
1 &			 0.932106 &	 0.185512 \\
2 &			 0.591838 &	 0.655292 \\
3 &			 0.32538 &	 0.863077 \\
4 &			 0.178121 &	 0.869268 \\


==> jagged_time_step/convRate/convRate_F6_S9 <==
Number of fluid steps= 6 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05828  &  \\
1 &			 0.917873 &	 0.205355 \\
2 &			 0.566563 &	 0.696058 \\
3 &			 0.301053 &	 0.912219 \\
4 &			 0.163456 &	 0.881115 \\


==> jagged_time_step/convRate/convRate_F7_S1 <==
Number of fluid steps= 7 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01965 &	 -0.028074 \\
2 &			 1.04234 &	 -0.0317519 \\


==> jagged_time_step/convRate/convRate_F7_S10 <==
Number of fluid steps= 7 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04132  &  \\
1 &			 0.85731 &	 0.280525 \\
2 &			 0.516389 &	 0.731359 \\
3 &			 0.276037 &	 0.903597 \\
4 &			 0.14954 &	 0.88433 \\


==> jagged_time_step/convRate/convRate_F7_S11 <==
Number of fluid steps= 7 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04072  &  \\
1 &			 0.844419 &	 0.301551 \\
2 &			 0.498466 &	 0.760464 \\
3 &			 0.257799 &	 0.951248 \\
4 &			 0.133972 &	 0.944315 \\


==> jagged_time_step/convRate/convRate_F7_S12 <==
Number of fluid steps= 7 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03817  &  \\
1 &			 0.834026 &	 0.315878 \\
2 &			 0.482387 &	 0.789901 \\
3 &			 0.242281 &	 0.99351 \\
4 &			 0.120704 &	 1.00521 \\


==> jagged_time_step/convRate/convRate_F7_S13 <==
Number of fluid steps= 7 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03319  &  \\
1 &			 0.824216 &	 0.326011 \\
2 &			 0.465121 &	 0.825416 \\
3 &			 0.226727 &	 1.03665 \\
4 &			 0.110134 &	 1.0417 \\


==> jagged_time_step/convRate/convRate_F7_S14 <==
Number of fluid steps= 7 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02457  &  \\
1 &			 0.799182 &	 0.358423 \\
2 &			 0.439299 &	 0.863321 \\
3 &			 0.207542 &	 1.0818 \\
4 &			 0.0986901 &	 1.07243 \\


==> jagged_time_step/convRate/convRate_F7_S15 <==
Number of fluid steps= 7 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02921  &  \\
1 &			 0.806631 &	 0.351557 \\
2 &			 0.44617 &	 0.854315 \\
3 &			 0.208989 &	 1.09417 \\
4 &			 0.0979118 &	 1.09387 \\


==> jagged_time_step/convRate/convRate_F7_S16 <==
Number of fluid steps= 7 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02692  &  \\
1 &			 0.804454 &	 0.352242 \\
2 &			 0.439236 &	 0.873014 \\
3 &			 0.202332 &	 1.11827 \\
4 &			 0.0934962 &	 1.11374 \\


==> jagged_time_step/convRate/convRate_F7_S17 <==
Number of fluid steps= 7 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.02512  &  \\
1 &			 0.799361 &	 0.358874 \\
2 &			 0.430694 &	 0.892184 \\
3 &			 0.194558 &	 1.14646 \\
4 &			 0.0888379 &	 1.13095 \\


==> jagged_time_step/convRate/convRate_F7_S18 <==
Number of fluid steps= 7 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0251  &  \\
1 &			 0.792998 &	 0.370376 \\
2 &			 0.423794 &	 0.903954 \\
3 &			 0.188397 &	 1.16959 \\
4 &			 0.0843845 &	 1.15873 \\


==> jagged_time_step/convRate/convRate_F7_S19 <==
Number of fluid steps= 7 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0228  &  \\
1 &			 0.78797 &	 0.376311 \\
2 &			 0.417303 &	 0.917045 \\
3 &			 0.18334 &	 1.18657 \\
4 &			 0.0809267 &	 1.17983 \\


==> jagged_time_step/convRate/convRate_F7_S2 <==
Number of fluid steps= 7 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01765  &  \\
1 &			 1.05003 &	 -0.0451891 \\
2 &			 1.09381 &	 -0.0589316 \\


==> jagged_time_step/convRate/convRate_F7_S20 <==
Number of fluid steps= 7 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01881  &  \\
1 &			 0.783267 &	 0.379309 \\
2 &			 0.409321 &	 0.936271 \\
3 &			 0.177077 &	 1.20886 \\
4 &			 0.077155 &	 1.19855 \\


==> jagged_time_step/convRate/convRate_F7_S3 <==
Number of fluid steps= 7 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03735  &  \\
1 &			 1.07673 &	 -0.0537538 \\
2 &			 1.12013 &	 -0.0570097 \\
3 &			 1.18074 &	 -0.0760251 \\


==> jagged_time_step/convRate/convRate_F7_S4 <==
Number of fluid steps= 7 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03771  &  \\
1 &			 1.0842 &	 -0.0632276 \\
2 &			 1.08217 &	 0.00270376 \\
3 &			 1.10884 &	 -0.0351241 \\
4 &			 1.17941 &	 -0.0890141 \\


==> jagged_time_step/convRate/convRate_F7_S5 <==
Number of fluid steps= 7 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05271  &  \\
1 &			 1.05815 &	 -0.0074361 \\
2 &			 0.9621 &	 0.137285 \\
3 &			 0.893732 &	 0.106345 \\
4 &			 0.898769 &	 -0.00810808 \\


==> jagged_time_step/convRate/convRate_F7_S6 <==
Number of fluid steps= 7 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.07649  &  \\
1 &			 0.993111 &	 0.116308 \\
2 &			 0.773487 &	 0.360578 \\
3 &			 0.591086 &	 0.388009 \\
4 &			 0.509931 &	 0.213066 \\


==> jagged_time_step/convRate/convRate_F7_S7 <==
Number of fluid steps= 7 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04279  &  \\
1 &			 0.869203 &	 0.262684 \\
2 &			 0.548601 &	 0.663936 \\
3 &			 0.314582 &	 0.802321 \\
4 &			 0.174311 &	 0.851773 \\


==> jagged_time_step/convRate/convRate_F7_S8 <==
Number of fluid steps= 7 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04717  &  \\
1 &			 0.87676 &	 0.256242 \\
2 &			 0.553189 &	 0.66441 \\
3 &			 0.310839 &	 0.831605 \\
4 &			 0.16884 &	 0.880511 \\


==> jagged_time_step/convRate/convRate_F7_S9 <==
Number of fluid steps= 7 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04374  &  \\
1 &			 0.869106 &	 0.264158 \\
2 &			 0.536449 &	 0.696091 \\
3 &			 0.294655 &	 0.864414 \\
4 &			 0.159632 &	 0.884277 \\


==> jagged_time_step/convRate/convRate_F8_S1 <==
Number of fluid steps= 8 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01887 &	 -0.02697 \\
2 &			 1.03984 &	 -0.0293916 \\


==> jagged_time_step/convRate/convRate_F8_S10 <==
Number of fluid steps= 8 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01895  &  \\
1 &			 0.80946 &	 0.332052 \\
2 &			 0.490888 &	 0.721566 \\
3 &			 0.269204 &	 0.866694 \\
4 &			 0.144672 &	 0.895914 \\


==> jagged_time_step/convRate/convRate_F8_S11 <==
Number of fluid steps= 8 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01754  &  \\
1 &			 0.799794 &	 0.347385 \\
2 &			 0.475459 &	 0.750308 \\
3 &			 0.255081 &	 0.898365 \\
4 &			 0.138291 &	 0.883248 \\


==> jagged_time_step/convRate/convRate_F8_S12 <==
Number of fluid steps= 8 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01028  &  \\
1 &			 0.782251 &	 0.369052 \\
2 &			 0.454001 &	 0.784936 \\
3 &			 0.238968 &	 0.925878 \\
4 &			 0.131515 &	 0.86159 \\


==> jagged_time_step/convRate/convRate_F8_S13 <==
Number of fluid steps= 8 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00902  &  \\
1 &			 0.776755 &	 0.377423 \\
2 &			 0.443231 &	 0.809401 \\
3 &			 0.224949 &	 0.978461 \\
4 &			 0.113794 &	 0.983173 \\


==> jagged_time_step/convRate/convRate_F8_S14 <==
Number of fluid steps= 8 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.00388  &  \\
1 &			 0.763551 &	 0.39479 \\
2 &			 0.427351 &	 0.837303 \\
3 &			 0.211638 &	 1.01382 \\
4 &			 0.103972 &	 1.0254 \\


==> jagged_time_step/convRate/convRate_F8_S15 <==
Number of fluid steps= 8 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.998593  &  \\
1 &			 0.755253 &	 0.402937 \\
2 &			 0.413551 &	 0.868895 \\
3 &			 0.199521 &	 1.05152 \\
4 &			 0.0958871 &	 1.05713 \\


==> jagged_time_step/convRate/convRate_F8_S16 <==
Number of fluid steps= 8 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.987522  &  \\
1 &			 0.731477 &	 0.433 \\
2 &			 0.391347 &	 0.902364 \\
3 &			 0.183871 &	 1.08975 \\
4 &			 0.0868258 &	 1.0825 \\


==> jagged_time_step/convRate/convRate_F8_S17 <==
Number of fluid steps= 8 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.993457  &  \\
1 &			 0.738946 &	 0.426989 \\
2 &			 0.39762 &	 0.894079 \\
3 &			 0.185292 &	 1.10159 \\
4 &			 0.0863575 &	 1.10141 \\


==> jagged_time_step/convRate/convRate_F8_S18 <==
Number of fluid steps= 8 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.990056  &  \\
1 &			 0.735552 &	 0.428683 \\
2 &			 0.390743 &	 0.912607 \\
3 &			 0.179697 &	 1.12065 \\
4 &			 0.0829082 &	 1.11598 \\


==> jagged_time_step/convRate/convRate_F8_S19 <==
Number of fluid steps= 8 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.99006  &  \\
1 &			 0.732067 &	 0.43554 \\
2 &			 0.384982 &	 0.927185 \\
3 &			 0.174051 &	 1.14528 \\
4 &			 0.0795047 &	 1.1304 \\


==> jagged_time_step/convRate/convRate_F8_S2 <==
Number of fluid steps= 8 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01878  &  \\
1 &			 1.04724 &	 -0.0397496 \\
2 &			 1.08842 &	 -0.0556433 \\


==> jagged_time_step/convRate/convRate_F8_S20 <==
Number of fluid steps= 8 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.985187  &  \\
1 &			 0.722586 &	 0.447228 \\
2 &			 0.374185 &	 0.949418 \\
3 &			 0.166389 &	 1.16919 \\
4 &			 0.0760942 &	 1.1287 \\


==> jagged_time_step/convRate/convRate_F8_S3 <==
Number of fluid steps= 8 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0269  &  \\
1 &			 1.07348 &	 -0.0639996 \\
2 &			 1.12402 &	 -0.0663724 \\


==> jagged_time_step/convRate/convRate_F8_S4 <==
Number of fluid steps= 8 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04524  &  \\
1 &			 1.08116 &	 -0.0487458 \\
2 &			 1.11035 &	 -0.0384345 \\
3 &			 1.177 &	 -0.0840998 \\
4 &			 1.26551 &	 -0.104605 \\


==> jagged_time_step/convRate/convRate_F8_S5 <==
Number of fluid steps= 8 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05521  &  \\
1 &			 1.06809 &	 -0.0175031 \\
2 &			 1.03722 &	 0.0423113 \\
3 &			 1.04772 &	 -0.0145313 \\
4 &			 1.10469 &	 -0.0763884 \\


==> jagged_time_step/convRate/convRate_F8_S6 <==
Number of fluid steps= 8 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.05713  &  \\
1 &			 1.01612 &	 0.057082 \\
2 &			 0.891119 &	 0.189381 \\
3 &			 0.812554 &	 0.133154 \\
4 &			 0.809252 &	 0.00587467 \\


==> jagged_time_step/convRate/convRate_F8_S7 <==
Number of fluid steps= 8 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.06373  &  \\
1 &			 0.93844 &	 0.180796 \\
2 &			 0.704147 &	 0.414388 \\
3 &			 0.527677 &	 0.416222 \\
4 &			 0.451291 &	 0.225597 \\


==> jagged_time_step/convRate/convRate_F8_S8 <==
Number of fluid steps= 8 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01772  &  \\
1 &			 0.809936 &	 0.329461 \\
2 &			 0.501699 &	 0.690986 \\
3 &			 0.285094 &	 0.815384 \\
4 &			 0.15578 &	 0.871928 \\


==> jagged_time_step/convRate/convRate_F8_S9 <==
Number of fluid steps= 8 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0239  &  \\
1 &			 0.818104 &	 0.323719 \\
2 &			 0.506067 &	 0.692956 \\
3 &			 0.282242 &	 0.842396 \\
4 &			 0.151569 &	 0.896958 \\


==> jagged_time_step/convRate/convRate_F9_S1 <==
Number of fluid steps= 9 
Number of solid steps= 1 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1  &  \\
1 &			 1.01814 &	 -0.025936 \\
2 &			 1.03756 &	 -0.0272588 \\


==> jagged_time_step/convRate/convRate_F9_S10 <==
Number of fluid steps= 9 
Number of solid steps= 10 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.996409  &  \\
1 &			 0.768494 &	 0.374704 \\
2 &			 0.468876 &	 0.712828 \\
3 &			 0.259112 &	 0.855631 \\
4 &			 0.137533 &	 0.913798 \\


==> jagged_time_step/convRate/convRate_F9_S11 <==
Number of fluid steps= 9 
Number of solid steps= 11 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.991487  &  \\
1 &			 0.762557 &	 0.378749 \\
2 &			 0.457204 &	 0.738007 \\
3 &			 0.248886 &	 0.877353 \\
4 &			 0.131965 &	 0.91533 \\


==> jagged_time_step/convRate/convRate_F9_S12 <==
Number of fluid steps= 9 
Number of solid steps= 12 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98659  &  \\
1 &			 0.749421 &	 0.396674 \\
2 &			 0.441076 &	 0.764749 \\
3 &			 0.237173 &	 0.895087 \\
4 &			 0.129151 &	 0.876881 \\


==> jagged_time_step/convRate/convRate_F9_S13 <==
Number of fluid steps= 9 
Number of solid steps= 13 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98338  &  \\
1 &			 0.741018 &	 0.40824 \\
2 &			 0.427115 &	 0.794884 \\
3 &			 0.224538 &	 0.927665 \\
4 &			 0.122399 &	 0.875368 \\


==> jagged_time_step/convRate/convRate_F9_S14 <==
Number of fluid steps= 9 
Number of solid steps= 14 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.98049  &  \\
1 &			 0.729277 &	 0.427036 \\
2 &			 0.413536 &	 0.818454 \\
3 &			 0.211498 &	 0.967369 \\
4 &			 0.11066 &	 0.93451 \\


==> jagged_time_step/convRate/convRate_F9_S15 <==
Number of fluid steps= 9 
Number of solid steps= 15 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.971526  &  \\
1 &			 0.716279 &	 0.439731 \\
2 &			 0.398958 &	 0.844285 \\
3 &			 0.199503 &	 0.999826 \\
4 &			 0.0990307 &	 1.01046 \\


==> jagged_time_step/convRate/convRate_F9_S16 <==
Number of fluid steps= 9 
Number of solid steps= 16 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.969115  &  \\
1 &			 0.70819 &	 0.452531 \\
2 &			 0.387807 &	 0.868798 \\
3 &			 0.189252 &	 1.03503 \\
4 &			 0.0915005 &	 1.04846 \\


==> jagged_time_step/convRate/convRate_F9_S17 <==
Number of fluid steps= 9 
Number of solid steps= 17 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.96114  &  \\
1 &			 0.698301 &	 0.460898 \\
2 &			 0.374302 &	 0.899646 \\
3 &			 0.178719 &	 1.06651 \\
4 &			 0.0849134 &	 1.07363 \\


==> jagged_time_step/convRate/convRate_F9_S18 <==
Number of fluid steps= 9 
Number of solid steps= 18 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.94899  &  \\
1 &			 0.676658 &	 0.487966 \\
2 &			 0.355242 &	 0.929625 \\
3 &			 0.165752 &	 1.09978 \\
4 &			 0.0775627 &	 1.09559 \\


==> jagged_time_step/convRate/convRate_F9_S19 <==
Number of fluid steps= 9 
Number of solid steps= 19 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.955776  &  \\
1 &			 0.683869 &	 0.482953 \\
2 &			 0.360918 &	 0.922049 \\
3 &			 0.167108 &	 1.11089 \\
4 &			 0.077289 &	 1.11245 \\


==> jagged_time_step/convRate/convRate_F9_S2 <==
Number of fluid steps= 9 
Number of solid steps= 2 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.01704  &  \\
1 &			 1.04519 &	 -0.0393888 \\
2 &			 1.32409 &	 -0.341236 \\


==> jagged_time_step/convRate/convRate_F9_S20 <==
Number of fluid steps= 9 
Number of solid steps= 20 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.952715  &  \\
1 &			 0.682102 &	 0.482057 \\
2 &			 0.356073 &	 0.937814 \\
3 &			 0.16303 &	 1.12704 \\
4 &			 0.074695 &	 1.12605 \\


==> jagged_time_step/convRate/convRate_F9_S3 <==
Number of fluid steps= 9 
Number of solid steps= 3 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.03108  &  \\
1 &			 1.06959 &	 -0.0529016 \\
2 &			 1.12214 &	 -0.0691948 \\


==> jagged_time_step/convRate/convRate_F9_S4 <==
Number of fluid steps= 9 
Number of solid steps= 4 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04951  &  \\
1 &			 1.08339 &	 -0.0458368 \\
2 &			 1.13211 &	 -0.0634615 \\
3 &			 1.94209 &	 -0.778596 \\


==> jagged_time_step/convRate/convRate_F9_S5 <==
Number of fluid steps= 9 
Number of solid steps= 5 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04145  &  \\
1 &			 1.07542 &	 -0.0463066 \\
2 &			 1.08836 &	 -0.0172556 \\
3 &			 1.14597 &	 -0.0744134 \\
4 &			 1.22691 &	 -0.0984601 \\


==> jagged_time_step/convRate/convRate_F9_S6 <==
Number of fluid steps= 9 
Number of solid steps= 6 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0521  &  \\
1 &			 1.03536 &	 0.0231393 \\
2 &			 0.981247 &	 0.0774442 \\
3 &			 0.97915 &	 0.00308645 \\
4 &			 1.02478 &	 -0.0657124 \\


==> jagged_time_step/convRate/convRate_F9_S7 <==
Number of fluid steps= 9 
Number of solid steps= 7 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.0431  &  \\
1 &			 0.974984 &	 0.097427 \\
2 &			 0.830433 &	 0.231515 \\
3 &			 0.745298 &	 0.156046 \\
4 &			 0.735287 &	 0.0195099 \\


==> jagged_time_step/convRate/convRate_F9_S8 <==
Number of fluid steps= 9 
Number of solid steps= 8 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 1.04248  &  \\
1 &			 0.886163 &	 0.234376 \\
2 &			 0.64617 &	 0.455658 \\
3 &			 0.476324 &	 0.439971 \\
4 &			 0.40443 &	 0.236053 \\


==> jagged_time_step/convRate/convRate_F9_S9 <==
Number of fluid steps= 9 
Number of solid steps= 9 
Refinement rate 	 Relative err 	 Order of time-conv
0 &			 0.988738  &  \\
1 &			 0.760213 &	 0.379185 \\
2 &			 0.464844 &	 0.709657 \\
3 &			 0.261343 &	 0.830802 \\
4 &			 0.140871 &	 0.89157 \\

